Thermodynamically consistent modeling of ion exchange membranes in multi-ionic environments

Ion exchange membranes are useful for a wide range of applications, including water desalination, fuel cells, and aqueous batteries. Accordingly, a variety of models for ion exchange membranes has been proposed, each emphasizing different aspects that govern their static and dynamic properties. By reviewing these models, we identify key physical contributions and beneficial modeling strategies. Based on these insights, we derive a thermodynamically consistent model by combining mass-action site occupation with mean-field electrostatic interactions along the polymer backbone. In this derivation, we explicitly account for multicomponent electrolytes at elevated concentrations. The parameters of the resulting model relate closely to those of other models, but gain consistency and interpretability through the underlying derivation. A discussion of the model parameters highlights redundancies and linkages between quantities that are commonly treated independently. Comparison to experimental data shows that both static and dynamic membrane properties are reproduced with good accuracy by the presented model. This makes it a promising basis for theory-driven membrane optimization and supports the tailored design of ion exchange membranes for various technologies.

==> 5_Results/Figures/Mixture_P_Mg_IOM.tex <==
x y z
5.0 5.0 -1.756769234298715e-10
5.0 6.344805015839611 -9.981505476500808e-11
5.0 8.051310137804697 -5.287706914309139e-11
5.0 10.216798589284712 -2.346043643343994e-11
5.0 12.96471898702334 -4.8421321887292604e-12
5.0 16.451722811563343 7.078935214222827e-12
5.0 20.87659468280201 1.4864817246737026e-11
5.0 26.491584531418546 2.014223513264233e-11
5.0 33.616787682496685 2.3954169891311752e-11
5.0 42.65839262086404 2.6971126079080737e-11
5.0 54.13183669370275 2.9620237618424135e-11
5.0 68.69118979416318 3.21631799190676e-11
5.0 87.16644110999944 3.473663430585456e-11
5.0 110.6108145535225 3.734789958181681e-11
5.0 140.3608101970589 3.9791314060000814e-11
5.0 178.11239451312218 4.162541789474961e-11
5.0 226.01768281801222 4.2766494681718223e-11
5.0 286.807625522434 4.3678383770145794e-11
5.0 363.94769219915764 4.4483958488572964e-11
5.0 461.8354285936932 4.498788398733193e-11
5.0 586.0511487667402 4.505629563991854e-11
5.0 743.6760536467558 4.469019053228929e-11
5.0 943.6959110675486 4.397659315355102e-11
5.0 1197.5133099937427 4.3036916422949756e-11
5.0 1519.5976911565988 4.199231356990644e-11
5.0 1928.3102105817359 4.094477496420017e-11
5.0 2446.9504592387466 3.997022905576265e-11
5.0 3105.0847094578075 3.91205385818316e-11
5.0 3940.2314078349555 3.8434331439749204e-11
5.0 5000.0 3.7968275500270484e-11

6.344805015839611 5.0 -2.6333914620552063e-10
6.344805015839611 6.344805015839611 -1.5840592820007323e-10
6.344805015839611 8.051310137804697 -9.245889872745768e-11
6.344805015839611 10.216798589284712 -5.039064446888034e-11
6.344805015839611 12.96471898702334 -2.3246499798265418e-11
6.344805015839611 16.451722811563343 -5.529299472248327e-12
6.344805015839611 20.87659468280201 6.221077378858085e-12
6.344805015839611 26.491584531418546 1.4221186400688221e-11
6.344805015839611 33.616787682496685 1.9907467730295126e-11
6.344805015839611 42.65839262086404 2.4215967402710994e-11
6.344805015839611 54.13183669370275 2.7754604865936005e-11
6.344805015839611 68.69118979416318 3.0908942215910266e-11
6.344805015839611 87.16644110999944 3.390092266233151e-11
6.344805015839611 110.6108145535225 3.679643459885146e-11
6.344805015839611 140.3608101970589 3.942932530164218e-11
6.344805015839611 178.11239451312218 4.138595326203474e-11
6.344805015839611 226.01768281801222 4.260715351984183e-11
6.344805015839611 286.807625522434 4.3572587141567204e-11
6.344805015839611 363.94769219915764 4.441266216674064e-11
6.344805015839611 461.8354285936932 4.493829974869814e-11
6.344805015839611 586.0511487667402 4.5020570828122335e-11
6.344805015839611 743.6760536467558 4.466365574049153e-11
6.344805015839611 943.6959110675486 4.395644896337198e-11
6.344805015839611 1197.5133099937427 4.302141842520661e-11
6.344805015839611 1519.5976911565988 4.1980306840333284e-11
6.344805015839611 1928.3102105817359 4.0935441819596453e-11
6.344805015839611 2446.9504592387466 3.996295657057938e-11
6.344805015839611 3105.0847094578075 3.911484959163941e-11
6.344805015839611 3940.2314078349555 3.8429846356253124e-11
6.344805015839611 5000.0 3.796469362922336e-11

8.051310137804697 5.0 -3.7201220010325237e-10
8.051310137804697 6.344805015839611 -2.3122147201051535e-10
8.051310137804697 8.051310137804697 -1.4175966163262338e-10
8.051310137804697 10.216798589284712 -8.399937689063286e-11
8.051310137804697 12.96471898702334 -4.6255081668470426e-11
8.051310137804697 16.451722811563343 -2.1316001768072725e-11
8.051310137804697 20.87659468280201 -4.6163809371779984e-12
8.051310137804697 26.491584531418546 6.788576614977039e-12
8.051310137804697 33.616787682496685 1.482240457320321e-11
8.051310137804697 42.65839262086404 2.075070503899557e-11
8.051310137804697 54.13183669370275 2.5406280748148876e-11
8.051310137804697 68.69118979416318 2.9329121990902914e-11
8.051310137804697 87.16644110999944 3.284765408919799e-11
8.051310137804697 110.6108145535225 3.6101051152580026e-11
8.051310137804697 140.3608101970589 3.897262340492749e-11
8.051310137804697 178.11239451312218 4.1083637172051e-11
8.051310137804697 226.01768281801222 4.2405872565962546e-11
8.051310137804697 286.807625522434 4.3438872173965145e-11
8.051310137804697 363.94769219915764 4.432249929005873e-11
8.051310137804697 461.8354285936932 4.487555850108036e-11
8.051310137804697 586.0511487667402 4.4975343645398745e-11
8.051310137804697 743.6760536467558 4.4630049007632073e-11
8.051310137804697 943.6959110675486 4.3930927604966046e-11
8.051310137804697 1197.5133099937427 4.30017783867773e-11
8.051310137804697 1519.5976911565988 4.19650880147879e-11
8.051310137804697 1928.3102105817359 4.0923609822968546e-11
8.051310137804697 2446.9504592387466 3.995373581499974e-11
8.051310137804697 3105.0847094578075 3.910763563450555e-11
8.051310137804697 3940.2314078349555 3.8424158400603413e-11
8.051310137804697 5000.0 3.796015053446251e-11

10.216798589284712 5.0 -5.059121648096189e-10
10.216798589284712 6.344805015839611 -3.2122149254446094e-10
10.216798589284712 8.051310137804697 -2.0286537679896084e-10
10.216798589284712 10.216798589284712 -1.2575879153462608e-10
10.216798589284712 12.96471898702334 -7.4906349793388e-11
10.216798589284712 16.451722811563343 -4.101239744583876e-11
10.216798589284712 20.87659468280201 -1.8160929431409142e-11
10.216798589284712 26.491584531418546 -2.514579868123489e-12
10.216798589284712 33.616787682496685 8.449223905287137e-12
10.216798589284712 42.65839262086404 1.6402660738582916e-11
10.216798589284712 54.13183669370275 2.2456780664245042e-11
10.216798589284712 68.69118979416318 2.7343154804390957e-11
10.216798589284712 87.16644110999944 3.1522623690643105e-11
10.216798589284712 110.6108145535225 3.522567605574462e-11
10.216798589284712 140.3608101970589 3.839732073374604e-11
10.216798589284712 178.11239451312218 4.070249778403158e-11
10.216798589284712 226.01768281801222 4.215192243688326e-11
10.216798589284712 286.807625522434 4.32700529248336e-11
10.216798589284712 363.94769219915764 4.420858190008708e-11
10.216798589284712 461.8354285936932 4.479622967217235e-11
10.216798589284712 586.0511487667402 4.491812251630936e-11
10.216798589284712 743.6760536467558 4.4587507528091936e-11
10.216798589284712 943.6959110675486 4.389860757525848e-11
10.216798589284712 1197.5133099937427 4.297689822828225e-11
10.216798589284712 1519.5976911565988 4.1945803611886865e-11
10.216798589284712 1928.3102105817359 4.090861377460559e-11
10.216798589284712 2446.9504592387466 3.994204721695976e-11
10.216798589284712 3105.0847094578075 3.9098489487447e-11
10.216798589284712 3940.2314078349555 3.841694610551767e-11
10.216798589284712 5000.0 3.7954389407123656e-11

12.96471898702334 5.0 -6.696390903312949e-10
12.96471898702334 6.344805015839611 -4.3170099663295695e-10
12.96471898702334 8.051310137804697 -2.7813766472145817e-10
12.96471898702334 10.216798589284712 -1.773593111183471e-10
12.96471898702334 12.96471898702334 -1.104071440622753e-10
12.96471898702334 16.451722811563343 -6.547700116627642e-11
12.96471898702334 20.87659468280201 -3.50205952303506e-11
12.96471898702334 26.491584531418546 -1.411664989693534e-11
12.96471898702334 33.616787682496685 4.879841235498241e-13
12.96471898702334 42.65839262086404 1.0963319116900096e-11
12.96471898702334 54.13183669370275 1.8762358125357147e-11
12.96471898702334 68.69118979416318 2.4852907258706758e-11
12.96471898702334 87.16644110999944 2.985958068825273e-11
12.96471898702334 110.6108145535225 3.4126088388762816e-11
12.96471898702334 140.3608101970589 3.767404277537678e-11
12.96471898702334 178.11239451312218 4.022281987066741e-11
12.96471898702334 226.01768281801222 4.1832015169075044e-11
12.96471898702334 286.807625522434 4.305720308952457e-11
12.96471898702334 363.94769219915764 4.4064818664672836e-11
12.96471898702334 461.8354285936932 4.4696024741174363e-11
12.96471898702334 586.0511487667402 4.484578425757038e-11
12.96471898702334 743.6760536467558 4.4533691105884493e-11
12.96471898702334 943.6959110675486 4.385769996363688e-11
12.96471898702334 1197.5133099937427 4.294539418470884e-11
12.96471898702334 1519.5976911565988 4.1921376959494234e-11
12.96471898702334 1928.3102105817359 4.0889613788587e-11
12.96471898702334 2446.9504592387466 3.992723436237613e-11
12.96471898702334 3105.0847094578075 3.90868965066464e-11
12.96471898702334 3940.2314078349555 3.840780278599979e-11
12.96471898702334 5000.0 3.794708478326451e-11

16.451722811563343 5.0 -8.67937181078909e-10
16.451722811563343 6.344805015839611 -5.66161709340932e-10
16.451722811563343 8.051310137804697 -3.7014815073458456e-10
16.451722811563343 10.216798589284712 -2.406789730747507e-10
16.451722811563343 12.96471898702334 -1.5412084563579666e-10
16.451722811563343 16.451722811563343 -9.569340061422646e-11
16.451722811563343 20.87659468280201 -5.590029913483641e-11
16.451722811563343 26.491584531418546 -2.851928580611915e-11
16.451722811563343 33.616787682496685 -9.415587637031555e-12
16.451722811563343 42.65839262086404 4.1845957713545445e-12
16.451722811563343 54.13183669370275 1.415092622538513e-11
16.451722811563343 68.69118979416318 2.1740278426465104e-11
16.451722811563343 87.16644110999944 2.777843686780471e-11
16.451722811563343 110.6108145535225 3.274862234010863e-11
16.451722811563343 140.3608101970589 3.676699432001432e-11
16.451722811563343 178.11239451312218 3.9620458057107445e-11
16.451722811563343 226.01768281801222 4.142980663888116e-11
16.451722811563343 286.807625522434 4.278930046842775e-11
16.451722811563343 363.94769219915764 4.388365661405162e-11
16.451722811563343 461.8354285936932 4.456960470247393e-11
16.451722811563343 586.0511487667402 4.475442705006788e-11
16.451722811563343 743.6760536467558 4.446566781692281e-11
16.451722811563343 943.6959110675486 4.38059585529597e-11
16.451722811563343 1197.5133099937427 4.2905525705333204e-11
16.451722811563343 1519.5976911565988 4.189045189880792e-11
16.451722811563343 1928.3102105817359 4.086555090578051e-11
16.451722811563343 2446.9504592387466 3.990846894274557e-11
16.451722811563343 3105.0847094578075 3.907220653302897e-11
16.451722811563343 3940.2314078349555 3.8396214512608934e-11
16.451722811563343 5000.0 3.793782527362151e-11

20.87659468280201 5.0 -1.105277604202068e-09
20.87659468280201 6.344805015839611 -7.28069670181164e-10
20.87659468280201 8.051310137804697 -4.815403900993519e-10
20.87659468280201 10.216798589284712 -3.177071754776927e-10
20.87659468280201 12.96471898702334 -2.075272104852614e-10
20.87659468280201 16.451722811563343 -1.3275067113961704e-10
20.87659468280201 20.87659468280201 -8.159361127239848e-11
20.87659468280201 26.491584531418546 -4.629511269637071e-11
20.87659468280201 33.616787682496685 -2.1670627988828485e-11
20.87659468280201 42.65839262086404 -4.222843506236915e-12
20.87659468280201 54.13183669370275 8.420110421559436e-12
20.87659468280201 68.69118979416318 1.7865402482196224e-11
20.87659468280201 87.16644110999944 2.5183779263287732e-11
20.87659468280201 110.6108145535225 3.102901265480395e-11
20.87659468280201 140.3608101970589 3.563307409912918e-11
20.87659468280201 178.11239451312218 3.8866143345058373e-11
20.87659468280201 226.01768281801222 4.092537229580041e-11
20.87659468280201 286.807625522434 4.245283960503451e-11
20.87659468280201 363.94769219915764 4.3655790771292594e-11
20.87659468280201 461.8354285936932 4.4410357756275664e-11
20.87659468280201 586.0511487667402 4.463919713470579e-11
20.87659468280201 743.6760536467558 4.4379777182256666e-11
20.87659468280201 943.6959110675486 4.3740571020738506e-11
20.87659468280201 1197.5133099937427 4.285510875974619e-11
20.87659468280201 1519.5976911565988 4.1851323770620934e-11
20.87659468280201 1928.3102105817359 4.083509204598845e-11
20.87659468280201 2446.9504592387466 3.988470694914768e-11
20.87659468280201 3105.0847094578075 3.9053599390607494e-11
20.87659468280201 3940.2314078349555 3.838153232782821e-11
20.87659468280201 5000.0 3.792609095271834e-11

26.491584531418546 5.0 -1.3852179542139197e-09
26.491584531418546 6.344805015839611 -9.204612236599983e-10
26.491584531418546 8.051310137804697 -6.147905717197016e-10
26.491584531418546 10.216798589284712 -4.1040187636857774e-10
26.491584531418546 12.96471898702334 -2.7213909361763453e-10
26.491584531418546 16.451722811563343 -1.7779626247615452e-10
26.491584531418546 20.87659468280201 -1.1295717772622975e-10
26.491584531418546 26.491584531418546 -6.807466364838422e-11
26.491584531418546 33.616787682496685 -3.6735097405935494e-11
26.491584531418546 42.65839262086404 -1.4587308806884736e-11
26.491584531418546 54.13183669370275 1.3376406270480514e-12
26.491584531418546 68.69118979416318 1.3066209846901552e-11
26.491584531418546 87.16644110999944 2.196415698622817e-11
26.491584531418546 110.6108145535225 2.889166824875651e-11
26.491584531418546 140.3608101970589 3.422120380584808e-11
26.491584531418546 178.11239451312218 3.7924872930384795e-11
26.491584531418546 226.01768281801222 4.0294705366645777e-11
26.491584531418546 286.807625522434 4.203143809845601e-11
26.491584531418546 363.94769219915764 4.3369853271350526e-11
26.491584531418546 461.8354285936932 4.421015134111237e-11
26.491584531418546 586.0511487667402 4.449408958150215e-11
26.491584531418546 743.6760536467558 4.4271469414036287e-11
26.491584531418546 943.6959110675486 4.36580290247133e-11
26.491584531418546 1197.5133099937427 4.279141113557833e-11
26.491584531418546 1519.5976911565988 4.18018553809294e-11
26.491584531418546 1928.3102105817359 4.0796562595329445e-11
26.491584531418546 2446.9504592387466 3.9854635065184505e-11
26.491584531418546 3105.0847094578075 3.9030041905619414e-11
26.491584531418546 3940.2314078349555 3.836293769811605e-11
26.491584531418546 5000.0 3.7911225785740354e-11

33.616787682496685 5.0 -1.7095193426558731e-09
33.616787682496685 6.344805015839611 -1.1453701195001811e-09
33.616787682496685 8.051310137804697 -7.718406470688154e-10
33.616787682496685 10.216798589284712 -5.204582016169059e-10
33.616787682496685 12.96471898702334 -3.4935898821118545e-10
33.616787682496685 16.451722811563343 -2.3194876807562966e-10
33.616787682496685 20.87659468280201 -1.5085885816064528e-10
33.616787682496685 26.491584531418546 -9.451635642621068e-11
33.616787682496685 33.616787682496685 -5.509896261787649e-11
33.616787682496685 42.65839262086404 -2.726706175930247e-11
33.616787682496685 54.13183669370275 -7.354090297849044e-12
33.616787682496685 68.69118979416318 7.160521054787409e-12
33.616787682496685 87.16644110999944 1.7992885099708576e-11
33.616787682496685 110.6108145535225 2.6249836610096934e-11
33.616787682496685 140.3608101970589 3.2472146068460334e-11
33.616787682496685 178.11239451312218 3.675553700970305e-11
33.616787682496685 226.01768281801222 3.950932554579598e-11
33.616787682496685 286.807625522434 4.1505485056886974e-11
33.616787682496685 363.94769219915764 4.3012106602612524e-11
33.616787682496685 461.8354285936932 4.3959069794294685e-11
33.616787682496685 586.0511487667402 4.4311727441078916e-11
33.616787682496685 743.6760536467558 4.4135121505369934e-11
33.616787682496685 943.6959110675486 4.355397650304155e-11
33.616787682496685 1197.5133099937427 4.271102810014526e-11
33.616787682496685 1519.5976911565988 4.173937583342936e-11
33.616787682496685 1928.3102105817359 4.074786526410841e-11
33.616787682496685 2446.9504592387466 3.9816604995775255e-11
33.616787682496685 3105.0847094578075 3.900023551342091e-11
33.616787682496685 3940.2314078349555 3.833940074855989e-11
33.616787682496685 5000.0 3.7892402945518475e-11

42.65839262086404 5.0 -2.0770647387757746e-09
42.65839262086404 6.344805015839611 -1.4030805960073744e-09
42.65839262086404 8.051310137804697 -9.535925523717849e-10
42.65839262086404 10.216798589284712 -6.489722790679132e-10
42.65839262086404 12.96471898702334 -4.4025960938604515e-10
42.65839262086404 16.451722811563343 -2.9615726938419e-10
42.65839262086404 20.87659468280201 -1.9608919283872833e-10
42.65839262086404 26.491584531418546 -1.2625181714707035e-10
42.65839262086404 33.616787682496685 -7.725110635859947e-11
42.65839262086404 42.65839262086404 -4.263072939355656e-11
42.65839262086404 54.13183669370275 -1.7926721745399204e-11
42.65839262086404 68.69118979416318 -4.761522131648994e-14
42.65839262086404 87.16644110999944 1.3131477665244439e-11
42.65839262086404 110.6108145535225 2.3007367992440376e-11
42.65839262086404 140.3608101970589 3.0319237284896846e-11
42.65839262086404 178.11239451312218 3.531102699661675e-11
42.65839262086404 226.01768281801222 3.853614356424753e-11
42.65839262086404 286.807625522434 4.0851914745406836e-11
42.65839262086404 363.94769219915764 4.256618572857797e-11
42.65839262086404 461.8354285936932 4.3645160708905595e-11
42.65839262086404 586.0511487667402 4.4083130237786194e-11
42.65839262086404 743.6760536467558 4.3963834695521815e-11
42.65839262086404 943.6959110675486 4.3423036885432486e-11
42.65839262086404 1197.5133099937427 4.2609738182071067e-11
42.65839262086404 1519.5976911565988 4.166056114604431e-11
42.65839262086404 1928.3102105817359 4.0686382058548124e-11
42.65839262086404 2446.9504592387466 3.976855449886351e-11
42.65839262086404 3105.0847094578075 3.89625519305578e-11
42.65839262086404 3940.2314078349555 3.8309627448878354e-11
42.65839262086404 5000.0 3.786858229829203e-11

54.13183669370275 5.0 -2.4827275027091677e-09
54.13183669370275 6.344805015839611 -1.6912737832708057e-09
54.13183669370275 8.051310137804697 -1.1592872265565703e-09
54.13183669370275 10.216798589284712 -7.960024271293708e-10
54.13183669370275 12.96471898702334 -5.452813762633698e-10
54.13183669370275 16.451722811563343 -3.709972927854897e-10
54.13183669370275 20.87659468280201 -2.492265072260432e-10
54.13183669370275 26.491584531418546 -1.6379836306595438e-10
54.13183669370275 33.616787682496685 -1.0362357403815857e-10
54.13183669370275 42.65839262086404 -6.102242670098205e-11
54.13183669370275 54.13183669370275 -3.0644512035221936e-11
54.13183669370275 68.69118979416318 -8.75502938981367e-12
54.13183669370275 87.16644110999944 7.2372622706846604e-12
54.13183669370275 110.6108145535225 1.906309162220151e-11
54.13183669370275 140.3608101970589 2.7690652998334726e-11
54.13183669370275 178.11239451312218 3.353918774403993e-11
54.13183669370275 226.01768281801222 3.7337805052083605e-11
54.13183669370275 286.807625522434 4.004423747390279e-11
54.13183669370275 363.94769219915764 4.201296342774717e-11
54.13183669370275 461.8354285936932 4.325423052330087e-11
54.13183669370275 586.0511487667402 4.379749358192869e-11
54.13183669370275 743.6760536467558 4.374922429821573e-11
54.13183669370275 943.6959110675486 4.325862520396629e-11
54.13183669370275 1197.5133099937427 4.248233974870397e-11
54.13183669370275 1519.5976911565988 4.15612967537995e-11
54.13183669370275 1928.3102105817359 4.060886008754608e-11
54.13183669370275 2446.9504592387466 3.970791298018711e-11
54.13183669370275 3105.0847094578075 3.8914956160263965e-11
54.13183669370275 3940.2314078349555 3.8271997316622796e-11
54.13183669370275 5000.0 3.7838458845883726e-11

68.69118979416318 5.0 -2.9164715511251233e-09
68.69118979416318 6.344805015839611 -2.0042258650106805e-09
68.69118979416318 8.051310137804697 -1.3858506205181155e-09
68.69118979416318 10.216798589284712 -9.600651742037438e-10
68.69118979416318 12.96471898702334 -6.638596954390003e-10
68.69118979416318 16.451722811563343 -4.5640393642077834e-10
68.69118979416318 20.87659468280201 -3.1045089049756256e-10
68.69118979416318 26.491584531418546 -2.07432328042306e-10
68.69118979416318 33.616787682496685 -1.3450710779545668e-10
68.69118979416318 42.65839262086404 -8.270653538283811e-11
68.69118979416318 54.13183669370275 -4.5728923150837275e-11
68.69118979416318 68.69118979416318 -1.9137141075386435e-11
68.69118979416318 87.16644110999944 1.7716607531917327e-13
68.69118979416318 110.6108145535225 1.4319147700806893e-11
68.69118979416318 140.3608101970589 2.4514029463071304e-11
68.69118979416318 178.11239451312218 3.138511178820102e-11
68.69118979416318 226.01768281801222 3.587383612147025e-11
68.69118979416318 286.807625522434 3.905302378211167e-11
68.69118979416318 363.94769219915764 4.1330653444550426e-11
68.69118979416318 461.8354285936932 4.276975555176111e-11
68.69118979416318 586.0511487667402 4.344201757637755e-11
68.69118979416318 743.6760536467558 4.3481223954727646e-11
68.69118979416318 943.6959110675486 4.305275525951031e-11
68.69118979416318 1197.5133099937427 4.2322476039398506e-11
68.69118979416318 1519.5976911565988 4.1436523977204e-11
68.69118979416318 1928.3102105817359 4.0511280664669103e-11
68.69118979416318 2446.9504592387466 3.963149198124519e-11
68.69118979416318 3105.0847094578075 3.885491555792261e-11
68.69118979416318 3940.2314078349555 3.8224487473779125e-11
68.69118979416318 5000.0 3.780039956963373e-11

87.16644110999944 5.0 -3.363065801585448e-09
87.16644110999944 6.344805015839611 -2.3323091678192243e-09
87.16644110999944 8.051310137804697 -1.627360994260326e-09
87.16644110999944 10.216798589284712 -1.1376542110681636e-09
87.16644110999944 12.96471898702334 -7.940278520450158e-10
87.16644110999944 16.451722811563343 -5.513627202062906e-10
87.16644110999944 20.87659468280201 -3.7931363282600104e-10
87.16644110999944 26.491584531418546 -2.570228402773148e-10
87.16644110999944 33.616787682496685 -1.6993467775293521e-10
87.16644110999944 42.65839262086404 -1.0778813473824057e-10
87.16644110999944 54.13183669370275 -6.330552109893123e-11
87.16644110999944 68.69118979416318 -3.1313293884868906e-11
87.16644110999944 87.16644110999944 -8.150084446163759e-12
87.16644110999944 110.6108145535225 8.694858618345135e-12
87.16644110999944 140.3608101970589 2.0724411483746913e-11
87.16644110999944 178.11239451312218 2.8795391879041773e-11
87.16644110999944 226.01768281801222 3.410301621212782e-11
87.16644110999944 286.807625522434 3.784711088925345e-11
87.16644110999944 363.94769219915764 4.049531566639852e-11
87.16644110999944 461.8354285936932 4.217300786160154e-11
87.16644110999944 586.0511487667402 4.300184430260681e-11
87.16644110999944 743.6760536467558 4.3147938486795525e-11
87.16644110999944 943.6959110675486 4.279586487986971e-11
87.16644110999944 1197.5133099937427 4.212245969860776e-11
87.16644110999944 1519.5976911565988 4.128007771712421e-11
87.16644110999944 1928.3102105817359 4.0388715542779475e-11
87.16644110999944 2446.9504592387466 3.953536119946718e-11
87.16644110999944 3105.0847094578075 3.8779294689527464e-11
87.16644110999944 3940.2314078349555 3.8164584417307543e-11
87.16644110999944 5000.0 3.775236978476156e-11

110.6108145535225 5.0 -3.802758860510637e-09
110.6108145535225 6.344805015839611 -2.66207681281815e-09
110.6108145535225 8.051310137804697 -1.8748414165727486e-09
110.6108145535225 10.216798589284712 -1.3229185254535013e-09
110.6108145535225 12.96471898702334 -9.320798185434104e-10
110.6108145535225 16.451722811563343 -6.536061649913581e-10
110.6108145535225 20.87659468280201 -4.5448668298118917e-10
110.6108145535225 26.491584531418546 -3.118366569075632e-10
110.6108145535225 33.616787682496685 -2.0953602014332097e-10
110.6108145535225 42.65839262086404 -1.3610845796437463e-10
110.6108145535225 54.13183669370275 -8.333119796526087e-11
110.6108145535225 68.69118979416318 -4.529749615951134e-11
110.6108145535225 87.16644110999944 -1.7781368404950896e-11
110.6108145535225 110.6108145535225 2.1476638204322828e-12
110.6108145535225 140.3608101970589 1.6276410881728256e-11
110.6108145535225 178.11239451312218 2.5724973701965647e-11
110.6108145535225 226.01768281801222 3.198748087260838e-11
110.6108145535225 286.807625522434 3.639586504769771e-11
110.6108145535225 363.94769219915764 3.9481977009021916e-11
110.6108145535225 461.8354285936932 4.1443532563412126e-11
110.6108145535225 586.0511487667402 4.246019144914826e-11
110.6108145535225 743.6760536467558 4.2735604118468343e-11
110.6108145535225 943.6959110675486 4.2476694428817244e-11
110.6108145535225 1197.5133099937427 4.1873120023573e-11
110.6108145535225 1519.5976911565988 4.1084528900195954e-11
110.6108145535225 1928.3102105817359 4.023517810714975e-11
110.6108145535225 2446.9504592387466 3.941471450681235e-11
110.6108145535225 3105.0847094578075 3.8684237955074735e-11
110.6108145535225 3940.2314078349555 3.808918291411246e-11
110.6108145535225 5000.0 3.769184545306312e-11

140.3608101970589 5.0 -4.2129708629839845e-09
140.3608101970589 6.344805015839611 -2.977084935923517e-09
140.3608101970589 8.051310137804697 -2.1165441533771794e-09
140.3608101970589 10.216798589284712 -1.5076414182281122e-09
140.3608101970589 12.96471898702334 -1.072398507324952e-09
140.3608101970589 16.451722811563343 -7.593874972656406e-10
140.3608101970589 20.87659468280201 -5.335365980995575e-10
140.3608101970589 26.491584531418546 -3.7033949139106166e-10
140.3608101970589 33.616787682496685 -2.523763556518788e-10
140.3608101970589 42.65839262086404 -1.6712130533805529e-10
140.3608101970589 54.13183669370275 -1.0550373244642314e-10
140.3608101970589 68.69118979416318 -6.093468046548491e-11
140.3608101970589 87.16644110999944 -2.864548574595756e-11
140.3608101970589 110.6108145535225 -5.298118081956536e-12
140.3608101970589 140.3608101970589 1.1160819627474731e-11
140.3608101970589 178.11239451312218 2.2147060459708348e-11
140.3608101970589 226.01768281801222 2.9499032367402704e-11
140.3608101970589 286.807625522434 3.4672847380529006e-11
140.3608101970589 363.94769219915764 3.826661497992331e-11
140.3608101970589 461.8354285936932 4.056015036527067e-11
140.3608101970589 586.0511487667402 4.179880306108752e-11
140.3608101970589 743.6760536467558 4.2228736310576806e-11
140.3608101970589 943.6959110675486 4.208227399048793e-11
140.3608101970589 1197.5133099937427 4.1563709378409654e-11
140.3608101970589 1519.5976911565988 4.0841055594548485e-11
140.3608101970589 1928.3102105817359 4.0043484582989897e-11
140.3608101970589 2446.9504592387466 3.926373502418778e-11
140.3608101970589 3105.0847094578075 3.856504529267758e-11
140.3608101970589 3940.2314078349555 3.799447459445895e-11
140.3608101970589 5000.0 3.7615716368180104e-11

178.11239451312218 5.0 -4.570522048995487e-09
178.11239451312218 6.344805015839611 -3.2592801348213693e-09
178.11239451312218 8.051310137804697 -2.338716806410911e-09
178.11239451312218 10.216798589284712 -1.6815811076084958e-09
178.11239451312218 12.96471898702334 -1.2075292166965704e-09
178.11239451312218 16.451722811563343 -8.634048859022736e-10
178.11239451312218 20.87659468280201 -6.127805600980104e-10
178.11239451312218 26.491584531418546 -4.300346817308902e-10
178.11239451312218 33.616787682496685 -2.968061335114087e-10
178.11239451312218 42.65839262086404 -1.997669136056605e-10
178.11239451312218 54.13183669370275 -1.2916317728410685e-10
178.11239451312218 68.69118979416318 -7.782747687697831e-11
178.11239451312218 87.16644110999944 -4.051061038333995e-11
178.11239451312218 110.6108145535225 -1.3516027793673243e-11
178.11239451312218 140.3608101970589 5.4241901054436605e-12
178.11239451312218 178.11239451312218 1.806596477040901e-11
178.11239451312218 226.01768281801222 2.6627897058790512e-11
178.11239451312218 286.807625522434 3.266112301857417e-11
178.11239451312218 363.94769219915764 3.682922230281323e-11
178.11239451312218 461.8354285936932 3.950266734993236e-11
178.11239451312218 586.0511487667402 4.099885961328724e-11
178.11239451312218 743.6760536467558 4.1610573116525696e-11
178.11239451312218 943.6959110675486 4.1598096977697586e-11
178.11239451312218 1197.5133099937427 4.118192430589602e-11
178.11239451312218 1519.5976911565988 4.0539381002771095e-11
178.11239451312218 1928.3102105817359 3.9805150641579056e-11
178.11239451312218 2446.9504592387466 3.907547546194031e-11
178.11239451312218 3105.0847094578075 3.8416050729342636e-11
178.11239451312218 3940.2314078349555 3.787583236295153e-11
178.11239451312218 5000.0 3.752017974609359e-11

226.01768281801222 5.0 -4.853506831389929e-09
226.01768281801222 6.344805015839611 -3.4904630219598086e-09
226.01768281801222 8.051310137804697 -2.5266305522059515e-09
226.01768281801222 10.216798589284712 -1.8331168569332596e-09
226.01768281801222 12.96471898702334 -1.3285286650347045e-09
226.01768281801222 16.451722811563343 -9.589422853204917e-10
226.01768281801222 20.87659468280201 -6.872965892098724e-10
226.01768281801222 26.491584531418546 -4.874025948770018e-10
226.01768281801222 33.616787682496685 -3.403710789618566e-10
226.01768281801222 42.65839262086404 -2.3237827123471774e-10
226.01768281801222 54.13183669370275 -1.5320797197475013e-10
226.01768281801222 68.69118979416318 -9.52672073168594e-11
226.01768281801222 87.16644110999944 -5.293035445473297e-11
226.01768281801222 110.6108145535225 -2.224159870889044e-11
226.01768281801222 140.3608101970589 -8.135480377118322e-13
226.01768281801222 178.11239451312218 1.3531850437883411e-11
226.01768281801222 226.01768281801222 2.3393559873245108e-11
226.01768281801222 286.807625522434 3.036011492970559e-11
226.01768281801222 363.94769219915764 3.51580242368316e-11
226.01768281801222 461.8354285936932 3.825442908983652e-11
226.01768281801222 586.0511487667402 4.004249050678386e-11
226.01768281801222 743.6760536467558 4.086393882339739e-11
226.01768281801222 943.6959110675486 4.1008580973242714e-11
226.01768281801222 1197.5133099937427 4.071411708003304e-11
226.01768281801222 1519.5976911565988 4.016783360237995e-11
226.01768281801222 1928.3102105817359 3.9510362926360954e-11
226.01768281801222 2446.9504592387466 3.884178083583983e-11
226.01768281801222 3105.0847094578075 3.8230521655771875e-11
226.01768281801222 3940.2314078349555 3.772770193257833e-11
226.01768281801222 5000.0 3.740063358488339e-11

286.807625522434 5.0 -5.04253069509608e-09
286.807625522434 6.344805015839611 -3.653654195941663e-09
286.807625522434 8.051310137804697 -2.665817288881622e-09
286.807625522434 10.216798589284712 -1.9502452753842983e-09
286.807625522434 12.96471898702334 -1.4256964708370207e-09
286.807625522434 16.451722811563343 -1.0383610850052938e-09
286.807625522434 20.87659468280201 -7.512225073446538e-10
286.807625522434 26.491584531418546 -5.380588603944652e-10
286.807625522434 33.616787682496685 -3.7987645661781816e-10
286.807625522434 42.65839262086404 -2.626884142095105e-10
286.807625522434 54.13183669370275 -1.76071604119632e-10
286.807625522434 68.69118979416318 -1.1219656415754118e-10
286.807625522434 87.16644110999944 -6.52036228196023e-11
286.807625522434 110.6108145535225 -3.105202640450751e-11
286.807625522434 140.3608101970589 -7.353028235414446e-12
286.807625522434 178.11239451312218 8.655234142367744e-12
286.807625522434 226.01768281801222 1.9856158416499896e-11
286.807625522434 286.807625522434 2.7793225363858792e-11
286.807625522434 363.94769219915764 3.3254579011315994e-11
286.807625522434 461.8354285936932 3.6805701084027456e-11
286.807625522434 586.0511487667402 3.8914975799456123e-11
286.807625522434 743.6760536467558 3.997264459526635e-11
286.807625522434 943.6959110675486 4.029792748406814e-11
286.807625522434 1197.5133099937427 4.014579345422675e-11
286.807625522434 1519.5976911565988 3.9713604959334164e-11
286.807625522434 1928.3102105817359 3.914808118308032e-11
286.807625522434 2446.9504592387466 3.8553293667746344e-11
286.807625522434 3105.0847094578075 3.8000607127091796e-11
286.807625522434 3940.2314078349555 3.754351985090082e-11
286.807625522434 5000.0 3.72515822075376e-11

363.94769219915764 5.0 -5.12252308058932e-09
363.94769219915764 6.344805015839611 -3.735095563230884e-09
363.94769219915764 8.051310137804697 -2.7439896984511263e-09
363.94769219915764 10.216798589284712 -2.022266694979881e-09
363.94769219915764 12.96471898702334 -1.4899593139701945e-09
363.94769219915764 16.451722811563343 -1.0941710490644692e-09
363.94769219915764 20.87659468280201 -7.985390496249589e-10
363.94769219915764 26.491584531418546 -5.772944029498031e-10
363.94769219915764 33.616787682496685 -4.117352612353642e-10
363.94769219915764 42.65839262086404 -2.880356816978856e-10
363.94769219915764 54.13183669370275 -1.9582605445905913e-10
363.94769219915764 68.69118979416318 -1.2724259278413529e-10
363.94769219915764 87.16644110999944 -7.63723124471427e-11
363.94769219915764 110.6108145535225 -3.940381926313321e-11
363.94769219915764 140.3608101970589 -1.3929628789372551e-11
363.94769219915764 178.11239451312218 3.6183747437878352e-12
363.94769219915764 226.01768281801222 1.612517056921696e-11
363.94769219915764 286.807625522434 2.5014399982827552e-11
363.94769219915764 363.94769219915764 3.1138911704992103e-11
363.94769219915764 461.8354285936932 3.515755374583759e-11
363.94769219915764 586.0511487667402 3.76075768655226e-11
363.94769219915764 743.6760536467558 3.8923481491273196e-11
363.94769219915764 943.6959110675486 3.945147807932252e-11
363.94769219915764 1197.5133099937427 3.946249755980807e-11
363.94769219915764 1519.5976911565988 3.9163294803026323e-11
363.94769219915764 1928.3102105817359 3.870634466195769e-11
363.94769219915764 2446.9504592387466 3.8199598130728744e-11
363.94769219915764 3105.0847094578075 3.7717375868801566e-11
363.94769219915764 3940.2314078349555 3.731568581233738e-11
363.94769219915764 5000.0 3.7066573867176495e-11

461.8354285936932 5.0 -5.0856326473242274e-09
461.8354285936932 6.344805015839611 -3.727004520879004e-09
461.8354285936932 8.051310137804697 -2.753577435079799e-09
461.8354285936932 10.216798589284712 -2.0420309617379523e-09
461.8354285936932 12.96471898702334 -1.514780796454373e-09
461.8354285936932 16.451722811563343 -1.120589583912817e-09
461.8354285936932 20.87659468280201 -8.242906349645702e-10
461.8354285936932 26.491584531418546 -6.00989403896418e-10
461.8354285936932 33.616787682496685 -4.326182930706979e-10
461.8354285936932 42.65839262086404 -3.0579551767984355e-10
461.8354285936932 54.13183669370275 -2.1043572277860128e-10
461.8354285936932 68.69118979416318 -1.3882836615415377e-10
461.8354285936932 87.16644110999944 -8.530984572839752e-11
461.8354285936932 110.6108145535225 -4.6819419696571004e-11
461.8354285936932 140.3608101970589 -2.023064936146721e-11
461.8354285936932 178.11239451312218 -1.3211714823670896e-12
461.8354285936932 226.01768281801222 1.2360019592567543e-11
461.8354285936932 286.807625522434 2.2110623929908744e-11
461.8354285936932 363.94769219915764 2.8853092214424295e-11
461.8354285936932 461.8354285936932 3.3325476000370424e-11
461.8354285936932 586.0511487667402 3.612067262511951e-11
461.8354285936932 743.6760536467558 3.7708722643305875e-11
461.8354285936932 943.6959110675486 3.84575984036012e-11
461.8354285936932 1197.5133099937427 3.865116336853951e-11
461.8354285936932 1519.5976911565988 3.8503833656712555e-11
461.8354285936932 1928.3102105817359 3.817286582539326e-11
461.8354285936932 2446.9504592387466 3.776957210811237e-11
461.8354285936932 3105.0847094578075 3.737099895194108e-11
461.8354285936932 3940.2314078349555 3.703563244361873e-11
461.8354285936932 5000.0 3.683820279655807e-11

586.0511487667402 5.0 -4.933485819517677e-09
586.0511487667402 6.344805015839611 -3.629581137559805e-09
586.0511487667402 8.051310137804697 -2.693596112075973e-09
586.0511487667402 10.216798589284712 -2.0076755515688064e-09
586.0511487667402 12.96471898702334 -1.4977371735302752e-09
586.0511487667402 16.451722811563343 -1.1149195476493568e-09
586.0511487667402 20.87659468280201 -8.257405670623259e-10
586.0511487667402 26.491584531418546 -6.065354769423446e-10
586.0511487667402 33.616787682496685 -4.401439008371038e-10
586.0511487667402 42.65839262086404 -3.1384106248268096e-10
586.0511487667402 54.13183669370275 -2.179874942945028e-10
586.0511487667402 68.69118979416318 -1.4527144927935594e-10
586.0511487667402 87.16644110999944 -9.12860304733162e-11
586.0511487667402 110.6108145535225 -5.315154800490981e-11
586.0511487667402 140.3608101970589 -2.5863529511433423e-11
586.0511487667402 178.11239451312218 -5.847318175936897e-12
586.0511487667402 226.01768281801222 8.756013377740528e-12
586.0511487667402 286.807625522434 1.9196741421513115e-11
586.0511487667402 363.94769219915764 2.646108683700477e-11
586.0511487667402 461.8354285936932 3.134145491140468e-11
586.0511487667402 586.0511487667402 3.446652566027584e-11
586.0511487667402 743.6760536467558 3.632881946456007e-11
586.0511487667402 943.6959110675486 3.730998501643195e-11
586.0511487667402 1197.5133099937427 3.770193947301469e-11
586.0511487667402 1519.5976911565988 3.77238417516412e-11
586.0511487667402 1928.3102105817359 3.75359880140335e-11
586.0511487667402 2446.9504592387466 3.725202320323575e-11
586.0511487667402 3105.0847094578075 3.695114241384799e-11
586.0511487667402 3940.2314078349555 3.669404478079916e-11
586.0511487667402 5000.0 3.655821694036848e-11

743.6760536467558 5.0 -4.677606992477832e-09
743.6760536467558 6.344805015839611 -3.4512043262568116e-09
743.6760536467558 8.051310137804697 -2.5698441890834133e-09
743.6760536467558 10.216798589284712 -1.9229035244740127e-09
743.6760536467558 12.96471898702334 -1.4408710330568752e-09
743.6760536467558 16.451722811563343 -1.0779299297456983e-09
743.6760536467558 20.87659468280201 -8.027120407820691e-10
743.6760536467558 26.491584531418546 -5.930614429660519e-10
743.6760536467558 33.616787682496685 -4.3289877217470314e-10
743.6760536467558 42.65839262086404 -3.102646061174438e-10
743.6760536467558 54.13183669370275 -2.1637675471306221e-10
743.6760536467558 68.69118979416318 -1.4617944478705436e-10
743.6760536467558 87.16644110999944 -9.543826609822009e-11
743.6760536467558 110.6108145535225 -5.8167206982770986e-11
743.6760536467558 140.3608101970589 -3.033369512414102e-11
743.6760536467558 178.11239451312218 -9.643059453247773e-12
743.6760536467558 226.01768281801222 5.511784693888891e-12
743.6760536467558 286.807625522434 1.6400171325415294e-11
743.6760536467558 363.94769219915764 2.40428960445537e-11
743.6760536467558 461.8354285936932 2.925304334148156e-11
743.6760536467558 586.0511487667402 3.267068916865771e-11
743.6760536467558 743.6760536467558 3.4794696021319954e-11
743.6760536467558 943.6959110675486 3.601008038418684e-11
743.6760536467558 1197.5133099937427 3.661035544634038e-11
743.6760536467558 1519.5976911565988 3.681540243764741e-11
743.6760536467558 1928.3102105817359 3.6786042025948946e-11
743.6760536467558 2446.9504592387466 3.663666762228483e-11
743.6760536467558 3105.0847094578075 3.64476342907667e-11
743.6760536467558 3940.2314078349555 3.628128792762983e-11
743.6760536467558 5000.0 3.6217785582135025e-11

943.6959110675486 5.0 -4.33299960815581e-09
943.6959110675486 6.344805015839611 -3.2028075799493894e-09
943.6959110675486 8.051310137804697 -2.3899535069148605e-09
943.6959110675486 10.216798589284712 -1.7925791957419006e-09
943.6959110675486 12.96471898702334 -1.3466640984613186e-09
943.6959110675486 16.451722811563343 -1.0099919442048813e-09
943.6959110675486 20.87659468280201 -7.536655041535604e-10
943.6959110675486 26.491584531418546 -5.579065418884446e-10
943.6959110675486 33.616787682496685 -4.0762710800488453e-10
943.6959110675486 42.65839262086404 -2.9470944666004154e-10
943.6959110675486 54.13183669370275 -2.1021915295051177e-10
943.6959110675486 68.69118979416318 -1.4644320456148185e-10
943.6959110675486 87.16644110999944 -9.79264706263294e-11
943.6959110675486 110.6108145535225 -6.105251832918251e-11
943.6959110675486 140.3608101970589 -3.3235860962624867e-11
943.6959110675486 178.11239451312218 -1.248491862534179e-11
943.6959110675486 226.01768281801222 2.783935994143714e-12
943.6959110675486 286.807625522434 1.3836967952673479e-11
943.6959110675486 363.94769219915764 2.1682557962973466e-11
943.6959110675486 461.8354285936932 2.711839959914468e-11
943.6959110675486 586.0511487667402 3.077103143408332e-11
943.6959110675486 743.6760536467558 3.3128833477869825e-11
943.6959110675486 943.6959110675486 3.4569044116728885e-11
943.6959110675486 1197.5133099937427 3.537950063658696e-11
943.6959110675486 1519.5976911565988 3.577608499518519e-11
943.6959110675486 1928.3102105817359 3.591704669359807e-11
943.6959110675486 2446.9504592387466 3.591546053456113e-11
943.6959110675486 3105.0847094578075 3.585144583880658e-11
943.6959110675486 3940.2314078349555 3.578809764811324e-11
943.6959110675486 5000.0 3.580798488423865e-11

1197.5133099937427 5.0 -3.871312005678583e-09
1197.5133099937427 6.344805015839611 -2.867073086753656e-09
1197.5133099937427 8.051310137804697 -2.1451291584647573e-09
1197.5133099937427 10.216798589284712 -1.614876852236628e-09
1197.5133099937427 12.96471898702334 -1.2193439592399274e-09
1197.5133099937427 16.451722811563343 -9.209466566929564e-10
1197.5133099937427 20.87659468280201 -6.939504874348115e-10
1197.5133099937427 26.491584531418546 -5.202254231331589e-10
1197.5133099937427 33.616787682496685 -3.867239167106995e-10
1197.5133099937427 42.65839262086404 -2.839025391592151e-10
1197.5133099937427 54.13183669370275 -2.046841024072265e-10
1197.5133099937427 68.69118979416318 -1.4374948940194717e-10
1197.5133099937427 87.16644110999944 -9.70461907411652e-11
1197.5133099937427 110.6108145535225 -6.144659017778373e-11
1197.5133099937427 140.3608101970589 -3.451043568465401e-11
1197.5133099937427 178.11239451312218 -1.431843116970776e-11
1197.5133099937427 226.01768281801222 6.465122334910139e-13
1197.5133099937427 286.807625522434 1.1586194650159017e-11
1197.5133099937427 363.94769219915764 1.9452484536825206e-11
1197.5133099937427 461.8354285936932 2.4997654785164507e-11
1197.5133099937427 586.0511487667402 2.8813853170709796e-11
1197.5133099937427 743.6760536467558 3.1364379721111795e-11
1197.5133099937427 943.6959110675486 3.3008574473235517e-11
1197.5133099937427 1197.5133099937427 3.4021679038237376e-11
1197.5133099937427 1519.5976911565988 3.461086327660041e-11
1197.5133099937427 1928.3102105817359 3.492855146816179e-11
1197.5133099937427 2446.9504592387466 3.508418681435998e-11
1197.5133099937427 3105.0847094578075 3.5155966648949385e-11
1197.5133099937427 3940.2314078349555 3.520655151818942e-11
1197.5133099937427 5000.0 3.532054914940362e-11

1519.5976911565988 5.0 -3.5652648330377083e-09
1519.5976911565988 6.344805015839611 -2.6449878394597947e-09
1519.5976911565988 8.051310137804697 -1.982767536528701e-09
1519.5976911565988 10.216798589284712 -1.495739352104231e-09
1519.5976911565988 12.96471898702334 -1.1318431440332994e-09
1519.5976911565988 16.451722811563343 -8.56787332115532e-10
1519.5976911565988 20.87659468280201 -6.471334192325107e-10
1519.5976911565988 26.491584531418546 -4.863856871554808e-10
1519.5976911565988 33.616787682496685 -3.6266042768919643e-10
1519.5976911565988 42.65839262086404 -2.6723353267287076e-10
1519.5976911565988 54.13183669370275 -1.9360057717802175e-10
1519.5976911565988 68.69118979416318 -1.3684880360398752e-10
1519.5976911565988 87.16644110999944 -9.322623330273434e-11
1519.5976911565988 110.6108145535225 -5.983965258012521e-11
1519.5976911565988 140.3608101970589 -3.4439346695841e-11
1519.5976911565988 178.11239451312218 -1.5263607457543355e-11
1519.5976911565988 226.01768281801222 -9.251345123394618e-13
1519.5976911565988 286.807625522434 9.67286349249456e-12
1519.5976911565988 363.94769219915764 1.7399342418463173e-11
1519.5976911565988 461.8354285936932 2.29428120730424e-11
1519.5976911565988 586.0511487667402 2.6847606797153708e-11
1519.5976911565988 743.6760536467558 2.954195849483657e-11
1519.5976911565988 943.6959110675486 3.135994854898245e-11
1519.5976911565988 1197.5133099937427 3.2558889541468087e-11
1519.5976911565988 1519.5976911565988 3.333339532166662e-11
1519.5976911565988 1928.3102105817359 3.382724108620671e-11
1519.5976911565988 2446.9504592387466 3.4144074765084614e-11
1519.5976911565988 3105.0847094578075 3.435844806292203e-11
1519.5976911565988 3940.2314078349555 3.45312771014737e-11
1519.5976911565988 5000.0 3.474891245051622e-11

1928.3102105817359 5.0 -3.227964612426676e-09
1928.3102105817359 6.344805015839611 -2.396667264661099e-09
1928.3102105817359 8.051310137804697 -1.7984099528320503e-09
1928.3102105817359 10.216798589284712 -1.3583465828660866e-09
1928.3102105817359 12.96471898702334 -1.0294525783755886e-09
1928.3102105817359 16.451722811563343 -7.807516252187632e-10
1928.3102105817359 20.87659468280201 -5.910703235286253e-10
1928.3102105817359 26.491584531418546 -4.4550715769007607e-10
1928.3102105817359 33.616787682496685 -3.3332812191887655e-10
1928.3102105817359 42.65839262086404 -2.4665560895020295e-10
1928.3102105817359 54.13183669370275 -1.796199703185512e-10
1928.3102105817359 68.69118979416318 -1.2779242007633864e-10
1928.3102105817359 87.16644110999944 -8.779551480103451e-11
1928.3102105817359 110.6108145535225 -5.702955680785523e-11
1928.3102105817359 140.3608101970589 -3.347698482883011e-11
1928.3102105817359 178.11239451312218 -1.5560595360460344e-11
1928.3102105817359 226.01768281801222 -2.0396852651056527e-12
1928.3102105817359 286.807625522434 8.06669049359199e-12
1928.3102105817359 363.94769219915764 1.5536869177452166e-11
1928.3102105817359 461.8354285936932 2.098946441552023e-11
1928.3102105817359 586.0511487667402 2.491579219895086e-11
1928.3102105817359 743.6760536467558 2.770458543713639e-11
1928.3102105817359 943.6959110675486 2.9661016075913586e-11
1928.3102105817359 1197.5133099937427 3.1021571966698965e-11
1928.3102105817359 1519.5976911565988 3.196605109809453e-11
1928.3102105817359 1928.3102105817359 3.262776959748522e-11
1928.3102105817359 2446.9504592387466 3.310303231809406e-11
1928.3102105817359 3105.0847094578075 3.346134831834296e-11
1928.3102105817359 3940.2314078349555 3.3760747065249945e-11
1928.3102105817359 5000.0 3.408952363711312e-11

2446.9504592387466 5.0 -2.9070461323984265e-09
2446.9504592387466 6.344805015839611 -2.159942081491911e-09
2446.9504592387466 8.051310137804697 -1.6222275626927837e-09
2446.9504592387466 10.216798589284712 -1.226641189735071e-09
2446.9504592387466 12.96471898702334 -9.309219230083085e-10
2446.9504592387466 16.451722811563343 -7.07229777547367e-10
2446.9504592387466 20.87659468280201 -5.365340711678234e-10
2446.9504592387466 26.491584531418546 -4.054409009183607e-10
2446.9504592387466 33.616787682496685 -3.043027098930925e-10
2446.9504592387466 42.65839262086404 -2.2604069714188322e-10
2446.9504592387466 54.13183669370275 -1.6538288185310854e-10
2446.9504592387466 68.69118979416318 -1.1835474517928747e-10
2446.9504592387466 87.16644110999944 -8.192909348603885e-11
2446.9504592387466 110.6108145535225 -5.3779702161144726e-11
2446.9504592387466 140.3608101970589 -3.2104706661192425e-11
2446.9504592387466 178.11239451312218 -1.5498176060213548e-11
2446.9504592387466 226.01768281801222 -2.855756417779191e-12
2446.9504592387466 286.807625522434 6.6951566307120416e-12
2446.9504592387466 363.94769219915764 1.3847360077080092e-11
2446.9504592387466 461.8354285936932 1.915263604189016e-11
2446.9504592387466 586.0511487667402 2.305082217705835e-11
2446.9504592387466 743.6760536467558 2.5891673876467814e-11
2446.9504592387466 943.6959110675486 2.795140338370594e-11
2446.9504592387466 1197.5133099937427 2.944537359346039e-11
2446.9504592387466 1519.5976911565988 3.0538183198333726e-11
2446.9504592387466 1928.3102105817359 3.135224935776406e-11
2446.9504592387466 2446.9504592387466 3.19759849170908e-11
2446.9504592387466 3105.0847094578075 3.247317373448181e-11
2446.9504592387466 3940.2314078349555 3.2898399605233e-11
2446.9504592387466 5000.0 3.3343409481030356e-11

3105.0847094578075 5.0 -2.6313064763317358e-09
3105.0847094578075 6.344805015839611 -1.9562098605691106e-09
3105.0847094578075 8.051310137804697 -1.4702925183059016e-09
3105.0847094578075 10.216798589284712 -1.1127780688332142e-09
3105.0847094578075 12.96471898702334 -8.454787152081019e-10
3105.0847094578075 16.451722811563343 -6.432364806668328e-10
3105.0847094578075 20.87659468280201 -4.888529107863471e-10
3105.0847094578075 26.491584531418546 -3.702228170083387e-10
3105.0847094578075 33.616787682496685 -2.786265394031439e-10
3105.0847094578075 42.65839262086404 -2.076663680056109e-10
3105.0847094578075 54.13183669370275 -1.52578548256757e-10
3105.0847094578075 68.69118979416318 -1.0977343870209026e-10
3105.0847094578075 87.16644110999944 -7.651936743612939e-11
3105.0847094578075 110.6108145535225 -5.072000209883347e-11
3105.0847094578075 140.3608101970589 -3.075444005972447e-11
3105.0847094578075 178.11239451312218 -1.53605636360677e-11
3105.0847094578075 226.01768281801222 -3.5490105887895435e-12
3105.0847094578075 286.807625522434 5.460718518693609e-12
3105.0847094578075 363.94769219915764 1.2287880948314849e-11
3105.0847094578075 461.8354285936932 1.7426019662047614e-11
3105.0847094578075 586.0511487667402 2.1269447783158385e-11
3105.0847094578075 743.6760536467558 2.413295692742873e-11
3105.0847094578075 943.6959110675486 2.6266476713431883e-11
3105.0847094578075 1197.5133099937427 2.7866063734854327e-11
3105.0847094578075 1519.5976911565988 2.9082403759316352e-11
3105.0847094578075 1928.3102105817359 3.002793624031738e-11
3105.0847094578075 2446.9504592387466 3.0783782761350014e-11
3105.0847094578075 3105.0847094578075 3.1408327940852633e-11
3105.0847094578075 3940.2314078349555 3.195324459531344e-11
3105.0847094578075 5000.0 3.2518124137108086e-11

3940.2314078349555 5.0 -2.4132777484455633e-09
3940.2314078349555 6.344805015839611 -1.794994165271882e-09
3940.2314078349555 8.051310137804697 -1.3499524902631423e-09
3940.2314078349555 10.216798589284712 -1.0224921207002663e-09
3940.2314078349555 12.96471898702334 -7.776387379492048e-10
3940.2314078349555 16.451722811563343 -5.923504373178042e-10
3940.2314078349555 20.87659468280201 -4.5087442094892734e-10
3940.2314078349555 26.491584531418546 -3.421221998364125e-10
3940.2314078349555 33.616787682496685 -2.5810583147297596e-10
3940.2314078349555 42.65839262086404 -1.9296414974492451e-10
3940.2314078349555 54.13183669370275 -1.4233301487321981e-10
3940.2314078349555 68.69118979416318 -1.0292453443121073e-10
3940.2314078349555 87.16644110999944 -7.223785217472486e-11
3940.2314078349555 110.6108145535225 -4.8355468485662375e-11
3940.2314078349555 140.3608101970589 -2.9796816542808145e-11
3940.2314078349555 178.11239451312218 -1.541123156446935e-11
3940.2314078349555 226.01768281801222 -4.298736387794774e-12
3940.2314078349555 286.807625522434 4.249055149751302e-12
3940.2314078349555 363.94769219915764 1.0793182295175622e-11
3940.2314078349555 461.8354285936932 1.5780444338377782e-11
3940.2314078349555 586.0511487667402 1.956807361694312e-11
3940.2314078349555 743.6760536467558 2.2441997708878648e-11
3940.2314078349555 943.6959110675486 2.4630250056558725e-11
3940.2314078349555 1197.5133099937427 2.6312790333551663e-11
3940.2314078349555 1519.5976911565988 2.7628841378730294e-11
3940.2314078349555 1928.3102105817359 2.868283244436078e-11
3940.2314078349555 2446.9504592387466 2.9550227670461054e-11
3940.2314078349555 3105.0847094578075 3.0285485548526216e-11
3940.2314078349555 3940.2314078349555 3.09396687965631e-11
3940.2314078349555 5000.0 3.163101822382368e-11

5000.0 5.0 -2.2608821880869176e-09
5000.0 6.344805015839611 -1.6823768761002923e-09
5000.0 8.051310137804697 -1.265957707550668e-09
5000.0 10.216798589284712 -9.595456703456238e-10
5000.0 12.96471898702334 -7.304163226127968e-10
5000.0 16.451722811563343 -5.570093703941529e-10
5000.0 20.87659468280201 -4.2458424552870286e-10
5000.0 26.491584531418546 -3.2276429435031574e-10
5000.0 33.616787682496685 -2.440737462048739e-10
5000.0 42.65839262086404 -1.83026748878542e-10
5000.0 54.13183669370275 -1.3553833747411978e-10
5000.0 68.69118979416318 -9.853097568543599e-11
5000.0 87.16644110999944 -6.966422763487101e-11
5000.0 110.6108145535225 -4.714444455416694e-11
5000.0 140.3608101970589 -2.9587952021978814e-11
5000.0 178.11239451312218 -1.592096169595357e-11
5000.0 226.01768281801222 -5.3053316389064576e-12
5000.0 286.807625522434 2.9170356703933966e-12
5000.0 363.94769219915764 9.266043236911576e-12
5000.0 461.8354285936932 1.415489684520437e-11
5000.0 586.0511487667402 1.791368768486626e-11
5000.0 743.6760536467558 2.080687058472526e-11
5000.0 943.6959110675486 2.3046035676868143e-11
5000.0 1197.5133099937427 2.4799111485832744e-11
5000.0 1519.5976911565988 2.6197015334390205e-11
5000.0 1928.3102105817359 2.7338801828732593e-11
5000.0 2446.9504592387466 2.8296705167241147e-11
5000.0 3105.0847094578075 2.912397141821213e-11
5000.0 3940.2314078349555 2.987640826766891e-11
5000.0 5000.0 3.0717923930562694e-11


==> 5_Results/Figures/Mixture_P_Mg_IOM_DM_diff.tex <==
x y z
5.0 5.0 0.9441435776549058
5.0 6.344805015839611 0.9556096925734091
5.0 8.051310137804697 0.979177546719098
5.0 10.216798589284712 1.0470738474591017
5.0 12.96471898702334 2.0104581851538743
5.0 16.451722811563343 0.6798610014477183
5.0 20.87659468280201 0.7900343907758793
5.0 26.491584531418546 0.8205294186597898
5.0 33.616787682496685 0.8339423765826354
5.0 42.65839262086404 0.8414706385365708
5.0 54.13183669370275 0.8469292659140425
5.0 68.69118979416318 0.852113018195934
5.0 87.16644110999944 0.8578812197004873
5.0 110.6108145535225 0.8638812958087865
5.0 140.3608101970589 0.8667889155230236
5.0 178.11239451312218 0.8601811054008446
5.0 226.01768281801222 0.8455341653134576
5.0 286.807625522434 0.8322980072172536
5.0 363.94769219915764 0.821607033162557
5.0 461.8354285936932 0.8103453586574013
5.0 586.0511487667402 0.7970039372526181
5.0 743.6760536467558 0.781498259532024
5.0 943.6959110675486 0.7644138859956763
5.0 1197.5133099937427 0.7466171490303788
5.0 1519.5976911565988 0.7290304860678695
5.0 1928.3102105817359 0.7124923599798622
5.0 2446.9504592387466 0.697686714709854
5.0 3105.0847094578075 0.6851479250565579
5.0 3940.2314078349555 0.6753849527887317
5.0 5000.0 0.669337343864734

6.344805015839611 5.0 0.9369302340480662
6.344805015839611 6.344805015839611 0.9435485719482479
6.344805015839611 8.051310137804697 0.9550992394323734
6.344805015839611 10.216798589284712 0.9786633336497168
6.344805015839611 12.96471898702334 1.04469437689421
6.344805015839611 16.451722811563343 1.7530127856902573
6.344805015839611 20.87659468280201 0.6522043808758664
6.344805015839611 26.491584531418546 0.7807940128878188
6.344805015839611 33.616787682496685 0.8154503310731352
6.344805015839611 42.65839262086404 0.8312383972367282
6.344805015839611 54.13183669370275 0.8408147643971438
6.344805015839611 68.69118979416318 0.848337410209457
6.344805015839611 87.16644110999944 0.8555263179586267
6.344805015839611 110.6108145535225 0.8624002070215786
6.344805015839611 140.3608101970589 0.8657939612738412
6.344805015839611 178.11239451312218 0.8593923883003053
6.344805015839611 226.01768281801222 0.8448682418178568
6.344805015839611 286.807625522434 0.8317497142920142
6.344805015839611 363.94769219915764 0.8211469192384139
6.344805015839611 461.8354285936932 0.8099503521274753
6.344805015839611 586.0511487667402 0.7966615726171069
6.344805015839611 743.6760536467558 0.7812019213547386
6.344805015839611 943.6959110675486 0.7641597015334103
6.344805015839611 1197.5133099937427 0.7464020214616379
6.344805015839611 1519.5976911565988 0.7288510896221799
6.344805015839611 1928.3102105817359 0.712344844340247
6.344805015839611 2446.9504592387466 0.6975668061400762
6.344805015839611 3105.0847094578075 0.6850511936896806
6.344805015839611 3940.2314078349555 0.6753070821653213
6.344805015839611 5000.0 0.669274416193239

8.051310137804697 5.0 0.9326170279979881
8.051310137804697 6.344805015839611 0.9370696250044959
8.051310137804697 8.051310137804697 0.9441851748272143
8.051310137804697 10.216798589284712 0.9567515023768469
8.051310137804697 12.96471898702334 0.9827791904443876
8.051310137804697 16.451722811563343 1.0582018155256256
8.051310137804697 20.87659468280201 2.2045964174506762
8.051310137804697 26.491584531418546 0.661509975135889
8.051310137804697 33.616787682496685 0.7803118910391185
8.051310137804697 42.65839262086404 0.8150311717716824
8.051310137804697 54.13183669370275 0.8319949228285416
8.051310137804697 68.69118979416318 0.8431737662940144
8.051310137804697 87.16644110999944 0.8524066587496569
8.051310137804697 110.6108145535225 0.8604762152916509
8.051310137804697 140.3608101970589 0.8645165708189709
8.051310137804697 178.11239451312218 0.85838587356449
8.051310137804697 226.01768281801222 0.8440211896411578
8.051310137804697 286.807625522434 0.8310534868167827
8.051310137804697 363.94769219915764 0.8205632272777601
8.051310137804697 461.8354285936932 0.8094495134955997
8.051310137804697 586.0511487667402 0.7962275765328608
8.051310137804697 743.6760536467558 0.7808262947629288
8.051310137804697 943.6959110675486 0.7638375035765925
8.051310137804697 1197.5133099937427 0.7461293155096678
8.051310137804697 1519.5976911565988 0.7286236603588125
8.051310137804697 1928.3102105817359 0.7121578147296632
8.051310137804697 2446.9504592387466 0.6974147667597735
8.051310137804697 3105.0847094578075 0.6849285300158945
8.051310137804697 3940.2314078349555 0.6752083263637986
8.051310137804697 5000.0 0.6691946017713161

10.216798589284712 5.0 0.929729269587311
10.216798589284712 6.344805015839611 0.9330310559492997
10.216798589284712 8.051310137804697 0.9380067157416759
10.216798589284712 10.216798589284712 0.946091499418958
10.216798589284712 12.96471898702334 0.960669933452516
10.216798589284712 16.451722811563343 0.9919607446707971
10.216798589284712 20.87659468280201 1.0917986728597942
10.216798589284712 26.491584531418546 8.13501897725371
10.216798589284712 33.616787682496685 0.6922235784482235
10.216798589284712 42.65839262086404 0.7866086388918929
10.216798589284712 54.13183669370275 0.8186556053309257
10.216798589284712 68.69118979416318 0.8359381212576695
10.216798589284712 87.16644110999944 0.8482203271461763
10.216798589284712 110.6108145535225 0.8579601711906558
10.216798589284712 140.3608101970589 0.862871296319677
10.216798589284712 178.11239451312218 0.8570994640963245
10.216798589284712 226.01768281801222 0.8429430592859736
10.216798589284712 286.807625522434 0.8301692595966936
10.216798589284712 363.94769219915764 0.8198228307327199
10.216798589284712 461.8354285936932 0.8088146309045413
10.216798589284712 586.0511487667402 0.7956775786660383
10.216798589284712 743.6760536467558 0.7803503072798503
10.216798589284712 943.6959110675486 0.763429212631485
10.216798589284712 1197.5133099937427 0.7457837166911432
10.216798589284712 1519.5976911565988 0.7283354106854744
10.216798589284712 1928.3102105817359 0.7119207410113054
10.216798589284712 2446.9504592387466 0.6972220232698548
10.216798589284712 3105.0847094578075 0.6847730073084748
10.216798589284712 3940.2314078349555 0.6750831033769669
10.216798589284712 5000.0 0.6690933890309667

12.96471898702334 5.0 0.9276404975464524
12.96471898702334 6.344805015839611 0.9302652126304157
12.96471898702334 8.051310137804697 0.934049756442894
12.96471898702334 10.216798589284712 0.9398554373516672
12.96471898702334 12.96471898702334 0.9494868744641332
12.96471898702334 16.451722811563343 0.9673921893500298
12.96471898702334 20.87659468280201 1.0082226422105862
12.96471898702334 26.491584531418546 1.1662676454148564
12.96471898702334 33.616787682496685 0.1310098965680786
12.96471898702334 42.65839262086404 0.7265858742885837
12.96471898702334 54.13183669370275 0.7969661067814844
12.96471898702334 68.69118979416318 0.8254471258270154
12.96471898702334 87.16644110999944 0.8425047863503639
12.96471898702334 110.6108145535225 0.8546411565020049
12.96471898702334 140.3608101970589 0.8607434508045291
12.96471898702334 178.11239451312218 0.8554521433538377
12.96471898702334 226.01768281801222 0.841569712559047
12.96471898702334 286.807625522434 0.8290460337192217
12.96471898702334 363.94769219915764 0.8188837752039372
12.96471898702334 461.8354285936932 0.8080100584458595
12.96471898702334 586.0511487667402 0.7949808218796441
12.96471898702334 743.6760536467558 0.7797473718029246
12.96471898702334 943.6959110675486 0.7629120170373113
12.96471898702334 1197.5133099937427 0.7453458956125925
12.96471898702334 1519.5976911565988 0.7279701954936384
12.96471898702334 1928.3102105817359 0.7116203213501532
12.96471898702334 2446.9504592387466 0.6969777406341332
12.96471898702334 3105.0847094578075 0.6845758705368108
12.96471898702334 3940.2314078349555 0.6749243512360292
12.96471898702334 5000.0 0.6689650606416865

16.451722811563343 5.0 0.9260543663459305
16.451722811563343 6.344805015839611 0.9282494795358612
16.451722811563343 8.051310137804697 0.9313090430246378
16.451722811563343 10.216798589284712 0.9358029615120177
16.451722811563343 12.96471898702334 0.9428353625315484
16.451722811563343 16.451722811563343 0.9548077600472332
16.451722811563343 20.87659468280201 0.9780538248571756
16.451722811563343 26.491584531418546 1.0365348251396798
16.451722811563343 33.616787682496685 1.3795999678259918
16.451722811563343 42.65839262086404 0.5292297766861265
16.451722811563343 54.13183669370275 0.7571932802150851
16.451722811563343 68.69118979416318 0.8094610325898679
16.451722811563343 87.16644110999944 0.8345152663877998
16.451722811563343 110.6108145535225 0.8502124944958895
16.451722811563343 140.3608101970589 0.8579768716732918
16.451722811563343 178.11239451312218 0.8533374687347033
16.451722811563343 226.01768281801222 0.8398185409345121
16.451722811563343 286.807625522434 0.8276188515373707
16.451722811563343 363.94769219915764 0.8176929419383627
16.451722811563343 461.8354285936932 0.8069908173827632
16.451722811563343 586.0511487667402 0.7940985467985965
16.451722811563343 743.6760536467558 0.7789839962514308
16.451722811563343 943.6959110675486 0.762257176834055
16.451722811563343 1197.5133099937427 0.7447914903777021
16.451722811563343 1519.5976911565988 0.7275076540317835
16.451722811563343 1928.3102105817359 0.7112397739350288
16.451722811563343 2446.9504592387466 0.696668243192806
16.451722811563343 3105.0847094578075 0.6843260578101119
16.451722811563343 3940.2314078349555 0.6747231451157994
16.451722811563343 5000.0 0.668802389810893

20.87659468280201 5.0 0.9248380515352146
20.87659468280201 6.344805015839611 0.9267355065728772
20.87659468280201 8.051310137804697 0.9293206963138674
20.87659468280201 10.216798589284712 0.9329954361368247
20.87659468280201 12.96471898702334 0.9384984089591225
20.87659468280201 16.451722811563343 0.9473072540561789
20.87659468280201 20.87659468280201 0.9628145092977005
20.87659468280201 26.491584531418546 0.9948957893462688
20.87659468280201 33.616787682496685 1.090188965574136
20.87659468280201 42.65839262086404 4.227966358797827
20.87659468280201 54.13183669370275 0.6651852148472659
20.87659468280201 68.69118979416318 0.7831654105013108
20.87659468280201 87.16644110999944 0.8229725944492904
20.87659468280201 110.6108145535225 0.8442123230322555
20.87659468280201 140.3608101970589 0.8543550463009296
20.87659468280201 178.11239451312218 0.8506143513197236
20.87659468280201 226.01768281801222 0.8375827499271333
20.87659468280201 286.807625522434 0.8258048961166494
20.87659468280201 363.94769219915764 0.8161831500429647
20.87659468280201 461.8354285936932 0.8057002426027216
20.87659468280201 586.0511487667402 0.7929820039450751
20.87659468280201 743.6760536467558 0.7780180742719852
20.87659468280201 943.6959110675486 0.7614285558504452
20.87659468280201 1197.5133099937427 0.7440898537595043
20.87659468280201 1519.5976911565988 0.7269221561330242
20.87659468280201 1928.3102105817359 0.7107579547025659
20.87659468280201 2446.9504592387466 0.6962762856604442
20.87659468280201 3105.0847094578075 0.6840096117650397
20.87659468280201 3940.2314078349555 0.6744682148761462
20.87659468280201 5000.0 0.6685962437628661

26.491584531418546 5.0 0.923966346429081
26.491584531418546 6.344805015839611 0.9256243750977787
26.491584531418546 8.051310137804697 0.9278685779032373
26.491584531418546 10.216798589284712 0.9309934454145348
26.491584531418546 12.96471898702334 0.9355237307780434
26.491584531418546 16.451722811563343 0.9424504266665825
26.491584531418546 20.87659468280201 0.953844418692589
26.491584531418546 26.491584531418546 0.9748355962078344
26.491584531418546 33.616787682496685 1.022697583065751
26.491584531418546 42.65839262086404 1.2182014984788223
26.491584531418546 54.13183669370275 0.2568471206510201
26.491584531418546 68.69118979416318 0.7339724517397226
26.491584531418546 87.16644110999944 0.8054792256758743
26.491584531418546 110.6108145535225 0.8359132029696612
26.491584531418546 140.3608101970589 0.8495709967317067
26.491584531418546 178.11239451312218 0.8470936696492986
26.491584531418546 226.01768281801222 0.8347236803167205
26.491584531418546 286.807625522434 0.8234985123359152
26.491584531418546 363.94769219915764 0.8142695250968479
26.491584531418546 461.8354285936932 0.8040670972296933
26.491584531418546 586.0511487667402 0.791570031189008
26.491584531418546 743.6760536467558 0.776796808094104
26.491584531418546 943.6959110675486 0.7603808284560917
26.491584531418546 1197.5133099937427 0.7432025222863686
26.491584531418546 1519.5976911565988 0.726181508190928
26.491584531418546 1928.3102105817359 0.7101482754348288
26.491584531418546 2446.9504592387466 0.6957801627319187
26.491584531418546 3105.0847094578075 0.6836089454618103
26.491584531418546 3940.2314078349555 0.6741453446049757
26.491584531418546 5000.0 0.6683350990020422

33.616787682496685 5.0 0.9235100918214235
33.616787682496685 6.344805015839611 0.9249263325714346
33.616787682496685 8.051310137804697 0.9268834334683484
33.616787682496685 10.216798589284712 0.9296007878251291
33.616787682496685 12.96471898702334 0.9334653754705076
33.616787682496685 16.451722811563343 0.9391819899654814
33.616787682496685 20.87659468280201 0.948129773323661
33.616787682496685 26.491584531418546 0.9633705304895044
33.616787682496685 33.616787682496685 0.9933484203916414
33.616787682496685 42.65839262086404 1.073664385780873
33.616787682496685 54.13183669370275 1.8706005917415185
33.616787682496685 68.69118979416318 0.6152011512868789
33.616787682496685 87.16644110999944 0.7769545249027249
33.616787682496685 110.6108145535225 0.8241007159099458
33.616787682496685 140.3608101970589 0.8431769610341302
33.616787682496685 178.11239451312218 0.8425185200997655
33.616787682496685 226.01768281801222 0.8310602140977582
33.616787682496685 286.807625522434 0.8205648057468552
33.616787682496685 363.94769219915764 0.8118450209228472
33.616787682496685 461.8354285936932 0.8020020792560127
33.616787682496685 586.0511487667402 0.7897861395424485
33.616787682496685 743.6760536467558 0.7752542083642622
33.616787682496685 943.6959110675486 0.7590573299237134
33.616787682496685 1197.5133099937427 0.7420813664435001
33.616787682496685 1519.5976911565988 0.7252453807138209
33.616787682496685 1928.3102105817359 0.7093773923622826
33.616787682496685 2446.9504592387466 0.6951526144344072
33.616787682496685 3105.0847094578075 0.6831019484109323
33.616787682496685 3940.2314078349555 0.6737366453165924
33.616787682496685 5000.0 0.6680044335134445

42.65839262086404 5.0 0.9236447113905814
42.65839262086404 6.344805015839611 0.924756465597069
42.65839262086404 8.051310137804697 0.9264125573171872
42.65839262086404 10.216798589284712 0.9287751497836846
42.65839262086404 12.96471898702334 0.932134889437713
42.65839262086404 16.451722811563343 0.9370123415326059
42.65839262086404 20.87659468280201 0.9443826683800762
42.65839262086404 26.491584531418546 0.956249739078474
42.65839262086404 33.616787682496685 0.9774500863886543
42.65839262086404 42.65839262086404 1.0235837210751397
42.65839262086404 54.13183669370275 1.19178547413394
42.65839262086404 68.69118979416318 0.011555206482187514
42.65839262086404 87.16644110999944 0.7244130473311369
42.65839262086404 110.6108145535225 0.8065840900333895
42.65839262086404 140.3608101970589 0.8344957052410366
42.65839262086404 178.11239451312218 0.8365337681945411
42.65839262086404 226.01768281801222 0.8263542864469027
42.65839262086404 286.807625522434 0.8168314156417459
42.65839262086404 363.94769219915764 0.8087749649180253
42.65839262086404 461.8354285936932 0.7993936492901704
42.65839262086404 586.0511487667402 0.7875350711490307
42.65839262086404 743.6760536467558 0.7733081485910402
42.65839262086404 943.6959110675486 0.7573875029259106
42.65839262086404 1197.5133099937427 0.7406663999706495
42.65839262086404 1519.5976911565988 0.7240634312286042
42.65839262086404 1928.3102105817359 0.7084036144661051
42.65839262086404 2446.9504592387466 0.6943595042399958
42.65839262086404 3105.0847094578075 0.6824608835231762
42.65839262086404 3940.2314078349555 0.6732196382235052
42.65839262086404 5000.0 0.6675859796618752

54.13183669370275 5.0 0.9246656484621928
54.13183669370275 6.344805015839611 0.9253461477035639
54.13183669370275 8.051310137804697 0.9266197112957034
54.13183669370275 10.216798589284712 0.9286027208299851
54.13183669370275 12.96471898702334 0.9315133866550274
54.13183669370275 16.451722811563343 0.9357443283552189
54.13183669370275 20.87659468280201 0.9420131867299046
54.13183669370275 26.491584531418546 0.9517173583885582
54.13183669370275 33.616787682496685 0.9679266839356871
54.13183669370275 42.65839262086404 0.9989846225596912
54.13183669370275 54.13183669370275 1.0792040496562003
54.13183669370275 68.69118979416318 1.7662303506516672
54.13183669370275 87.16644110999944 0.6017498877555348
54.13183669370275 110.6108145535225 0.7789598500099258
54.13183669370275 140.3608101970589 0.82245393426587
54.13183669370275 178.11239451312218 0.8286377862833314
54.13183669370275 226.01768281801222 0.82029032095638
54.13183669370275 286.807625522434 0.8120781042413544
54.13183669370275 363.94769219915764 0.8048905173833112
54.13183669370275 461.8354285936932 0.7961032032521942
54.13183669370275 586.0511487667402 0.7846988335726401
54.13183669370275 743.6760536467558 0.7708569709664197
54.13183669370275 943.6959110675486 0.7552839624227982
54.13183669370275 1197.5133099937427 0.7388832135698561
54.13183669370275 1519.5976911565988 0.7225731042694278
54.13183669370275 1928.3102105817359 0.7071750282781539
54.13183669370275 2446.9504592387466 0.6933582336380395
54.13183669370275 3105.0847094578075 0.6816510689250479
54.13183669370275 3940.2314078349555 0.6725661684364751
54.13183669370275 5000.0 0.6670568206340427

68.69118979416318 5.0 0.9269927052673731
68.69118979416318 6.344805015839611 0.927054144202808
68.69118979416318 8.051310137804697 0.9277955884180158
68.69118979416318 10.216798589284712 0.9292985321538791
68.69118979416318 12.96471898702334 0.9317253628267295
68.69118979416318 16.451722811563343 0.9353744683067903
68.69118979416318 20.87659468280201 0.9407868402142927
68.69118979416318 26.491584531418546 0.9489798825737662
68.69118979416318 33.616787682496685 0.9620434778452378
68.69118979416318 42.65839262086404 0.9850201408545853
68.69118979416318 54.13183669370275 1.0342371347295427
68.69118979416318 68.69118979416318 1.213282916560714
68.69118979416318 87.16644110999944 0.03754034633361074
68.69118979416318 110.6108145535225 0.7308412331354025
68.69118979416318 140.3608101970589 0.8052418329202234
68.69118979416318 178.11239451312218 0.8181024336233449
68.69118979416318 226.01768281801222 0.8124460247354247
68.69118979416318 286.807625522434 0.8060236256881704
68.69118979416318 363.94769219915764 0.799981126029726
68.69118979416318 461.8354285936932 0.7919596401488319
68.69118979416318 586.0511487667402 0.7811323333047738
68.69118979416318 743.6760536467558 0.7677757453764125
68.69118979416318 943.6959110675486 0.7526391994028917
68.69118979416318 1197.5133099937427 0.736640096771494
68.69118979416318 1519.5976911565988 0.720697111443661
68.69118979416318 1928.3102105817359 0.7056273265852188
68.69118979416318 2446.9504592387466 0.6920958925389982
68.69118979416318 3105.0847094578075 0.6806293139642252
68.69118979416318 3940.2314078349555 0.671741083734921
68.69118979416318 5000.0 0.6663882834664235

87.16644110999944 5.0 0.93113511498487
87.16644110999944 6.344805015839611 0.9303533814637185
87.16644110999944 8.051310137804697 0.9303569822658846
87.16644110999944 10.216798589284712 0.9312088965087166
87.16644110999944 12.96471898702334 0.933032487789757
87.16644110999944 16.451722811563343 0.9360563178648511
87.16644110999944 20.87659468280201 0.9406941398258132
87.16644110999944 26.491584531418546 0.9477075777174746
87.16644110999944 33.616787682496685 0.958588646208247
87.16644110999944 42.65839262086404 0.9766409004900248
87.16644110999944 54.13183669370275 1.0109875188019386
87.16644110999944 68.69118979416318 1.100721253112918
87.16644110999944 87.16644110999944 2.0877142220332052
87.16644110999944 110.6108145535225 0.6302810952487807
87.16644110999944 140.3608101970589 0.7795373693191142
87.16644110999944 178.11239451312218 0.803832906642607
87.16644110999944 226.01768281801222 0.8022501473302104
87.16644110999944 286.807625522434 0.7983096407115496
87.16644110999944 363.94769219915764 0.7937861899318069
87.16644110999944 461.8354285936932 0.7867537182755756
87.16644110999944 586.0511487667402 0.7766588120558766
87.16644110999944 743.6760536467558 0.7639123409799539
87.16644110999944 943.6959110675486 0.7493221148908441
87.16644110999944 1197.5133099937427 0.7338249285160773
87.16644110999944 1519.5976911565988 0.7183406687304076
87.16644110999944 1928.3102105817359 0.7036813728163426
87.16644110999944 2446.9504592387466 0.6905071425823217
87.16644110999944 3105.0847094578075 0.6793421055032998
87.16644110999944 3940.2314078349555 0.6707006982000892
87.16644110999944 5000.0 0.6655446490414643

110.6108145535225 5.0 0.9375819621501442
110.6108145535225 6.344805015839611 0.9357573220609056
110.6108145535225 8.051310137804697 0.9348015422381643
110.6108145535225 10.216798589284712 0.934784708565103
110.6108145535225 12.96471898702334 0.9358143115182356
110.6108145535225 16.451722811563343 0.9380737986480578
110.6108145535225 20.87659468280201 0.9418860369247944
110.6108145535225 26.491584531418546 0.9478325796737094
110.6108145535225 33.616787682496685 0.9570126422081963
110.6108145535225 42.65839262086404 0.9717093232725466
110.6108145535225 54.13183669370275 0.9975474075560848
110.6108145535225 68.69118979416318 1.0536029600365147
110.6108145535225 87.16644110999944 1.2803024142579889
110.6108145535225 110.6108145535225 0.30579285900577974
110.6108145535225 140.3608101970589 0.7384547146339574
110.6108145535225 178.11239451312218 0.784106553251032
110.6108145535225 226.01768281801222 0.7889208731743595
110.6108145535225 286.807625522434 0.7884821116754546
110.6108145535225 363.94769219915764 0.7859868251223501
110.6108145535225 461.8354285936932 0.7802327438867155
110.6108145535225 586.0511487667402 0.77106567278916
110.6108145535225 743.6760536467558 0.7590837477245035
110.6108145535225 943.6959110675486 0.745174646739792
110.6108145535225 1197.5133099937427 0.7303020760627907
110.6108145535225 1519.5976911565988 0.7153886434793564
110.6108145535225 1928.3102105817359 0.7012406114088177
110.6108145535225 2446.9504592387466 0.6885119039246406
110.6108145535225 3105.0847094578075 0.6777235717756176
110.6108145535225 3940.2314078349555 0.6693910260296331
110.6108145535225 5000.0 0.6644816214978705

140.3608101970589 5.0 0.9465935246645801
140.3608101970589 6.344805015839611 0.9436457276807045
140.3608101970589 8.051310137804697 0.9415707904535318
140.3608101970589 10.216798589284712 0.940477570609854
140.3608101970589 12.96471898702334 0.9404889116450811
140.3608101970589 16.451722811563343 0.9417739024904328
140.3608101970589 20.87659468280201 0.944599757188582
140.3608101970589 26.491584531418546 0.9494230119242103
140.3608101970589 33.616787682496685 0.9570725902552878
140.3608101970589 42.65839262086404 0.9691807405956004
140.3608101970589 54.13183669370275 0.9894295406299762
140.3608101970589 68.69118979416318 1.0284469653883646
140.3608101970589 87.16644110999944 1.1376770712647932
140.3608101970589 110.6108145535225 7.338353557731288
140.3608101970589 140.3608101970589 0.6648114676197002
140.3608101970589 178.11239451312218 0.7560502646328622
140.3608101970589 226.01768281801222 0.771376092605647
140.3608101970589 286.807625522434 0.7759717277258014
140.3608101970589 363.94769219915764 0.7761993920960878
140.3608101970589 461.8354285936932 0.7720969313278552
140.3608101970589 586.0511487667402 0.7641014961855677
140.3608101970589 743.6760536467558 0.7530733200760558
140.3608101970589 943.6959110675486 0.740009074891614
140.3608101970589 1197.5133099937427 0.725909695300922
140.3608101970589 1519.5976911565988 0.7117029020810136
140.3608101970589 1928.3102105817359 0.6981885271562039
140.3608101970589 2446.9504592387466 0.6860129793085818
140.3608101970589 3105.0847094578075 0.6756933123771917
140.3608101970589 3940.2314078349555 0.6677458380025098
140.3608101970589 5000.0 0.6631446372023893

178.11239451312218 5.0 0.9579121595673894
178.11239451312218 6.344805015839611 0.9539713547871275
178.11239451312218 8.051310137804697 0.9507774243071188
178.11239451312218 10.216798589284712 0.9485004437636526
178.11239451312218 12.96471898702334 0.9473093499586677
178.11239451312218 16.451722811563343 0.947393985340408
178.11239451312218 20.87659468280201 0.9490048212629094
178.11239451312218 26.491584531418546 0.95252281578323
178.11239451312218 33.616787682496685 0.9585916659228676
178.11239451312218 42.65839262086404 0.9684033768241317
178.11239451312218 54.13183669370275 0.9844413002150153
178.11239451312218 68.69118979416318 1.0130233064317522
178.11239451312218 87.16644110999944 1.0780963193020345
178.11239451312218 110.6108145535225 1.4452276652747063
178.11239451312218 140.3608101970589 0.4996003775563117
178.11239451312218 178.11239451312218 0.7145053393584032
178.11239451312218 226.01768281801222 0.7481068489198405
178.11239451312218 286.807625522434 0.7600780233416211
178.11239451312218 363.94769219915764 0.7639739508961545
178.11239451312218 461.8354285936932 0.7619993936887808
178.11239451312218 586.0511487667402 0.7554758613863333
178.11239451312218 743.6760536467558 0.7456300914747366
178.11239451312218 943.6959110675486 0.7336068247508827
178.11239451312218 1197.5133099937427 0.7204581273773321
178.11239451312218 1519.5976911565988 0.7071203828756744
178.11239451312218 1928.3102105817359 0.6943865127533129
178.11239451312218 2446.9504592387466 0.6828938559269434
178.11239451312218 3105.0847094578075 0.6731542532414173
178.11239451312218 3940.2314078349555 0.6656846420754344
178.11239451312218 5000.0 0.6614670201202135

226.01768281801222 5.0 0.9704774307172934
226.01768281801222 6.344805015839611 0.965901403976554
226.01768281801222 8.051310137804697 0.9618133011497741
226.01768281801222 10.216798589284712 0.9584371197742114
226.01768281801222 12.96471898702334 0.9559988487883628
226.01768281801222 16.451722811563343 0.9547344786953085
226.01768281801222 20.87659468280201 0.9549138411037403
226.01768281801222 26.491584531418546 0.9568889211944319
226.01768281801222 33.616787682496685 0.9611857442580637
226.01768281801222 42.65839262086404 0.9686894877760132
226.01768281801222 54.13183669370275 0.9810757344967463
226.01768281801222 68.69118979416318 1.0021178141075862
226.01768281801222 87.16644110999944 1.0439433952662738
226.01768281801222 110.6108145535225 1.1918015503456754
226.01768281801222 140.3608101970589 0.186680902384722
226.01768281801222 178.11239451312218 0.6493212760459309
226.01768281801222 226.01768281801222 0.7170123573829138
226.01768281801222 286.807625522434 0.7399676762263113
226.01768281801222 363.94769219915764 0.7488027916553084
226.01768281801222 461.8354285936932 0.7495529141159153
226.01768281801222 586.0511487667402 0.7448640102568002
226.01768281801222 743.6760536467558 0.7364717757698234
226.01768281801222 943.6959110675486 0.7257201196655204
226.01768281801222 1197.5133099937427 0.7137303911900699
226.01768281801222 1519.5976911565988 0.7014526665949148
226.01768281801222 1928.3102105817359 0.6896727556461756
226.01768281801222 2446.9504592387466 0.6790171332268575
226.01768281801222 3105.0847094578075 0.6699908191894104
226.01768281801222 3940.2314078349555 0.6631107827609128
226.01768281801222 5000.0 0.6593681491804746

286.807625522434 5.0 0.9823058473539152
286.807625522434 6.344805015839611 0.9775804408901151
286.807625522434 8.051310137804697 0.9730151568869339
286.807625522434 10.216798589284712 0.9688456097459918
286.807625522434 12.96471898702334 0.9653301172534295
286.807625522434 16.451722811563343 0.9627462097323153
286.807625522434 20.87659468280201 0.9613975948213211
286.807625522434 26.491584531418546 0.9616388578542742
286.807625522434 33.616787682496685 0.9639291065714661
286.807625522434 42.65839262086404 0.9689366321543368
286.807625522434 54.13183669370275 0.977752304298611
286.807625522434 68.69118979416318 0.9924525597731491
286.807625522434 87.16644110999944 1.0189720070404047
286.807625522434 110.6108145535225 1.097090137767734
286.807625522434 140.3608101970589 2.9467101858446894
286.807625522434 178.11239451312218 0.538065735795068
286.807625522434 226.01768281801222 0.6752250386385192
286.807625522434 286.807625522434 0.7147054363474573
286.807625522434 363.94769219915764 0.730146592632384
286.807625522434 461.8354285936932 0.7343476222418823
286.807625522434 586.0511487667402 0.7319192962804021
286.807625522434 743.6760536467558 0.7252937483814009
286.807625522434 943.6959110675486 0.7160782575893944
286.807625522434 1197.5133099937427 0.7054862439398834
286.807625522434 1519.5976911565988 0.6944881964750256
286.807625522434 1928.3102105817359 0.6838630010124348
286.807625522434 2446.9504592387466 0.674224221647631
286.807625522434 3105.0847094578075 0.6660679231812967
286.807625522434 3940.2314078349555 0.6599100179605477
286.807625522434 5000.0 0.6567518648670545

363.94769219915764 5.0 0.9906665207682684
363.94769219915764 6.344805015839611 0.9862313813460868
363.94769219915764 8.051310137804697 0.9816558730088858
363.94769219915764 10.216798589284712 0.9771329003836488
363.94769219915764 12.96471898702334 0.9729008009456683
363.94769219915764 16.451722811563343 0.9692378141116154
363.94769219915764 20.87659468280201 0.9664587733225501
363.94769219915764 26.491584531418546 0.9649196473673529
363.94769219915764 33.616787682496685 0.9650358774097498
363.94769219915764 42.65839262086404 0.9673177732619057
363.94769219915764 54.13183669370275 0.9724125296389515
363.94769219915764 68.69118979416318 0.9811457315299364
363.94769219915764 87.16644110999944 0.9958554617585772
363.94769219915764 110.6108145535225 1.0433065420793586
363.94769219915764 140.3608101970589 1.4872517847941122
363.94769219915764 178.11239451312218 0.3222652359532013
363.94769219915764 226.01768281801222 0.6190290099711375
363.94769219915764 286.807625522434 0.6833461792663466
363.94769219915764 363.94769219915764 0.7074866990634191
363.94769219915764 461.8354285936932 0.715984062054379
363.94769219915764 586.0511487667402 0.716296703586482
363.94769219915764 743.6760536467558 0.7117865632125694
363.94769219915764 943.6959110675486 0.7044006857459258
363.94769219915764 1197.5133099937427 0.6954716131358217
363.94769219915764 1519.5976911565988 0.6859986554097554
363.94769219915764 1928.3102105817359 0.6767544294149693
363.94769219915764 2446.9504592387466 0.6683372586617097
363.94769219915764 3105.0847094578075 0.6612314533739668
363.94769219915764 3940.2314078349555 0.6559500499183463
363.94769219915764 5000.0 0.6535055094205173

461.8354285936932 5.0 0.9923025763039116
461.8354285936932 6.344805015839611 0.9884148422152349
461.8354285936932 8.051310137804697 0.9841805430942705
461.8354285936932 10.216798589284712 0.9797164705265677
461.8354285936932 12.96471898702334 0.9751937645558508
461.8354285936932 16.451722811563343 0.9708387169326597
461.8354285936932 20.87659468280201 0.9669300904454938
461.8354285936932 26.491584531418546 0.9637946432324636
461.8354285936932 33.616787682496685 0.9617997080905296
461.8354285936932 42.65839262086404 0.9613251706535915
461.8354285936932 54.13183669370275 0.9626279377012885
461.8354285936932 68.69118979416318 0.9653982470280742
461.8354285936932 87.16644110999944 0.9705610517954899
461.8354285936932 110.6108145535225 1.0092054023402555
461.8354285936932 140.3608101970589 1.2798443252268015
461.8354285936932 178.11239451312218 0.20190645654341277
461.8354285936932 226.01768281801222 0.5441232385519719
461.8354285936932 286.807625522434 0.6451188690321764
461.8354285936932 363.94769219915764 0.680409340451383
461.8354285936932 461.8354285936932 0.6941246529913755
461.8354285936932 586.0511487667402 0.6976899471562048
461.8354285936932 743.6760536467558 0.6956644769583592
461.8354285936932 943.6959110675486 0.6904191342666255
461.8354285936932 1197.5133099937427 0.6834354300555952
461.8354285936932 1519.5976911565988 0.6757512769089531
461.8354285936932 1928.3102105817359 0.668134134694691
461.8354285936932 2446.9504592387466 0.6611644859388657
461.8354285936932 3105.0847094578075 0.6553112626064417
461.8354285936932 3940.2314078349555 0.6510818217834011
461.8354285936932 5000.0 0.6495001833742551

586.0511487667402 5.0 0.9837947655377968
586.0511487667402 6.344805015839611 0.9805493504651174
586.0511487667402 8.051310137804697 0.9768658620120895
586.0511487667402 10.216798589284712 0.9727881290905911
586.0511487667402 12.96471898702334 0.9684076093151877
586.0511487667402 16.451722811563343 0.9638712721134669
586.0511487667402 20.87659468280201 0.9593840429497255
586.0511487667402 26.491584531418546 0.9551999809537058
586.0511487667402 33.616787682496685 0.9515836725147742
586.0511487667402 42.65839262086404 0.9486722520776328
586.0511487667402 54.13183669370275 0.9460150692853795
586.0511487667402 68.69118979416318 0.9420938989248416
586.0511487667402 87.16644110999944 0.9446491537338149
586.0511487667402 110.6108145535225 0.9943162451013772
586.0511487667402 140.3608101970589 1.2126101854469709
586.0511487667402 178.11239451312218 2.4909814962312633
586.0511487667402 226.01768281801222 0.44669468888811165
586.0511487667402 286.807625522434 0.5997127254087526
586.0511487667402 363.94769219915764 0.648717338624901
586.0511487667402 461.8354285936932 0.6685616835381808
586.0511487667402 586.0511487667402 0.6758822160027874
586.0511487667402 743.6760536467558 0.6767059554078106
586.0511487667402 943.6959110675486 0.6739102592307679
586.0511487667402 1197.5133099937427 0.6691555420022987
586.0511487667402 1519.5976911565988 0.6635287713806868
586.0511487667402 1928.3102105817359 0.6577938204977022
586.0511487667402 2446.9504592387466 0.652510502696219
586.0511487667402 3105.0847094578075 0.6481278632048727
586.0511487667402 3940.2314078349555 0.64514354784308
586.0511487667402 5000.0 0.6445930567179313

743.6760536467558 5.0 0.9641352190654497
743.6760536467558 6.344805015839611 0.9615688968382203
743.6760536467558 8.051310137804697 0.958569613791544
743.6760536467558 10.216798589284712 0.955128919994861
743.6760536467558 12.96471898702334 0.9512664580671907
743.6760536467558 16.451722811563343 0.947034017530811
743.6760536467558 20.87659468280201 0.9425057070994397
743.6760536467558 26.491584531418546 0.9377277188389926
743.6760536467558 33.616787682496685 0.932552236657805
743.6760536467558 42.65839262086404 0.9262045434076926
743.6760536467558 54.13183669370275 0.9175407855524914
743.6760536467558 68.69118979416318 0.9139702661596096
743.6760536467558 87.16644110999944 0.9344556475111447
743.6760536467558 110.6108145535225 0.9964992867823232
743.6760536467558 140.3608101970589 1.189273731522242
743.6760536467558 178.11239451312218 9.08753576437309
743.6760536467558 226.01768281801222 0.32590256627082975
743.6760536467558 286.807625522434 0.5476123405721776
743.6760536467558 363.94769219915764 0.6125456519235493
743.6760536467558 461.8354285936932 0.6392914771794889
743.6760536467558 586.0511487667402 0.6508056994910434
743.6760536467558 743.6760536467558 0.6548040228877217
743.6760536467558 943.6959110675486 0.6547382476321806
743.6760536467558 1197.5133099937427 0.6524740693993882
743.6760536467558 1519.5976911565988 0.649157845007673
743.6760536467558 1928.3102105817359 0.6455519535371936
743.6760536467558 2446.9504592387466 0.6421927603413092
743.6760536467558 3105.0847094578075 0.6395041302479607
743.6760536467558 3940.2314078349555 0.6379686531378258
743.6760536467558 5000.0 0.6386328250803086

943.6959110675486 5.0 0.9347591892513131
943.6959110675486 6.344805015839611 0.9326158387754123
943.6959110675486 8.051310137804697 0.930000806088939
943.6959110675486 10.216798589284712 0.9268168595455062
943.6959110675486 12.96471898702334 0.9229259899140707
943.6959110675486 16.451722811563343 0.918102107775369
943.6959110675486 20.87659468280201 0.9119596568925447
943.6959110675486 26.491584531418546 0.9047897246253713
943.6959110675486 33.616787682496685 0.8955743939382607
943.6959110675486 42.65839262086404 0.8912323863630526
943.6959110675486 54.13183669370275 0.8957181405141119
943.6959110675486 68.69118979416318 0.9106872468742545
943.6959110675486 87.16644110999944 0.9405252613580454
943.6959110675486 110.6108145535225 1.0032163197650728
943.6959110675486 140.3608101970589 1.183871711734895
943.6959110675486 178.11239451312218 3.6122876620967057
943.6959110675486 226.01768281801222 0.18778677926058615
943.6959110675486 286.807625522434 0.49032914775309167
943.6959110675486 363.94769219915764 0.572436716583751
943.6959110675486 461.8354285936932 0.6065749786846373
943.6959110675486 586.0511487667402 0.6225984886235986
943.6959110675486 743.6760536467558 0.6300194522460713
943.6959110675486 943.6959110675486 0.6329031786444549
943.6959110675486 1197.5133099937427 0.6333400182995207
943.6959110675486 1519.5976911565988 0.6325454843052769
943.6959110675486 1928.3102105817359 0.6312835402903144
943.6959110675486 2446.9504592387466 0.6300650246478128
943.6959110675486 3105.0847094578075 0.6292830659632104
943.6959110675486 3940.2314078349555 0.6293988381656345
943.6959110675486 5000.0 0.6314696338353457

1197.5133099937427 5.0 0.8845843069686291
1197.5133099937427 6.344805015839611 0.8834137230295428
1197.5133099937427 8.051310137804697 0.8822294736630605
1197.5133099937427 10.216798589284712 0.8811396789360623
1197.5133099937427 12.96471898702334 0.8802936519464348
1197.5133099937427 16.451722811563343 0.8798803348981605
1197.5133099937427 20.87659468280201 0.8801327557911296
1197.5133099937427 26.491584531418546 0.8813594482066595
1197.5133099937427 33.616787682496685 0.8840336108434855
1197.5133099937427 42.65839262086404 0.8889838233654218
1197.5133099937427 54.13183669370275 0.8977795750577906
1197.5133099937427 68.69118979416318 0.9135994055452059
1197.5133099937427 87.16644110999944 0.9436354217125005
1197.5133099937427 110.6108145535225 1.0079169741084932
1197.5133099937427 140.3608101970589 1.1911096162528467
1197.5133099937427 178.11239451312218 3.0270251887863977
1197.5133099937427 226.01768281801222 0.0480489906163217
1197.5133099937427 286.807625522434 0.43031156907809265
1197.5133099937427 363.94769219915764 0.5293284114779239
1197.5133099937427 461.8354285936932 0.5709614917095025
1197.5133099937427 586.0511487667402 0.5916426078039773
1197.5133099937427 743.6760536467558 0.6026246512395823
1197.5133099937427 943.6959110675486 0.6085863205431415
1197.5133099937427 1197.5133099937427 0.6118531151923424
1197.5133099937427 1519.5976911565988 0.6137192783660474
1197.5133099937427 1928.3102105817359 0.6149555533011569
1197.5133099937427 2446.9504592387466 0.6160471682120174
1197.5133099937427 3105.0847094578075 0.61735187354628
1197.5133099937427 3940.2314078349555 0.6193030731679072
1197.5133099937427 5000.0 0.622970844818518

1519.5976911565988 5.0 0.8708402023658297
1519.5976911565988 6.344805015839611 0.870668965147181
1519.5976911565988 8.051310137804697 0.8705160442891873
1519.5976911565988 10.216798589284712 0.870423361999681
1519.5976911565988 12.96471898702334 0.8704649748055736
1519.5976911565988 16.451722811563343 0.8707675456139858
1519.5976911565988 20.87659468280201 0.8715437601360534
1519.5976911565988 26.491584531418546 0.8731484121908564
1519.5976911565988 33.616787682496685 0.8761771685612308
1519.5976911565988 42.65839262086404 0.8816534341157355
1519.5976911565988 54.13183669370275 0.8914187265875597
1519.5976911565988 68.69118979416318 0.9090612164946793
1519.5976911565988 87.16644110999944 0.942545407550083
1519.5976911565988 110.6108145535225 1.013847509776784
1519.5976911565988 140.3608101970589 1.214860484922963
1519.5976911565988 178.11239451312218 3.105856471135414
1519.5976911565988 226.01768281801222 0.07210652761753893
1519.5976911565988 286.807625522434 0.3704117753364951
1519.5976911565988 363.94769219915764 0.48443773231450976
1519.5976911565988 461.8354285936932 0.5332608376666126
1519.5976911565988 586.0511487667402 0.558567572993734
1519.5976911565988 743.6760536467558 0.5731234203325061
1519.5976911565988 943.6959110675486 0.5821796184405479
1519.5976911565988 1197.5133099937427 0.5882987291313103
1519.5976911565988 1519.5976911565988 0.5928643538342058
1519.5976911565988 1928.3102105817359 0.5966630669432229
1519.5976911565988 2446.9504592387466 0.6001584112876455
1519.5976911565988 3105.0847094578075 0.6036711010605815
1519.5976911565988 3940.2314078349555 0.6076026167560504
1519.5976911565988 5000.0 0.6130441971728985

1928.3102105817359 5.0 0.8479559417887023
1928.3102105817359 6.344805015839611 0.8481808719061962
1928.3102105817359 8.051310137804697 0.8485201139139025
1928.3102105817359 10.216798589284712 0.8490366158697253
1928.3102105817359 12.96471898702334 0.8498296172302825
1928.3102105817359 16.451722811563343 0.8510564736942329
1928.3102105817359 20.87659468280201 0.8529687744169357
1928.3102105817359 26.491584531418546 0.8559740610671952
1928.3102105817359 33.616787682496685 0.8607464957250591
1928.3102105817359 42.65839262086404 0.8684394258938892
1928.3102105817359 54.13183669370275 0.8811339453672449
1928.3102105817359 68.69118979416318 0.9029126513937347
1928.3102105817359 87.16644110999944 0.9429174627622643
1928.3102105817359 110.6108145535225 1.0266512256603166
1928.3102105817359 140.3608101970589 1.2628152199378242
1928.3102105817359 178.11239451312218 3.7268120732320345
1928.3102105817359 226.01768281801222 0.15840661741590933
1928.3102105817359 286.807625522434 0.313073057481881
1928.3102105817359 363.94769219915764 0.4390717695790815
1928.3102105817359 461.8354285936932 0.49446588340119946
1928.3102105817359 586.0511487667402 0.5242111649567394
1928.3102105817359 743.6760536467558 0.5422341163069834
1928.3102105817359 943.6959110675486 0.5542858754289246
1928.3102105817359 1197.5133099937427 0.563161347536228
1928.3102105817359 1519.5976911565988 0.5703463856969622
1928.3102105817359 1928.3102105817359 0.5766580346294411
1928.3102105817359 2446.9504592387466 0.5825484657782676
1928.3102105817359 3105.0847094578075 0.5883056369432771
1928.3102105817359 3940.2314078349555 0.5943010116848756
1928.3102105817359 5000.0 0.6016703752941993

2446.9504592387466 5.0 0.8234195786513222
2446.9504592387466 6.344805015839611 0.8241103418497495
2446.9504592387466 8.051310137804697 0.8250328148335966
2446.9504592387466 10.216798589284712 0.8262780060945353
2446.9504592387466 12.96471898702334 0.8279797852216602
2446.9504592387466 16.451722811563343 0.8303389824557075
2446.9504592387466 20.87659468280201 0.8336635609153533
2446.9504592387466 26.491584531418546 0.8384382625521909
2446.9504592387466 33.616787682496685 0.8454516779495894
2446.9504592387466 42.65839262086404 0.8560443345110348
2446.9504592387466 54.13183669370275 0.872640009947659
2446.9504592387466 68.69118979416318 0.9000342628370768
2446.9504592387466 87.16644110999944 0.9491180001825221
2446.9504592387466 110.6108145535225 1.050948009055935
2446.9504592387466 140.3608101970589 1.343919500970759
2446.9504592387466 178.11239451312218 5.549869871036368
2446.9504592387466 226.01768281801222 0.21273314411909963
2446.9504592387466 286.807625522434 0.259630107564721
2446.9504592387466 363.94769219915764 0.39441634198962355
2446.9504592387466 461.8354285936932 0.4556364319087709
2446.9504592387466 586.0511487667402 0.4895378264689602
2446.9504592387466 743.6760536467558 0.5108307293624703
2446.9504592387466 943.6959110675486 0.5256803912082705
2446.9504592387466 1197.5133099937427 0.537105585047891
2446.9504592387466 1519.5976911565988 0.5467096891300376
2446.9504592387466 1928.3102105817359 0.5553610570883523
2446.9504592387466 2446.9504592387466 0.5635191109654712
2446.9504592387466 3105.0847094578075 0.5714527717967836
2446.9504592387466 3940.2314078349555 0.5795176472087904
2446.9504592387466 5000.0 0.5889500611604337

3105.0847094578075 5.0 0.8022483983680349
3105.0847094578075 6.344805015839611 0.8033796533873505
3105.0847094578075 8.051310137804697 0.8048591992821811
3105.0847094578075 10.216798589284712 0.8068090097364843
3105.0847094578075 12.96471898702334 0.8094028168274376
3105.0847094578075 16.451722811563343 0.8128936887903168
3105.0847094578075 20.87659468280201 0.8176602417036908
3105.0847094578075 26.491584531418546 0.8242872166712077
3105.0847094578075 33.616787682496685 0.8337142921491927
3105.0847094578075 42.65839262086404 0.8475307408212222
3105.0847094578075 54.13183669370275 0.8686155820088912
3105.0847094578075 68.69118979416318 0.9027157389004405
3105.0847094578075 87.16644110999944 0.963100090852337
3105.0847094578075 110.6108145535225 1.0887083916647973
3105.0847094578075 140.3608101970589 1.464438518617935
3105.0847094578075 178.11239451312218 13.529048232292157
3105.0847094578075 226.01768281801222 0.24959406885223268
3105.0847094578075 286.807625522434 0.20995865033620356
3105.0847094578075 363.94769219915764 0.3513134419867264
3105.0847094578075 461.8354285936932 0.4177456761158619
3105.0847094578075 586.0511487667402 0.4555179421822279
3105.0847094578075 743.6760536467558 0.47984420845694664
3105.0847094578075 943.6959110675486 0.4972331328247221
3105.0847094578075 1197.5133099937427 0.5109202988832267
3105.0847094578075 1519.5976911565988 0.5226435857759777
3105.0847094578075 1928.3102105817359 0.5333486260291274
3105.0847094578075 2446.9504592387466 0.5435296806767598
3105.0847094578075 3105.0847094578075 0.5534634946284529
3105.0847094578075 3940.2314078349555 0.5635264039125554
3105.0847094578075 5000.0 0.5751829231402161

3940.2314078349555 5.0 0.7859136482991425
3940.2314078349555 6.344805015839611 0.7874404010359147
3940.2314078349555 8.051310137804697 0.7894237850010065
3940.2314078349555 10.216798589284712 0.7920166465454149
3940.2314078349555 12.96471898702334 0.795433538625296
3940.2314078349555 16.451722811563343 0.7999826368026934
3940.2314078349555 20.87659468280201 0.8061191433411409
3940.2314078349555 26.491584531418546 0.8145389800247862
3940.2314078349555 33.616787682496685 0.8263530819038749
3940.2314078349555 42.65839262086404 0.8434356098404695
3940.2314078349555 54.13183669370275 0.8691905144835981
3940.2314078349555 68.69118979416318 0.9104692841334269
3940.2314078349555 87.16644110999944 0.9833426620563814
3940.2314078349555 110.6108145535225 1.1363524443566897
3940.2314078349555 140.3608101970589 1.616214039006356
3940.2314078349555 178.11239451312218 44.41806986990806
3940.2314078349555 226.01768281801222 0.2879697442138008
3940.2314078349555 286.807625522434 0.1622498356085955
3940.2314078349555 363.94769219915764 0.3099712824415937
3940.2314078349555 461.8354285936932 0.3814704548022551
3940.2314078349555 586.0511487667402 0.42296726010240504
3940.2314078349555 743.6760536467558 0.45013123207949884
3940.2314078349555 943.6959110675486 0.46979996336121677
3940.2314078349555 1197.5133099937427 0.48543204021865105
3940.2314078349555 1519.5976911565988 0.49891999640301204
3940.2314078349555 1928.3102105817359 0.5113165076669857
3940.2314078349555 2446.9504592387466 0.5231871057468218
3940.2314078349555 3105.0847094578075 0.5348613282076312
3940.2314078349555 3940.2314078349555 0.5468156806162285
3940.2314078349555 5000.0 0.5610439314324476

5000.0 5.0 0.7737862203673428
5000.0 6.344805015839611 0.7756363238966787
5000.0 8.051310137804697 0.778033200432384
5000.0 10.216798589284712 0.7811562594965682
5000.0 12.96471898702334 0.7852555842390304
5000.0 16.451722811563343 0.7906878639868786
5000.0 20.87659468280201 0.7979764718297838
5000.0 26.491584531418546 0.807917033477131
5000.0 33.616787682496685 0.8217742254553292
5000.0 42.65839262086404 0.8416775868060292
5000.0 54.13183669370275 0.8714974490564197
5000.0 68.69118979416318 0.9190558102847295
5000.0 87.16644110999944 1.0028566021837186
5000.0 110.6108145535225 1.1797104488925156
5000.0 140.3608101970589 1.7502692001743323
5000.0 178.11239451312218 14.528135110980399
5000.0 226.01768281801222 0.3509676757977323
5000.0 286.807625522434 0.11221546225663406
5000.0 363.94769219915764 0.26946427320562333
5000.0 461.8354285936932 0.346880553861806
5000.0 586.0511487667402 0.3923367826516743
5000.0 743.6760536467558 0.4223183485377907
5000.0 943.6959110675486 0.4440995076610512
5000.0 1197.5133099937427 0.4614072827927426
5000.0 1519.5976911565988 0.4763214712704917
5000.0 1928.3102105817359 0.4900380353526254
5000.0 2446.9504592387466 0.5032420616740035
5000.0 3105.0847094578075 0.5163920582857623
5000.0 3940.2314078349555 0.5302433627705582
5000.0 5000.0 0.5481308224388828


==> 5_Results/Figures/Mixture_P_Na_IOM.tex <==
x y z
5.0 5.0 3.781636036525894e-10
5.0 6.344805015839611 3.0303837920755776e-10
5.0 8.051310137804697 2.358697140755617e-10
5.0 10.216798589284712 1.7588574862678533e-10
5.0 12.96471898702334 1.2237545073224064e-10
5.0 16.451722811563343 7.467852699968047e-11
5.0 20.87659468280201 3.21669563616475e-11
5.0 26.491584531418546 -5.789347878998331e-12
5.0 33.616787682496685 -3.988694979808118e-11
5.0 42.65839262086404 -7.10083311644191e-11
5.0 54.13183669370275 -1.0043322291751607e-10
5.0 68.69118979416318 -1.3016271314533881e-10
5.0 87.16644110999944 -1.631553447213148e-10
5.0 110.6108145535225 -2.019358966392815e-10
5.0 140.3608101970589 -2.3923191699409657e-10
5.0 178.11239451312218 -2.39556691160627e-10
5.0 226.01768281801222 -1.739681499589384e-10
5.0 286.807625522434 -8.324695428614687e-11
5.0 363.94769219915764 -1.278740550872007e-11
5.0 461.8354285936932 3.060418120147963e-11
5.0 586.0511487667402 5.513875435558789e-11
5.0 743.6760536467558 6.856716215244917e-11
5.0 943.6959110675486 7.574464355985105e-11
5.0 1197.5133099937427 7.942502150332029e-11
5.0 1519.5976911565988 8.114449127755152e-11
5.0 1928.3102105817359 8.177857343225428e-11
5.0 2446.9504592387466 8.185769115657524e-11
5.0 3105.0847094578075 8.175091866810736e-11
5.0 3940.2314078349555 8.180350692555882e-11
5.0 5000.0 8.254552783011332e-11

6.344805015839611 5.0 4.1641048690094113e-10
6.344805015839611 6.344805015839611 3.4643024587313754e-10
6.344805015839611 8.051310137804697 2.837295775445678e-10
6.344805015839611 10.216798589284712 2.2763154096949508e-10
6.344805015839611 12.96471898702334 1.775075358175432e-10
6.344805015839611 16.451722811563343 1.3277113704198642e-10
6.344805015839611 20.87659468280201 9.286516982976347e-11
6.344805015839611 26.491584531418546 5.72364614742941e-11
6.344805015839611 33.616787682496685 2.528765288766439e-11
6.344805015839611 42.65839262086404 -3.7126224134754396e-12
6.344805015839611 54.13183669370275 -3.0788785986607333e-11
6.344805015839611 68.69118979416318 -5.750198050491919e-11
6.344805015839611 87.16644110999944 -8.612606192421156e-11
6.344805015839611 110.6108145535225 -1.1859182679085697e-10
6.344805015839611 140.3608101970589 -1.4941714866651975e-10
6.344805015839611 178.11239451312218 -1.5194133264676796e-10
6.344805015839611 226.01768281801222 -1.0474251948374172e-10
6.344805015839611 286.807625522434 -3.860396852868987e-11
6.344805015839611 363.94769219915764 1.2605196160458261e-11
6.344805015839611 461.8354285936932 4.385197344097781e-11
6.344805015839611 586.0511487667402 6.124066970366117e-11
6.344805015839611 743.6760536467558 7.051408222825897e-11
6.344805015839611 943.6959110675486 7.525822755516576e-11
6.344805015839611 1197.5133099937427 7.749878606525824e-11
6.344805015839611 1519.5976911565988 7.836073812208466e-11
6.344805015839611 1928.3102105817359 7.84840437775375e-11
6.344805015839611 2446.9504592387466 7.826006150624878e-11
6.344805015839611 3105.0847094578075 7.797171274166772e-11
6.344805015839611 3940.2314078349555 7.790543894986687e-11
6.344805015839611 5000.0 7.853915969412452e-11

8.051310137804697 5.0 4.410682097030145e-10
8.051310137804697 6.344805015839611 3.7537803942410983e-10
8.051310137804697 8.051310137804697 3.163647329746841e-10
8.051310137804697 10.216798589284712 2.634415195659323e-10
8.051310137804697 12.96471898702334 2.1605707970464593e-10
8.051310137804697 16.451722811563343 1.736928241564376e-10
8.051310137804697 20.87659468280201 1.3585450145566175e-10
8.051310137804697 26.491584531418546 1.0205396194629969e-10
8.051310137804697 33.616787682496685 7.177304726889244e-11
8.051310137804697 42.65839262086404 4.439542753553163e-11
8.051310137804697 54.13183669370275 1.9085469971489134e-11
8.051310137804697 68.69118979416318 -5.397284984234723e-12
8.051310137804697 87.16644110999944 -3.083064849923766e-11
8.051310137804697 110.6108145535225 -5.871514212773096e-11
8.051310137804697 140.3608101970589 -8.485443866663375e-11
8.051310137804697 178.11239451312218 -8.893933362461615e-11
8.051310137804697 226.01768281801222 -5.496236816463828e-11
8.051310137804697 286.807625522434 -6.507683294637414e-12
8.051310137804697 363.94769219915764 3.085355811802933e-11
8.051310137804697 461.8354285936932 5.3364965440074846e-11
8.051310137804697 586.0511487667402 6.561484014319181e-11
8.051310137804697 743.6760536467558 7.190103845767023e-11
8.051310137804697 943.6959110675486 7.489635656038453e-11
8.051310137804697 1197.5133099937427 7.610261609431354e-11
8.051310137804697 1519.5976911565988 7.634897778833537e-11
8.051310137804697 1928.3102105817359 7.610595724598893e-11
8.051310137804697 2446.9504592387466 7.566488600226986e-11
8.051310137804697 3105.0847094578075 7.5246718542711e-11
8.051310137804697 3940.2314078349555 7.50955994385871e-11
8.051310137804697 5000.0 7.565195000965472e-11

10.216798589284712 5.0 4.557867370288208e-10
10.216798589284712 6.344805015839611 3.939431129084338e-10
10.216798589284712 8.051310137804697 3.3820003373044493e-10
10.216798589284712 10.216798589284712 2.8806138049811057e-10
10.216798589284712 12.96471898702334 2.4305290952281656e-10
10.216798589284712 16.451722811563343 2.0272264024934615e-10
10.216798589284712 20.87659468280201 1.6663632643515435e-10
10.216798589284712 26.491584531418546 1.3436485330568865e-10
10.216798589284712 33.616787682496685 1.054574300197221e-10
10.216798589284712 42.65839262086404 7.938972355777653e-11
10.216798589284712 54.13183669370275 5.547093561940409e-11
10.216798589284712 68.69118979416318 3.270131691203446e-11
10.216798589284712 87.16644110999944 9.671869409359085e-12
10.216798589284712 110.6108145535225 -1.4798072800238505e-11
10.216798589284712 140.3608101970589 -3.7454769413268065e-11
10.216798589284712 178.11239451312218 -4.2660642311622777e-11
10.216798589284712 226.01768281801222 -1.8393825465212666e-11
10.216798589284712 286.807625522434 1.7062286791527282e-11
10.216798589284712 363.94769219915764 4.424472087819335e-11
10.216798589284712 461.8354285936932 6.033661476384933e-11
10.216798589284712 586.0511487667402 6.881123558076387e-11
10.216798589284712 743.6760536467558 7.290381531533084e-11
10.216798589284712 943.6959110675486 7.461565544200885e-11
10.216798589284712 1197.5133099937427 7.506344130784669e-11
10.216798589284712 1519.5976911565988 7.485888279245017e-11
10.216798589284712 1928.3102105817359 7.434795646680625e-11
10.216798589284712 2446.9504592387466 7.374848256781084e-11
10.216798589284712 3105.0847094578075 7.323587697634246e-11
10.216798589284712 3940.2314078349555 7.30232045068831e-11
10.216798589284712 5000.0 7.352334575088268e-11

12.96471898702334 5.0 4.6271624935595586e-10
12.96471898702334 6.344805015839611 4.0455570791191925e-10
12.96471898702334 8.051310137804697 3.519136757520203e-10
12.96471898702334 10.216798589284712 3.0438821649834093e-10
12.96471898702334 12.96471898702334 2.615850390325832e-10
12.96471898702334 16.451722811563343 2.231206685825019e-10
12.96471898702334 20.87659468280201 1.8862126917074274e-10
12.96471898702334 26.491584531418546 1.577146945227343e-10
12.96471898702334 33.616787682496685 1.3001104435740893e-10
12.96471898702334 42.65839262086404 1.0506335045036317e-10
12.96471898702334 54.13183669370275 8.229606989373522e-11
12.96471898702334 68.69118979416318 6.08950607133153e-11
12.96471898702334 87.16644110999944 3.973163878361467e-11
12.96471898702334 110.6108145535225 1.7868215823616756e-11
12.96471898702334 140.3608101970589 -2.1420076919535174e-12
12.96471898702334 178.11239451312218 -8.152474196938155e-12
12.96471898702334 226.01768281801222 8.87634616942945e-12
12.96471898702334 286.807625522434 3.462915301548124e-11
12.96471898702334 363.94769219915764 5.421340865182648e-11
12.96471898702334 461.8354285936932 6.551499862635857e-11
12.96471898702334 586.0511487667402 7.117397465340101e-11
12.96471898702334 743.6760536467558 7.363169401593217e-11
12.96471898702334 943.6959110675486 7.438791127614348e-11
12.96471898702334 1197.5133099937427 7.427172245321724e-11
12.96471898702334 1519.5976911565988 7.373250282847325e-11
12.96471898702334 1928.3102105817359 7.302327652763515e-11
12.96471898702334 2446.9504592387466 7.230700503298401e-11
12.96471898702334 3105.0847094578075 7.172512380360535e-11
12.96471898702334 3940.2314078349555 7.146750907002664e-11
12.96471898702334 5000.0 7.192651109321435e-11

16.451722811563343 5.0 4.631350645223954e-10
16.451722811563343 6.344805015839611 4.0869556082056603e-10
16.451722811563343 8.051310137804697 3.591655068738098e-10
16.451722811563343 10.216798589284712 3.1424187687953496e-10
16.451722811563343 12.96471898702334 2.7361478646756855e-10
16.451722811563343 16.451722811563343 2.3697301732566715e-10
16.451722811563343 20.87659468280201 2.040056976849605e-10
16.451722811563343 26.491584531418546 1.7439822953275417e-10
16.451722811563343 33.616787682496685 1.478187756840577e-10
16.451722811563343 42.65839262086404 1.238887895887795e-10
16.451722811563343 54.13183669370275 1.021280345747309e-10
16.451722811563343 68.69118979416318 8.186940942017592e-11
16.451722811563343 87.16644110999944 6.22017081526248e-11
16.451722811563343 110.6108145535225 4.2375957645932285e-11
16.451722811563343 140.3608101970589 2.4420432306881318e-11
16.451722811563343 178.11239451312218 1.7842414454725517e-11
16.451722811563343 226.01768281801222 2.942179680327775e-11
16.451722811563343 286.807625522434 4.7851729848704005e-11
16.451722811563343 363.94769219915764 6.170208556873033e-11
16.451722811563343 461.8354285936932 6.939079465746258e-11
16.451722811563343 586.0511487667402 7.29280405590149e-11
16.451722811563343 743.6760536467558 7.415527383846726e-11
16.451722811563343 943.6959110675486 7.419339324312965e-11
16.451722811563343 1197.5133099937427 7.365434755373761e-11
16.451722811563343 1519.5976911565988 7.286499041625858e-11
16.451722811563343 1928.3102105817359 7.200821511266341e-11
16.451722811563343 2446.9504592387466 7.120560311380973e-11
16.451722811563343 3105.0847094578075 7.057296254476448e-11
16.451722811563343 3940.2314078349555 7.028268546973592e-11
16.451722811563343 5000.0 7.07116639614264e-11

20.87659468280201 5.0 4.5779628033000855e-10
20.87659468280201 6.344805015839611 4.072621454924799e-10
20.87659468280201 8.051310137804697 3.609893873291403e-10
20.87659468280201 10.216798589284712 3.1877788816498064e-10
20.87659468280201 12.96471898702334 2.80406672135859e-10
20.87659468280201 16.451722811563343 2.4564115051486347e-10
20.87659468280201 20.87659468280201 2.1423707168372374e-10
20.87659468280201 26.491584531418546 1.859396001789997e-10
20.87659468280201 33.616787682496685 1.6047458351675387e-10
20.87659468280201 42.65839262086404 1.3752687793914599e-10
20.87659468280201 54.13183669370275 1.1669826900718812e-10
20.87659468280201 68.69118979416318 9.744153996561671e-11
20.87659468280201 87.16644110999944 7.901778813331e-11
20.87659468280201 110.6108145535225 6.08275788642713e-11
20.87659468280201 140.3608101970589 4.4504711901531005e-11
20.87659468280201 178.11239451312218 3.754414452256143e-11
20.87659468280201 226.01768281801222 4.4996758290078284e-11
20.87659468280201 286.807625522434 5.7859904971375406e-11
20.87659468280201 363.94769219915764 6.735179826596826e-11
20.87659468280201 461.8354285936932 7.229687517136482e-11
20.87659468280201 586.0511487667402 7.422518185622032e-11
20.87659468280201 743.6760536467558 7.452114979075578e-11
20.87659468280201 943.6959110675486 7.401724242316559e-11
20.87659468280201 1197.5133099937427 7.316019936967588e-11
20.87659468280201 1519.5976911565988 7.218372110934463e-11
20.87659468280201 1928.3102105817359 7.12174113506658e-11
20.87659468280201 2446.9504592387466 7.035142068307581e-11
20.87659468280201 3105.0847094578075 6.968209684121807e-11
20.87659468280201 3940.2314078349555 6.936856042042004e-11
20.87659468280201 5000.0 6.977599712067888e-11

26.491584531418546 5.0 4.4714434454139467e-10
26.491584531418546 6.344805015839611 4.007989201088016e-10
26.491584531418546 8.051310137804697 3.5802554197804076e-10
26.491584531418546 10.216798589284712 3.187281085134264e-10
26.491584531418546 12.96471898702334 2.8277735820718705e-10
26.491584531418546 16.451722811563343 2.500189310033751e-10
26.491584531418546 20.87659468280201 2.202788154124031e-10
26.491584531418546 26.491584531418546 1.9336479047865716e-10
26.491584531418546 33.616787682496685 1.690614371162184e-10
26.491584531418546 42.65839262086404 1.4711461119592792e-10
26.491584531418546 54.13183669370275 1.271994827218713e-10
26.491584531418546 68.69118979416318 1.0886961077327462e-10
26.491584531418546 87.16644110999944 9.15257042962283e-11
26.491584531418546 110.6108145535225 7.46897311039725e-11
26.491584531418546 140.3608101970589 5.96999496491239e-11
26.491584531418546 178.11239451312218 5.250768546891999e-11
26.491584531418546 226.01768281801222 5.682988574050105e-11
26.491584531418546 286.807625522434 6.544409969307163e-11
26.491584531418546 363.94769219915764 7.16099068421539e-11
26.491584531418546 461.8354285936932 7.446448130723136e-11
26.491584531418546 586.0511487667402 7.516975426628686e-11
26.491584531418546 743.6760536467558 7.476012078552851e-11
26.491584531418546 943.6959110675486 7.384735552612851e-11
26.491584531418546 1197.5133099937427 7.275193261910293e-11
26.491584531418546 1519.5976911565988 7.163643621361013e-11
26.491584531418546 1928.3102105817359 7.058982503168775e-11
26.491584531418546 2446.9504592387466 6.967829311721144e-11
26.491584531418546 3105.0847094578075 6.898336087105477e-11
26.491584531418546 3940.2314078349555 6.86540442639113e-11
26.491584531418546 5000.0 6.904665167313806e-11

33.616787682496685 5.0 4.3147179867687463e-10
33.616787682496685 6.344805015839611 3.8964821503516505e-10
33.616787682496685 8.051310137804697 3.5067490709517004e-10
33.616787682496685 10.216798589284712 3.1455570265994957e-10
33.616787682496685 12.96471898702334 2.812521945931681e-10
33.616787682496685 16.451722811563343 2.5069144384617483e-10
33.616787682496685 20.87659468280201 2.2277192214422383e-10
33.616787682496685 26.491584531418546 1.9736638362029284e-10
33.616787682496685 33.616787682496685 1.743195797491354e-10
33.616787682496685 42.65839262086404 1.534374409264821e-10
33.616787682496685 54.13183669370275 1.344629929808265e-10
33.616787682496685 68.69118979416318 1.1703713710018244e-10
33.616787682496685 87.16644110999944 1.0067643930650343e-10
33.616787682496685 110.6108145535225 8.500407245230657e-11
33.616787682496685 140.3608101970589 7.113927072339365e-11
33.616787682496685 178.11239451312218 6.38443018808042e-11
33.616787682496685 226.01768281801222 6.579914081336511e-11
33.616787682496685 286.807625522434 7.116797343788258e-11
33.616787682496685 363.94769219915764 7.479411936276288e-11
33.616787682496685 461.8354285936932 7.605656007696326e-11
33.616787682496685 586.0511487667402 7.583400463371361e-11
33.616787682496685 743.6760536467558 7.489198332792865e-11
33.616787682496685 943.6959110675486 7.36730414639451e-11
33.616787682496685 1197.5133099937427 7.240100366738816e-11
33.616787682496685 1519.5976911565988 7.118411667727462e-11
33.616787682496685 1928.3102105817359 7.008033120880221e-11
33.616787682496685 2446.9504592387466 6.91375850169191e-11
33.616787682496685 3105.0847094578075 6.842610674033667e-11
33.616787682496685 3940.2314078349555 6.80872260098435e-11
33.616787682496685 5000.0 6.847054393735755e-11

42.65839262086404 5.0 4.110495533075222e-10
42.65839262086404 6.344805015839611 3.740744971672545e-10
42.65839262086404 8.051310137804697 3.392165212707383e-10
42.65839262086404 10.216798589284712 3.065680427180832e-10
42.65839262086404 12.96471898702334 2.761750044287584e-10
42.65839262086404 16.451722811563343 2.4804289512232014e-10
42.65839262086404 20.87659468280201 2.221419989624473e-10
42.65839262086404 26.491584531418546 1.9841060287679213e-10
42.65839262086404 33.616787682496685 1.7675429494568286e-10
42.65839262086404 42.65839262086404 1.570384963080728e-10
42.65839262086404 54.13183669370275 1.3907033913119859e-10
42.65839262086404 68.69118979416318 1.2256846812938097e-10
42.65839262086404 87.16644110999944 1.0714791072172762e-10
42.65839262086404 110.6108145535225 9.251862103549758e-11
42.65839262086404 140.3608101970589 7.964120073015192e-11
42.65839262086404 178.11239451312218 7.235939571902393e-11
42.65839262086404 226.01768281801222 7.254056802389256e-11
42.65839262086404 286.807625522434 7.54384705062243e-11
42.65839262086404 363.94769219915764 7.71322339052435e-11
42.65839262086404 461.8354285936932 7.718840087179044e-11
42.65839262086404 586.0511487667402 7.62674758822932e-11
42.65839262086404 743.6760536467558 7.492841608105125e-11
42.65839262086404 943.6959110675486 7.348409518998529e-11
42.65839262086404 1197.5133099937427 7.208449764391328e-11
42.65839262086404 1519.5976911565988 7.079647752239615e-11
42.65839262086404 1928.3102105817359 6.965442583570457e-11
42.65839262086404 2446.9504592387466 6.869243358905077e-11
42.65839262086404 3105.0847094578075 6.797217434892495e-11
42.65839262086404 3940.2314078349555 6.762916582813168e-11
42.65839262086404 5000.0 6.800799779839654e-11

54.13183669370275 5.0 3.862431584286887e-10
54.13183669370275 6.344805015839611 3.543730958131375e-10
54.13183669370275 8.051310137804697 3.239083467063924e-10
54.13183669370275 10.216798589284712 2.9501022325708016e-10
54.13183669370275 12.96471898702334 2.677953859713375e-10
54.13183669370275 16.451722811563343 2.4233897107411576e-10
54.13183669370275 20.87659468280201 2.1867793802866938e-10
54.13183669370275 26.491584531418546 1.9681343869665603e-10
54.13183669370275 33.616787682496685 1.767105094606765e-10
54.13183669370275 42.65839262086404 1.5829261090794117e-10
54.13183669370275 54.13183669370275 1.4142773473970863e-10
54.13183669370275 68.69118979416318 1.259049352757179e-10
54.13183669370275 87.16644110999944 1.11424611514876e-10
54.13183669370275 110.6108145535225 9.777320097000703e-11
54.13183669370275 140.3608101970589 8.580140444382041e-11
54.13183669370275 178.11239451312218 7.864179127770182e-11
54.13183669370275 226.01768281801222 7.751863956568619e-11
54.13183669370275 286.807625522434 7.855105303780131e-11
54.13183669370275 363.94769219915764 7.878774924807541e-11
54.13183669370275 461.8354285936932 7.794087940857515e-11
54.13183669370275 586.0511487667402 7.650298759394285e-11
54.13183669370275 743.6760536467558 7.48747477222391e-11
54.13183669370275 943.6959110675486 7.32701094109632e-11
54.13183669370275 1197.5133099937427 7.178299351139984e-11
54.13183669370275 1519.5976911565988 7.044898078857054e-11
54.13183669370275 1928.3102105817359 6.928473745509829e-11
54.13183669370275 2446.9504592387466 6.831396820736929e-11
54.13183669370275 3105.0847094578075 6.759194121726251e-11
54.13183669370275 3940.2314078349555 6.724983807335436e-11
54.13183669370275 5000.0 6.762858901558422e-11

68.69118979416318 5.0 3.576121928259355e-10
68.69118979416318 6.344805015839611 3.3096724933566566e-10
68.69118979416318 8.051310137804697 3.0507867918820206e-10
68.69118979416318 10.216798589284712 2.8014942596774303e-10
68.69118979416318 12.96471898702334 2.56345869567679e-10
68.69118979416318 16.451722811563343 2.3379737011764465e-10
68.69118979416318 20.87659468280201 2.1259679286443443e-10
68.69118979416318 26.491584531418546 1.928009863572083e-10
68.69118979416318 33.616787682496685 1.7442971940789146e-10
68.69118979416318 42.65839262086404 1.5746093136760803e-10
68.69118979416318 54.13183669370275 1.4181945588419133e-10
68.69118979416318 68.69118979416318 1.273582314725833e-10
68.69118979416318 87.16644110999944 1.1385248244762148e-10
68.69118979416318 110.6108145535225 1.0115759268562059e-10
68.69118979416318 140.3608101970589 9.005472980926481e-11
68.69118979416318 178.11239451312218 8.312382550881642e-11
68.69118979416318 226.01768281801222 8.107341762551201e-11
68.69118979416318 286.807625522434 8.071998291272164e-11
68.69118979416318 363.94769219915764 7.987696572840045e-11
68.69118979416318 461.8354285936932 7.836925499047892e-11
68.69118979416318 586.0511487667402 7.656055815614205e-11
68.69118979416318 743.6760536467558 7.473105689829233e-11
68.69118979416318 943.6959110675486 7.301992979966414e-11
68.69118979416318 1197.5133099937427 7.147905816782993e-11
68.69118979416318 1519.5976911565988 7.012076424236498e-11
68.69118979416318 1928.3102105817359 6.894862743875126e-11
68.69118979416318 2446.9504592387466 6.797872296367315e-11
68.69118979416318 3105.0847094578075 6.726162845217606e-11
68.69118979416318 3940.2314078349555 6.6925371017706e-11
68.69118979416318 5000.0 6.730832582707747e-11

87.16644110999944 5.0 3.2597746238182413e-10
87.16644110999944 6.344805015839611 3.044843799062931e-10
87.16644110999944 8.051310137804697 2.832044132601445e-10
87.16644110999944 10.216798589284712 2.6235063401699936e-10
87.16644110999944 12.96471898702334 2.42112567131174e-10
87.16644110999944 16.451722811563343 2.226523558016072e-10
87.16644110999944 20.87659468280201 2.0410218836434855e-10
87.16644110999944 26.491584531418546 1.8656226006622903e-10
87.16644110999944 33.616787682496685 1.700980831540207e-10
87.16644110999944 42.65839262086404 1.5473531727292747e-10
87.16644110999944 54.13183669370275 1.404496499981601e-10
87.16644110999944 68.69118979416318 1.2715081428638393e-10
87.16644110999944 87.16644110999944 1.1467924478631974e-10
87.16644110999944 110.6108145535225 1.0295331758645224e-10
87.16644110999944 140.3608101970589 9.27192431144205e-11
87.16644110999944 178.11239451312218 8.612351808273702e-11
87.16644110999944 226.01768281801222 8.345342536577013e-11
87.16644110999944 286.807625522434 8.209938051687164e-11
87.16644110999944 363.94769219915764 8.048086057855392e-11
87.16644110999944 461.8354285936932 7.850925110520367e-11
87.16644110999944 586.0511487667402 7.64500819316376e-11
87.16644110999944 743.6760536467558 7.449287742815088e-11
87.16644110999944 943.6959110675486 7.272121774595418e-11
87.16644110999944 1197.5133099937427 7.115614086072723e-11
87.16644110999944 1519.5976911565988 6.979314718449666e-11
87.16644110999944 1928.3102105817359 6.862647238837876e-11
87.16644110999944 2446.9504592387466 6.766679406932564e-11
87.16644110999944 3105.0847094578075 6.696139027447124e-11
87.16644110999944 3940.2314078349555 6.66360970158665e-11
87.16644110999944 5000.0 6.702766499438196e-11

110.6108145535225 5.0 2.92433527429115e-10
110.6108145535225 6.344805015839611 2.7579333932414006e-10
110.6108145535225 8.051310137804697 2.5896283705993395e-10
110.6108145535225 10.216798589284712 2.421351485827701e-10
110.6108145535225 12.96471898702334 2.254948953682373e-10
110.6108145535225 16.451722811563343 2.092121823186603e-10
110.6108145535225 20.87659468280201 1.934375429717974e-10
110.6108145535225 26.491584531418546 1.7829749192098266e-10
110.6108145535225 33.616787682496685 1.6388986607280244e-10
110.6108145535225 42.65839262086404 1.5027749566395617e-10
110.6108145535225 54.13183669370275 1.3747805630923748e-10
110.6108145535225 68.69118979416318 1.254492097123984e-10
110.6108145535225 87.16644110999944 1.1408641784253603e-10
110.6108145535225 110.6108145535225 1.033657550005885e-10
110.6108145535225 140.3608101970589 9.402949332618329e-11
110.6108145535225 178.11239451312218 8.787566994694137e-11
110.6108145535225 226.01768281801222 8.483960637068358e-11
110.6108145535225 286.807625522434 8.279859502761701e-11
110.6108145535225 363.94769219915764 8.065376918435496e-11
110.6108145535225 461.8354285936932 7.83815066326623e-11
110.6108145535225 586.0511487667402 7.617328676737667e-11
110.6108145535225 743.6760536467558 7.415170962344507e-11
110.6108145535225 943.6959110675486 7.236011846173948e-11
110.6108145535225 1197.5133099937427 7.079774993431196e-11
110.6108145535225 1519.5976911565988 6.944852214102106e-11
110.6108145535225 1928.3102105817359 6.83003939621546e-11
110.6108145535225 2446.9504592387466 6.7360481337304e-11
110.6108145535225 3105.0847094578075 6.66739092711239e-11
110.6108145535225 3940.2314078349555 6.636512397183689e-11
110.6108145535225 5000.0 6.677006323718186e-11

140.3608101970589 5.0 2.582871717496648e-10
140.3608101970589 6.344805015839611 2.459818282276194e-10
140.3608101970589 8.051310137804697 2.332378390675974e-10
140.3608101970589 10.216798589284712 2.2020613360399466e-10
140.3608101970589 12.96471898702334 2.0704252929872048e-10
140.3608101970589 16.451722811563343 1.939013809948935e-10
140.3608101970589 20.87659468280201 1.8092945045849786e-10
140.3608101970589 26.491584531418546 1.6825995174708567e-10
140.3608101970589 33.616787682496685 1.5600630557814558e-10
140.3608101970589 42.65839262086404 1.4425449664906761e-10
140.3608101970589 54.13183669370275 1.3305214741224012e-10
140.3608101970589 68.69118979416318 1.2239338262126266e-10
140.3608101970589 87.16644110999944 1.1221669216155962e-10
140.3608101970589 110.6108145535225 1.0255079111368953e-10
140.3608101970589 140.3608101970589 9.416372652697003e-11
140.3608101970589 178.11239451312218 8.855618491996965e-11
140.3608101970589 226.01768281801222 8.536380656656456e-11
140.3608101970589 286.807625522434 8.289415493567823e-11
140.3608101970589 363.94769219915764 8.043022731356134e-11
140.3608101970589 461.8354285936932 7.799514884682706e-11
140.3608101970589 586.0511487667402 7.572535829094622e-11
140.3608101970589 743.6760536467558 7.369549973087254e-11
140.3608101970589 943.6959110675486 7.192106773905285e-11
140.3608101970589 1197.5133099937427 7.03868629462284e-11
140.3608101970589 1519.5976911565988 6.906953296351775e-11
140.3608101970589 1928.3102105817359 6.795330435978333e-11
140.3608101970589 2446.9504592387466 6.704326133880505e-11
140.3608101970589 3105.0847094578075 6.638333329789541e-11
140.3608101970589 3940.2314078349555 6.60972544529025e-11
140.3608101970589 5000.0 6.652088741477366e-11

178.11239451312218 5.0 2.2492015287974023e-10
178.11239451312218 6.344805015839611 2.1626307760305085e-10
178.11239451312218 8.051310137804697 2.0706500951105749e-10
178.11239451312218 10.216798589284712 1.974247071677137e-10
178.11239451312218 12.96471898702334 1.874545730100178e-10
178.11239451312218 16.451722811563343 1.7727567121096365e-10
178.11239451312218 20.87659468280201 1.6701217619603688e-10
178.11239451312218 26.491584531418546 1.567853151728238e-10
178.11239451312218 33.616787682496685 1.4670653646827875e-10
178.11239451312218 42.65839262086404 1.3686902355191494e-10
178.11239451312218 54.13183669370275 1.273357853437111e-10
178.11239451312218 68.69118979416318 1.1812321758221445e-10
178.11239451312218 87.16644110999944 1.0919830585757904e-10
178.11239451312218 110.6108145535225 1.0063852492892497e-10
178.11239451312218 140.3608101970589 9.326819768424974e-11
178.11239451312218 178.11239451312218 8.830215764942272e-11
178.11239451312218 226.01768281801222 8.512399067146443e-11
178.11239451312218 286.807625522434 8.243983586123487e-11
178.11239451312218 363.94769219915764 7.983091093983537e-11
178.11239451312218 461.8354285936932 7.735103710506297e-11
178.11239451312218 586.0511487667402 7.509653968057792e-11
178.11239451312218 743.6760536467558 7.310924990643658e-11
178.11239451312218 943.6959110675486 7.138680332800594e-11
178.11239451312218 1197.5133099937427 6.990557497256668e-11
178.11239451312218 1519.5976911565988 6.863850340610233e-11
178.11239451312218 1928.3102105817359 6.756820433304532e-11
178.11239451312218 2446.9504592387466 6.66990109991288e-11
178.11239451312218 3105.0847094578075 6.607445925972548e-11
178.11239451312218 3940.2314078349555 6.58181504194543e-11
178.11239451312218 5000.0 6.626657138747452e-11

226.01768281801222 5.0 1.936074192502998e-10
226.01768281801222 6.344805015839611 1.878283092807602e-10
226.01768281801222 8.051310137804697 1.8152082125410987e-10
226.01768281801222 10.216798589284712 1.747343106653299e-10
226.01768281801222 12.96471898702334 1.6753477421777338e-10
226.01768281801222 16.451722811563343 1.6000214318099143e-10
226.01768281801222 20.87659468280201 1.5222651151594947e-10
226.01768281801222 26.491584531418546 1.4430327598254955e-10
226.01768281801222 33.616787682496685 1.363269126939325e-10
226.01768281801222 42.65839262086404 1.283825143761291e-10
226.01768281801222 54.13183669370275 1.2053315907231132e-10
226.01768281801222 68.69118979416318 1.1280149556121638e-10
226.01768281801222 87.16644110999944 1.0516631661805545e-10
226.01768281801222 110.6108145535225 9.775553902410766e-11
226.01768281801222 140.3608101970589 9.148036784257792e-11
226.01768281801222 178.11239451312218 8.722871686621642e-11
226.01768281801222 226.01768281801222 8.419751936107593e-11
226.01768281801222 286.807625522434 8.147584873319067e-11
226.01768281801222 363.94769219915764 7.886833481758135e-11
226.01768281801222 461.8354285936932 7.644510427061841e-11
226.01768281801222 586.0511487667402 7.427397946357233e-11
226.01768281801222 743.6760536467558 7.237592749638844e-11
226.01768281801222 943.6959110675486 7.073868015942701e-11
226.01768281801222 1197.5133099937427 6.93350340642314e-11
226.01768281801222 1519.5976911565988 6.813712968903335e-11
226.01768281801222 1928.3102105817359 6.712772197724595e-11
226.01768281801222 2446.9504592387466 6.631145113775704e-11
226.01768281801222 3105.0847094578075 6.573212030425273e-11
226.01768281801222 3940.2314078349555 6.551368971154582e-11
226.01768281801222 5000.0 6.599396113189703e-11

286.807625522434 5.0 1.653582171698766e-10
286.807625522434 6.344805015839611 1.6169922115819905e-10
286.807625522434 8.051310137804697 1.5759602603568116e-10
286.807625522434 10.216798589284712 1.5306054322182947e-10
286.807625522434 12.96471898702334 1.4811945980740438e-10
286.807625522434 16.451722811563343 1.4281374818806713e-10
286.807625522434 20.87659468280201 1.3719701321957654e-10
286.807625522434 26.491584531418546 1.3133249735692493e-10
286.807625522434 33.616787682496685 1.2528830984932415e-10
286.807625522434 42.65839262086404 1.1912979039858427e-10
286.807625522434 54.13183669370275 1.129065607511794e-10
286.807625522434 68.69118979416318 1.066315785350118e-10
286.807625522434 87.16644110999944 1.0027905415488322e-10
286.807625522434 110.6108145535225 9.404799170467865e-11
286.807625522434 140.3608101970589 8.895030871813663e-11
286.807625522434 178.11239451312218 8.544206545195112e-11
286.807625522434 226.01768281801222 8.265311106626959e-11
286.807625522434 286.807625522434 8.003766161073603e-11
286.807625522434 363.94769219915764 7.75526912294262e-11
286.807625522434 461.8354285936932 7.5272085997116e-11
286.807625522434 586.0511487667402 7.32440507123581e-11
286.807625522434 743.6760536467558 7.14778430395373e-11
286.807625522434 943.6959110675486 6.995741318863578e-11
286.807625522434 1197.5133099937427 6.865575134948484e-11
286.807625522434 1519.5976911565988 6.754649387160578e-11
286.807625522434 1928.3102105817359 6.661392341100365e-11
286.807625522434 2446.9504592387466 6.586382114488126e-11
286.807625522434 3105.0847094578075 6.534077204809453e-11
286.807625522434 3940.2314078349555 6.516949835246762e-11
286.807625522434 5000.0 6.568982389025239e-11

363.94769219915764 5.0 1.408364905149642e-10
363.94769219915764 6.344805015839611 1.3863296702216594e-10
363.94769219915764 8.051310137804697 1.3609731144846006e-10
363.94769219915764 10.216798589284712 1.3321952193713247e-10
363.94769219915764 12.96471898702334 1.2999977542715232e-10
363.94769219915764 16.451722811563343 1.2644941227487862e-10
363.94769219915764 20.87659468280201 1.2259097655125894e-10
363.94769219915764 26.491584531418546 1.1845697458515736e-10
363.94769219915764 33.616787682496685 1.1408671519445993e-10
363.94769219915764 42.65839262086404 1.0951977017374327e-10
363.94769219915764 54.13183669370275 1.0478266522016103e-10
363.94769219915764 68.69118979416318 9.986458349471822e-11
363.94769219915764 87.16644110999944 9.472689571224967e-11
363.94769219915764 110.6108145535225 8.971335999705006e-11
363.94769219915764 140.3608101970589 8.585263204665702e-11
363.94769219915764 178.11239451312218 8.304723454733687e-11
363.94769219915764 226.01768281801222 8.056148609991771e-11
363.94769219915764 286.807625522434 7.816440392618486e-11
363.94769219915764 363.94769219915764 7.589785552537834e-11
363.94769219915764 461.8354285936932 7.382973318047892e-11
363.94769219915764 586.0511487667402 7.199527059075941e-11
363.94769219915764 743.6760536467558 7.039863339759941e-11
363.94769219915764 943.6959110675486 6.902437636031387e-11
363.94769219915764 1197.5133099937427 6.784839606843314e-11
363.94769219915764 1519.5976911565988 6.684748734616013e-11
363.94769219915764 1928.3102105817359 6.60084638102677e-11
363.94769219915764 2446.9504592387466 6.533883327733497e-11
363.94769219915764 3105.0847094578075 6.488430832103865e-11
363.94769219915764 3940.2314078349555 6.477067471644764e-11
363.94769219915764 5000.0 6.5340529013566e-11

461.8354285936932 5.0 1.20334062617643e-10
461.8354285936932 6.344805015839611 1.190620564360146e-10
461.8354285936932 8.051310137804697 1.1756434447723757e-10
461.8354285936932 10.216798589284712 1.1582271537876116e-10
461.8354285936932 12.96471898702334 1.1382418091210726e-10
461.8354285936932 16.451722811563343 1.1156242975302674e-10
461.8354285936932 20.87659468280201 1.0903870057622099e-10
461.8354285936932 26.491584531418546 1.0626160220685479e-10
461.8354285936932 33.616787682496685 1.0324499624589182e-10
461.8354285936932 42.65839262086404 1.000018836003308e-10
461.8354285936932 54.13183669370275 9.652932898162564e-11
461.8354285936932 68.69118979416318 9.278046761502229e-11
461.8354285936932 87.16644110999944 8.874009547315379e-11
461.8354285936932 110.6108145535225 8.505145175587619e-11
461.8354285936932 140.3608101970589 8.23686512017656e-11
461.8354285936932 178.11239451312218 8.015109172671562e-11
461.8354285936932 226.01768281801222 7.800420608889126e-11
461.8354285936932 286.807625522434 7.590616006719734e-11
461.8354285936932 363.94769219915764 7.392712390780404e-11
461.8354285936932 461.8354285936932 7.212330447447451e-11
461.8354285936932 586.0511487667402 7.052177171893293e-11
461.8354285936932 743.6760536467558 6.912589258868801e-11
461.8354285936932 943.6959110675486 6.792354557267369e-11
461.8354285936932 1197.5133099937427 6.689518091744701e-11
461.8354285936932 1519.5976911565988 6.60217489393485e-11
461.8354285936932 1928.3102105817359 6.5293172256977e-11
461.8354285936932 2446.9504592387466 6.471898434591397e-11
461.8354285936932 3105.0847094578075 6.434616912037858e-11
461.8354285936932 3940.2314078349555 6.430175478784678e-11
461.8354285936932 5000.0 6.493194081147201e-11

586.0511487667402 5.0 1.0376143654523966e-10
586.0511487667402 6.344805015839611 1.0304794343088231e-10
586.0511487667402 8.051310137804697 1.0219171257885194e-10
586.0511487667402 10.216798589284712 1.0117491432802588e-10
586.0511487667402 12.96471898702334 9.998125777148535e-11
586.0511487667402 16.451722811563343 9.859708645036027e-11
586.0511487667402 20.87659468280201 9.701214475986828e-11
586.0511487667402 26.491584531418546 9.521940352474537e-11
586.0511487667402 33.616787682496685 9.32125975879168e-11
586.0511487667402 42.65839262086404 9.097809529911661e-11
586.0511487667402 54.13183669370275 8.847411560180094e-11
586.0511487667402 68.69118979416318 8.56262154614917e-11
586.0511487667402 87.16644110999944 8.27032239470183e-11
586.0511487667402 110.6108145535225 8.044385619002949e-11
586.0511487667402 140.3608101970589 7.863250049486433e-11
586.0511487667402 178.11239451312218 7.686659152242953e-11
586.0511487667402 226.01768281801222 7.507958624994767e-11
586.0511487667402 286.807625522434 7.332882396228214e-11
586.0511487667402 363.94769219915764 7.16777557648532e-11
586.0511487667402 461.8354285936932 7.016975650920514e-11
586.0511487667402 586.0511487667402 6.882700357687909e-11
586.0511487667402 743.6760536467558 6.765431001667933e-11
586.0511487667402 943.6959110675486 6.664406348163937e-11
586.0511487667402 1197.5133099937427 6.578188502506918e-11
586.0511487667402 1519.5976911565988 6.505320050278792e-11
586.0511487667402 1928.3102105817359 6.445116633537452e-11
586.0511487667402 2446.9504592387466 6.398732021740626e-11
586.0511487667402 3105.0847094578075 6.370982623191983e-11
586.0511487667402 3940.2314078349555 6.374699359361076e-11
586.0511487667402 5000.0 6.444959456970151e-11

743.6760536467558 5.0 9.06941103096314e-11
743.6760536467558 6.344805015839611 9.029681004383201e-11
743.6760536467558 8.051310137804697 8.981260762342518e-11
743.6760536467558 10.216798589284712 8.922721029071581e-11
743.6760536467558 12.96471898702334 8.852567650403394e-11
743.6760536467558 16.451722811563343 8.769265303874936e-11
743.6760536467558 20.87659468280201 8.671204966824417e-11
743.6760536467558 26.491584531418546 8.556501121211311e-11
743.6760536467558 33.616787682496685 8.422340601726512e-11
743.6760536467558 42.65839262086404 8.263540466621403e-11
743.6760536467558 54.13183669370275 8.075079025281426e-11
743.6760536467558 68.69118979416318 7.884271178460399e-11
743.6760536467558 87.16644110999944 7.734169937252509e-11
743.6760536467558 110.6108145535225 7.604590063502286e-11
743.6760536467558 140.3608101970589 7.471839227017424e-11
743.6760536467558 178.11239451312218 7.332293648570657e-11
743.6760536467558 226.01768281801222 7.190349621784086e-11
743.6760536467558 286.807625522434 7.05149177460278e-11
743.6760536467558 363.94769219915764 6.92030818459253e-11
743.6760536467558 461.8354285936932 6.800070053166494e-11
743.6760536467558 586.0511487667402 6.692701816794039e-11
743.6760536467558 743.6760536467558 6.598891159598103e-11
743.6760536467558 943.6959110675486 6.518320785854806e-11
743.6760536467558 1197.5133099937427 6.45004290786671e-11
743.6760536467558 1519.5976911565988 6.393018269916831e-11
743.6760536467558 1928.3102105817359 6.346855101849493e-11
743.6760536467558 2446.9504592387466 6.312873358279254e-11
743.6760536467558 3105.0847094578075 6.295973814121542e-11
743.6760536467558 3940.2314078349555 6.309105518274014e-11
743.6760536467558 5000.0 6.387925942368284e-11

943.6959110675486 5.0 8.044905570109206e-11
943.6959110675486 6.344805015839611 8.021534647538633e-11
943.6959110675486 8.051310137804697 7.992509671878667e-11
943.6959110675486 10.216798589284712 7.956551040037171e-11
943.6959110675486 12.96471898702334 7.912048996105762e-11
943.6959110675486 16.451722811563343 7.856883979437212e-11
943.6959110675486 20.87659468280201 7.788222948496879e-11
943.6959110675486 26.491584531418546 7.706607422468144e-11
943.6959110675486 33.616787682496685 7.605474758098459e-11
943.6959110675486 42.65839262086404 7.510601409374585e-11
943.6959110675486 54.13183669370275 7.428058400255162e-11
943.6959110675486 68.69118979416318 7.349671277426661e-11
943.6959110675486 87.16644110999944 7.265817098599053e-11
943.6959110675486 110.6108145535225 7.17303611117272e-11
943.6959110675486 140.3608101970589 7.072392466941237e-11
943.6959110675486 178.11239451312218 6.966927461429772e-11
943.6959110675486 226.01768281801222 6.860257716458258e-11
943.6959110675486 286.807625522434 6.75593604288342e-11
943.6959110675486 363.94769219915764 6.65711381341832e-11
943.6959110675486 461.8354285936932 6.566309557733586e-11
943.6959110675486 586.0511487667402 6.485245023730018e-11
943.6959110675486 743.6760536467558 6.414771648774433e-11
943.6959110675486 943.6959110675486 6.35492834303612e-11
943.6959110675486 1197.5133099937427 6.305170440503707e-11
943.6959110675486 1519.5976911565988 6.264803563422819e-11
943.6959110675486 1928.3102105817359 6.233665113989423e-11
943.6959110675486 2446.9504592387466 6.213181362912839e-11
943.6959110675486 3105.0847094578075 6.208283443081916e-11
943.6959110675486 3940.2314078349555 6.232020182061517e-11
943.6959110675486 5000.0 6.320801682528769e-11

1197.5133099937427 5.0 7.191174060286507e-11
1197.5133099937427 6.344805015839611 7.179488464138633e-11
1197.5133099937427 8.051310137804697 7.1657527987179e-11
1197.5133099937427 10.216798589284712 7.149782310538146e-11
1197.5133099937427 12.96471898702334 7.131344860714264e-11
1197.5133099937427 16.451722811563343 7.110080465859807e-11
1197.5133099937427 20.87659468280201 7.085417687950848e-11
1197.5133099937427 26.491584531418546 7.056543200959486e-11
1197.5133099937427 33.616787682496685 7.022476099796399e-11
1197.5133099937427 42.65839262086404 6.982249013761973e-11
1197.5133099937427 54.13183669370275 6.935136867588992e-11
1197.5133099937427 68.69118979416318 6.880852441010223e-11
1197.5133099937427 87.16644110999944 6.819658782647359e-11
1197.5133099937427 110.6108145535225 6.752395072184753e-11
1197.5133099937427 140.3608101970589 6.680436780873297e-11
1197.5133099937427 178.11239451312218 6.605608710448799e-11
1197.5133099937427 226.01768281801222 6.530058290303435e-11
1197.5133099937427 286.807625522434 6.4560905596344e-11
1197.5133099937427 363.94769219915764 6.385969637572545e-11
1197.5133099937427 461.8354285936932 6.321702280021513e-11
1197.5133099937427 586.0511487667402 6.264833259002119e-11
1197.5133099937427 743.6760536467558 6.216295963315459e-11
1197.5133099937427 943.6959110675486 6.176371227739252e-11
1197.5133099937427 1197.5133099937427 6.144810166414432e-11
1197.5133099937427 1519.5976911565988 6.121174257978065e-11
1197.5133099937427 1928.3102105817359 6.105454544247887e-11
1197.5133099937427 2446.9504592387466 6.099113487250747e-11
1197.5133099937427 3105.0847094578075 6.107050629872466e-11
1197.5133099937427 3940.2314078349555 6.142402750620951e-11
1197.5133099937427 5000.0 6.242599972663837e-11

1519.5976911565988 5.0 6.648114180960749e-11
1519.5976911565988 6.344805015839611 6.64230945914316e-11
1519.5976911565988 8.051310137804697 6.635074286752371e-11
1519.5976911565988 10.216798589284712 6.626096231340269e-11
1519.5976911565988 12.96471898702334 6.615016078410279e-11
1519.5976911565988 16.451722811563343 6.601432083992856e-11
1519.5976911565988 20.87659468280201 6.584911076222225e-11
1519.5976911565988 26.491584531418546 6.565008735443419e-11
1519.5976911565988 33.616787682496685 6.54130101780651e-11
1519.5976911565988 42.65839262086404 6.513427497710872e-11
1519.5976911565988 54.13183669370275 6.481145405882989e-11
1519.5976911565988 68.69118979416318 6.444390543211071e-11
1519.5976911565988 87.16644110999944 6.403338466990867e-11
1519.5976911565988 110.6108145535225 6.35845705930912e-11
1519.5976911565988 140.3608101970589 6.310540182899579e-11
1519.5976911565988 178.11239451312218 6.26071181593148e-11
1519.5976911565988 226.01768281801222 6.210391073708558e-11
1519.5976911565988 286.807625522434 6.161211372366404e-11
1519.5976911565988 363.94769219915764 6.114892586130008e-11
1519.5976911565988 461.8354285936932 6.073074511073019e-11
1519.5976911565988 586.0511487667402 6.03713288329384e-11
1519.5976911565988 743.6760536467558 6.00801545273643e-11
1519.5976911565988 943.6959110675486 5.98615131889245e-11
1519.5976911565988 1197.5133099937427 5.971498547987112e-11
1519.5976911565988 1519.5976911565988 5.963801510625203e-11
1519.5976911565988 1928.3102105817359 5.963143956414876e-11
1519.5976911565988 2446.9504592387466 5.970967713430861e-11
1519.5976911565988 3105.0847094578075 5.992093312266852e-11
1519.5976911565988 3940.2314078349555 6.039769830159006e-11
1519.5976911565988 5000.0 6.152896518165938e-11

1928.3102105817359 5.0 6.179838073106936e-11
1928.3102105817359 6.344805015839611 6.176326641077722e-11
1928.3102105817359 8.051310137804697 6.171946355098048e-11
1928.3102105817359 10.216798589284712 6.16650541230932e-11
1928.3102105817359 12.96471898702334 6.159782097186226e-11
1928.3102105817359 16.451722811563343 6.151526632865203e-11
1928.3102105817359 20.87659468280201 6.141466999915822e-11
1928.3102105817359 26.491584531418546 6.129320244824872e-11
1928.3102105817359 33.616787682496685 6.114810733899025e-11
1928.3102105817359 42.65839262086404 6.097696367524035e-11
1928.3102105817359 54.13183669370275 6.077802862289378e-11
1928.3102105817359 68.69118979416318 6.055064815914209e-11
1928.3102105817359 87.16644110999944 6.029570543562329e-11
1928.3102105817359 110.6108145535225 6.001605775466899e-11
1928.3102105817359 140.3608101970589 5.971689510460225e-11
1928.3102105817359 178.11239451312218 5.940593804901428e-11
1928.3102105817359 226.01768281801222 5.909338419883112e-11
1928.3102105817359 286.807625522434 5.879151586039403e-11
1928.3102105817359 363.94769219915764 5.851390640758405e-11
1928.3102105817359 461.8354285936932 5.827422287136374e-11
1928.3102105817359 586.0511487667402 5.808472952895968e-11
1928.3102105817359 743.6760536467558 5.795475419058984e-11
1928.3102105817359 943.6959110675486 5.7889572629963085e-11
1928.3102105817359 1197.5133099937427 5.789036326950963e-11
1928.3102105817359 1519.5976911565988 5.795606171984481e-11
1928.3102105817359 1928.3102105817359 5.808821125441202e-11
1928.3102105817359 2446.9504592387466 5.830085277031066e-11
1928.3102105817359 3105.0847094578075 5.864138753304177e-11
1928.3102105817359 3940.2314078349555 5.9244545133337e-11
1928.3102105817359 5000.0 6.052198168285433e-11

2446.9504592387466 5.0 5.787398097571654e-11
2446.9504592387466 6.344805015839611 5.785448333638465e-11
2446.9504592387466 8.051310137804697 5.7830107793042235e-11
2446.9504592387466 10.216798589284712 5.779974942725133e-11
2446.9504592387466 12.96471898702334 5.776211700043889e-11
2446.9504592387466 16.451722811563343 5.771573666466556e-11
2446.9504592387466 20.87659468280201 5.7658978015987975e-11
2446.9504592387466 26.491584531418546 5.759011347204706e-11
2446.9504592387466 33.616787682496685 5.750742299527678e-11
2446.9504592387466 42.65839262086404 5.740935556882933e-11
2446.9504592387466 54.13183669370275 5.729475479922199e-11
2446.9504592387466 68.69118979416318 5.716314814456876e-11
2446.9504592387466 87.16644110999944 5.701508632692194e-11
2446.9504592387466 110.6108145535225 5.685250484056849e-11
2446.9504592387466 140.3608101970589 5.6679061351999904e-11
2446.9504592387466 178.11239451312218 5.650038685109999e-11
2446.9504592387466 226.01768281801222 5.6324175445885485e-11
2446.9504592387466 286.807625522434 5.6160030792241306e-11
2446.9504592387466 363.94769219915764 5.6018994134890907e-11
2446.9504592387466 461.8354285936932 5.591271157067634e-11
2446.9504592387466 586.0511487667402 5.585227058342903e-11
2446.9504592387466 743.6760536467558 5.5846865405874947e-11
2446.9504592387466 943.6959110675486 5.590264118284621e-11
2446.9504592387466 1197.5133099937427 5.602230713166767e-11
2446.9504592387466 1519.5976911565988 5.620638929351918e-11
2446.9504592387466 1928.3102105817359 5.6457416215182744e-11
2446.9504592387466 2446.9504592387466 5.67894877435773e-11
2446.9504592387466 3105.0847094578075 5.725002171563471e-11
2446.9504592387466 3940.2314078349555 5.797881862612915e-11
2446.9504592387466 5000.0 5.942499969693209e-11

3105.0847094578075 5.0 5.463185638029386e-11
3105.0847094578075 6.344805015839611 5.462170387363267e-11
3105.0847094578075 8.051310137804697 5.460899322335885e-11
3105.0847094578075 10.216798589284712 5.459313559550618e-11
3105.0847094578075 12.96471898702334 5.457343846360435e-11
3105.0847094578075 16.451722811563343 5.454910570652782e-11
3105.0847094578075 20.87659468280201 5.451924995057744e-11
3105.0847094578075 26.491584531418546 5.448292442763806e-11
3105.0847094578075 33.616787682496685 5.4439183079234256e-11
3105.0847094578075 42.65839262086404 5.4387178755135545e-11
3105.0847094578075 54.13183669370275 5.4326308650347844e-11
3105.0847094578075 68.69118979416318 5.4256412545521263e-11
3105.0847094578075 87.16644110999944 5.417802213813398e-11
3105.0847094578075 110.6108145535225 5.4092648303796906e-11
3105.0847094578075 140.3608101970589 5.4003078296213624e-11
3105.0847094578075 178.11239451312218 5.391363816956768e-11
3105.0847094578075 226.01768281801222 5.383036044000977e-11
3105.0847094578075 286.807625522434 5.376098451199229e-11
3105.0847094578075 363.94769219915764 5.371471545778842e-11
3105.0847094578075 461.8354285936932 5.370168074037578e-11
3105.0847094578075 586.0511487667402 5.373207084713088e-11
3105.0847094578075 743.6760536467558 5.381504596553327e-11
3105.0847094578075 943.6959110675486 5.395765715474598e-11
3105.0847094578075 1197.5133099937427 5.416428001774455e-11
3105.0847094578075 1519.5976911565988 5.44374140760596e-11
3105.0847094578075 1928.3102105817359 5.478129182720235e-11
3105.0847094578075 2446.9504592387466 5.521121701623742e-11
3105.0847094578075 3105.0847094578075 5.577672035391638e-11
3105.0847094578075 3940.2314078349555 5.662872889796471e-11
3105.0847094578075 5000.0 5.828293032394973e-11

3940.2314078349555 5.0 5.1966526248978295e-11
3940.2314078349555 6.344805015839611 5.1961770353884553e-11
3940.2314078349555 8.051310137804697 5.195581573281355e-11
3940.2314078349555 10.216798589284712 5.1948386847550844e-11
3940.2314078349555 12.96471898702334 5.1939160478161586e-11
3940.2314078349555 16.451722811563343 5.1927766953092835e-11
3940.2314078349555 20.87659468280201 5.191379838668522e-11
3940.2314078349555 26.491584531418546 5.1896828294995355e-11
3940.2314078349555 33.616787682496685 5.187644843220916e-11
3940.2314078349555 42.65839262086404 5.185233012558911e-11
3940.2314078349555 54.13183669370275 5.182431798859898e-11
3940.2314078349555 68.69118979416318 5.1792563399599e-11
3940.2314078349555 87.16644110999944 5.1757701633833246e-11
3940.2314078349555 110.6108145535225 5.1721069944566065e-11
3940.2314078349555 140.3608101970589 5.1684953125829854e-11
3940.2314078349555 178.11239451312218 5.1652828822812855e-11
3940.2314078349555 226.01768281801222 5.162956894846365e-11
3940.2314078349555 286.807625522434 5.1621538298317215e-11
3940.2314078349555 363.94769219915764 5.1636522666570137e-11
3940.2314078349555 461.8354285936932 5.168342095363366e-11
3940.2314078349555 586.0511487667402 5.17716629958483e-11
3940.2314078349555 743.6760536467558 5.191038239945499e-11
3940.2314078349555 943.6959110675486 5.210751033668913e-11
3940.2314078349555 1197.5133099937427 5.2369194285844975e-11
3940.2314078349555 1519.5976911565988 5.270034881220431e-11
3940.2314078349555 1928.3102105817359 5.310791018486082e-11
3940.2314078349555 2446.9504592387466 5.36103022338538e-11
3940.2314078349555 3105.0847094578075 5.426326589010928e-11
3940.2314078349555 3940.2314078349555 5.524141807819585e-11
3940.2314078349555 5000.0 5.718996152627206e-11

5000.0 5.0 4.979026053223809e-11
5000.0 6.344805015839611 4.9788505941260916e-11
5000.0 8.051310137804697 4.978631673709105e-11
5000.0 10.216798589284712 4.9783597979250715e-11
5000.0 12.96471898702334 4.97802417834892e-11
5000.0 16.451722811563343 4.977613073807778e-11
5000.0 20.87659468280201 4.977114569146561e-11
5000.0 26.491584531418546 4.9765180571355107e-11
5000.0 33.616787682496685 4.9758167886341184e-11
5000.0 42.65839262086404 4.9750119847526484e-11
5000.0 54.13183669370275 4.9741190936252864e-11
5000.0 68.69118979416318 4.973176850489458e-11
5000.0 87.16644110999944 4.9722596923534627e-11
5000.0 110.6108145535225 4.971493787489958e-11
5000.0 140.3608101970589 4.971076304528106e-11
5000.0 178.11239451312218 4.971296536349097e-11
5000.0 226.01768281801222 4.972556162044719e-11
5000.0 286.807625522434 4.975384400884042e-11
5000.0 363.94769219915764 4.9804425525363165e-11
5000.0 461.8354285936932 4.9885118811742115e-11
5000.0 586.0511487667402 5.000460101702918e-11
5000.0 743.6760536467558 5.017186452189836e-11
5000.0 943.6959110675486 5.0395563660137207e-11
5000.0 1197.5133099937427 5.068359142617355e-11
5000.0 1519.5976911565988 5.104366487488054e-11
5000.0 1928.3102105817359 5.148667432822816e-11
5000.0 2446.9504592387466 5.2037222912152994e-11
5000.0 3105.0847094578075 5.2765291918501835e-11
5000.0 3940.2314078349555 5.389745965685797e-11
5000.0 5000.0 5.63693556900999e-11


==> 5_Results/Figures/Mixture_P_Na_IOM_DM_diff.tex <==
x y z
5.0 5.0 0.9357122570269507
5.0 6.344805015839611 0.9396617969769004
5.0 8.051310137804697 0.9453680642658056
5.0 10.216798589284712 0.9542735643600961
5.0 12.96471898702334 0.9699043079148161
5.0 16.451722811563343 1.0039044196287459
5.0 20.87659468280201 1.1348138364464346
5.0 26.491584531418546 0.46343832203962254
5.0 33.616787682496685 0.821078035816349
5.0 42.65839262086404 0.8846459875171702
5.0 54.13183669370275 0.9318831504769416
5.0 68.69118979416318 0.9928885153880423
5.0 87.16644110999944 1.0891105054099535
5.0 110.6108145535225 1.2420282754048306
5.0 140.3608101970589 1.4399429785274336
5.0 178.11239451312218 1.5577375132219105
5.0 226.01768281801222 1.4723851369162775
5.0 286.807625522434 1.2797332575400033
5.0 363.94769219915764 0.8065054706734263
5.0 461.8354285936932 1.7939900488792277
5.0 586.0511487667402 1.5546480403114686
5.0 743.6760536467558 1.536194051948734
5.0 943.6959110675486 1.5585108258019733
5.0 1197.5133099937427 1.593699728878291
5.0 1519.5976911565988 1.6315568947623298
5.0 1928.3102105817359 1.6690889750533588
5.0 2446.9504592387466 1.7106982663646644
5.0 3105.0847094578075 1.772713989002807
5.0 3940.2314078349555 1.9003650092205158
5.0 5000.0 2.2602997753771015

6.344805015839611 5.0 0.9311237937998545
6.344805015839611 6.344805015839611 0.9335137947991391
6.344805015839611 8.051310137804697 0.9366628634801553
6.344805015839611 10.216798589284712 0.9409844789184443
6.344805015839611 12.96471898702334 0.9472081987920999
6.344805015839611 16.451722811563343 0.9567354431372296
6.344805015839611 20.87659468280201 0.972674197240357
6.344805015839611 26.491584531418546 1.0040644695385603
6.344805015839611 33.616787682496685 1.1021342048401608
6.344805015839611 42.65839262086404 0.5267518775362248
6.344805015839611 54.13183669370275 0.927285797079896
6.344805015839611 68.69118979416318 1.0346049885379813
6.344805015839611 87.16644110999944 1.16525793244315
6.344805015839611 110.6108145535225 1.3591254603361733
6.344805015839611 140.3608101970589 1.6035274093949017
6.344805015839611 178.11239451312218 1.7520063883997263
6.344805015839611 226.01768281801222 1.6761170724731824
6.344805015839611 286.807625522434 1.544578829493899
6.344805015839611 363.94769219915764 1.2883370509806118
6.344805015839611 461.8354285936932 1.341919502239284
6.344805015839611 586.0511487667402 1.3605097414361396
6.344805015839611 743.6760536467558 1.3912496656131155
6.344805015839611 943.6959110675486 1.4287165870793754
6.344805015839611 1197.5133099937427 1.4675655672676085
6.344805015839611 1519.5976911565988 1.5040830480569891
6.344805015839611 1928.3102105817359 1.5372987268795146
6.344805015839611 2446.9504592387466 1.5707713388816573
6.344805015839611 3105.0847094578075 1.6159239742759268
6.344805015839611 3940.2314078349555 1.70225818122788
6.344805015839611 5000.0 1.926361590934274

8.051310137804697 5.0 0.9282388896546284
8.051310137804697 6.344805015839611 0.9299208190890709
8.051310137804697 8.051310137804697 0.9320218770591421
8.051310137804697 10.216798589284712 0.9347223310635583
8.051310137804697 12.96471898702334 0.9382888677147728
8.051310137804697 16.451722811563343 0.9431112795671587
8.051310137804697 20.87659468280201 0.9497320061679936
8.051310137804697 26.491584531418546 0.9587742699156799
8.051310137804697 33.616787682496685 0.9703207509285031
8.051310137804697 42.65839262086404 0.9800543205650443
8.051310137804697 54.13183669370275 0.9449194771696514
8.051310137804697 68.69118979416318 3.7655756379828893
8.051310137804697 87.16644110999944 1.5856649902962014
8.051310137804697 110.6108145535225 1.7709653849905793
8.051310137804697 140.3608101970589 2.082155521301206
8.051310137804697 178.11239451312218 2.3089622515782295
8.051310137804697 226.01768281801222 2.4456005855577567
8.051310137804697 286.807625522434 1.711286579138651
8.051310137804697 363.94769219915764 1.0936183948966371
8.051310137804697 461.8354285936932 1.2155369904094846
8.051310137804697 586.0511487667402 1.26495574735163
8.051310137804697 743.6760536467558 1.306586200103397
8.051310137804697 943.6959110675486 1.3469923777713633
8.051310137804697 1197.5133099937427 1.3851331990741569
8.051310137804697 1519.5976911565988 1.4191723660741709
8.051310137804697 1928.3102105817359 1.4487338069054692
8.051310137804697 2446.9504592387466 1.4766296965506214
8.051310137804697 3105.0847094578075 1.5113074233612958
8.051310137804697 3940.2314078349555 1.5735550973973964
8.051310137804697 5000.0 1.7260021090133202

10.216798589284712 5.0 0.926222413064871
10.216798589284712 6.344805015839611 0.927537937049841
10.216798589284712 8.051310137804697 0.9291253543936783
10.216798589284712 10.216798589284712 0.9310866548622154
10.216798589284712 12.96471898702334 0.9335584268552103
10.216798589284712 16.451722811563343 0.9367095680867696
10.216798589284712 20.87659468280201 0.940702269487737
10.216798589284712 26.491584531418546 0.9455299409947547
10.216798589284712 33.616787682496685 0.9504578473268835
10.216798589284712 42.65839262086404 0.9521220828445148
10.216798589284712 54.13183669370275 0.9377282554823247
10.216798589284712 68.69118979416318 0.857205580672156
10.216798589284712 87.16644110999944 0.4732310515387462
10.216798589284712 110.6108145535225 2.27451516033424
10.216798589284712 140.3608101970589 16.37970538322737
10.216798589284712 178.11239451312218 13.628528047052637
10.216798589284712 226.01768281801222 2.661711421856711
10.216798589284712 286.807625522434 0.6839883970051449
10.216798589284712 363.94769219915764 1.0600406628234254
10.216798589284712 461.8354285936932 1.1572568505575576
10.216798589284712 586.0511487667402 1.2093035331842124
10.216798589284712 743.6760536467558 1.252288219286409
10.216798589284712 943.6959110675486 1.2920586573368695
10.216798589284712 1197.5133099937427 1.3283527368156678
10.216798589284712 1519.5976911565988 1.359933159902214
10.216798589284712 1928.3102105817359 1.3865776447372637
10.216798589284712 2446.9504592387466 1.4105152955835687
10.216798589284712 3105.0847094578075 1.4382615141845818
10.216798589284712 3940.2314078349555 1.4853035861217503
10.216798589284712 5000.0 1.5954737898212195

12.96471898702334 5.0 0.9247021527219313
12.96471898702334 6.344805015839611 0.925813619623796
12.96471898702334 8.051310137804697 0.9271245469530652
12.96471898702334 10.216798589284712 0.928703102322698
12.96471898702334 12.96471898702334 0.9306370308568152
12.96471898702334 16.451722811563343 0.9330253327261594
12.96471898702334 20.87659468280201 0.9359416318056321
12.96471898702334 26.491584531418546 0.9393161382194484
12.96471898702334 33.616787682496685 0.9425888774164963
12.96471898702334 42.65839262086404 0.9437328856509408
12.96471898702334 54.13183669370275 0.936535967153217
12.96471898702334 68.69118979416318 0.9030910184991655
12.96471898702334 87.16644110999944 0.794349031182063
12.96471898702334 110.6108145535225 0.4966101080551966
12.96471898702334 140.3608101970589 0.0813156136118813
12.96471898702334 178.11239451312218 0.3509060483670151
12.96471898702334 226.01768281801222 0.30811711396311553
12.96471898702334 286.807625522434 0.8508785968189597
12.96471898702334 363.94769219915764 1.0463492488508945
12.96471898702334 461.8354285936932 1.1243983485543534
12.96471898702334 586.0511487667402 1.1736525757651002
12.96471898702334 743.6760536467558 1.2153242809615359
12.96471898702334 943.6959110675486 1.2534635698850356
12.96471898702334 1197.5133099937427 1.2877810402970826
12.96471898702334 1519.5976911565988 1.3172266086498354
12.96471898702334 1928.3102105817359 1.3415860473544152
12.96471898702334 2446.9504592387466 1.3626449514480634
12.96471898702334 3105.0847094578075 1.3856020461158656
12.96471898702334 3940.2314078349555 1.4225032027977762
12.96471898702334 5000.0 1.5057992891305623

16.451722811563343 5.0 0.9235009223243977
16.451722811563343 6.344805015839611 0.9244896213659082
16.451722811563343 8.051310137804697 0.9256421826048981
16.451722811563343 10.216798589284712 0.9270089113487019
16.451722811563343 12.96471898702334 0.9286540927911514
16.451722811563343 16.451722811563343 0.9306483855551493
16.451722811563343 20.87659468280201 0.9330409554430383
16.451722811563343 26.491584531418546 0.9357750868836896
16.451722811563343 33.616787682496685 0.9384611926155667
16.451722811563343 42.65839262086404 0.9397924294738165
16.451722811563343 54.13183669370275 0.9360860060856987
16.451722811563343 68.69118979416318 0.9178248421044002
16.451722811563343 87.16644110999944 0.8626421445365923
16.451722811563343 110.6108145535225 0.7298432906816416
16.451722811563343 140.3608101970589 0.5104527414170363
16.451722811563343 178.11239451312218 0.4143563441772143
16.451722811563343 226.01768281801222 0.6496648866800803
16.451722811563343 286.807625522434 0.9106061313407556
16.451722811563343 363.94769219915764 1.039033062354694
16.451722811563343 461.8354285936932 1.103731339499322
16.451722811563343 586.0511487667402 1.1493769128334632
16.451722811563343 743.6760536467558 1.1890974026157015
16.451722811563343 943.6959110675486 1.225464091620342
16.451722811563343 1197.5133099937427 1.2579902105767666
16.451722811563343 1519.5976911565988 1.2856699177010122
16.451722811563343 1928.3102105817359 1.3082500622106255
16.451722811563343 2446.9504592387466 1.3271796109141987
16.451722811563343 3105.0847094578075 1.3467271577567481
16.451722811563343 3940.2314078349555 1.3765966356987303
16.451722811563343 5000.0 1.441894058871492

20.87659468280201 5.0 0.922547111903665
20.87659468280201 6.344805015839611 0.9234472978246608
20.87659468280201 8.051310137804697 0.924499481084809
20.87659468280201 10.216798589284712 0.9257415476238973
20.87659468280201 12.96471898702334 0.9272235917173682
20.87659468280201 16.451722811563343 0.9290020279668132
20.87659468280201 20.87659468280201 0.9311178640895174
20.87659468280201 26.491584531418546 0.9335354564318495
20.87659468280201 33.616787682496685 0.935985166773388
20.87659468280201 42.65839262086404 0.9375760007138662
20.87659468280201 54.13183669370275 0.9358867644427636
20.87659468280201 68.69118979416318 0.9249712388373039
20.87659468280201 87.16644110999944 0.8917714278205838
20.87659468280201 110.6108145535225 0.8148640179272344
20.87659468280201 140.3608101970589 0.694818896216012
20.87659468280201 178.11239451312218 0.6467587047000752
20.87659468280201 226.01768281801222 0.7790699090609
20.87659468280201 286.807625522434 0.9406261056238637
20.87659468280201 363.94769219915764 1.0345404116819616
20.87659468280201 461.8354285936932 1.0898021690082136
20.87659468280201 586.0511487667402 1.132121949336978
20.87659468280201 743.6760536467558 1.1699019193634308
20.87659468280201 943.6959110675486 1.2046357475949487
20.87659468280201 1197.5133099937427 1.23563282998092
20.87659468280201 1519.5976911565988 1.2618816126308805
20.87659468280201 1928.3102105817359 1.283078634786971
20.87659468280201 2446.9504592387466 1.3004154774377064
20.87659468280201 3105.0847094578075 1.3174853578106103
20.87659468280201 3940.2314078349555 1.342341494370401
20.87659468280201 5000.0 1.395122829122158

26.491584531418546 5.0 0.9218470138662102
26.491584531418546 6.344805015839611 0.9226555738490265
26.491584531418546 8.051310137804697 0.9236247238456452
26.491584531418546 10.216798589284712 0.9247810414391991
26.491584531418546 12.96471898702334 0.9261634222295558
26.491584531418546 16.451722811563343 0.9278181305996952
26.491584531418546 20.87659468280201 0.9297819390127869
26.491584531418546 26.491584531418546 0.932036369438611
26.491584531418546 33.616787682496685 0.9343924206875025
26.491584531418546 42.65839262086404 0.9362170322402703
26.491584531418546 54.13183669370275 0.9358147152504145
26.491584531418546 68.69118979416318 0.9291296322429906
26.491584531418546 87.16644110999944 0.9075783868416825
26.491584531418546 110.6108145535225 0.8579137246153759
26.491584531418546 140.3608101970589 0.7828172339354906
26.491584531418546 178.11239451312218 0.7567468781639118
26.491584531418546 226.01768281801222 0.8456600407817185
26.491584531418546 286.807625522434 0.9582566023351391
26.491584531418546 363.94769219915764 1.0315248916664477
26.491584531418546 461.8354285936932 1.0799442235277308
26.491584531418546 586.0511487667402 1.1194441137669586
26.491584531418546 743.6760536467558 1.1554889507101378
26.491584531418546 943.6959110675486 1.1888040179203172
26.491584531418546 1197.5133099937427 1.218527361277943
26.491584531418546 1519.5976911565988 1.2436264655976492
26.491584531418546 1928.3102105817359 1.26374876071619
26.491584531418546 2446.9504592387466 1.279887049393368
26.491584531418546 3105.0847094578075 1.295133067459863
26.491584531418546 3940.2314078349555 1.3163445837328127
26.491584531418546 5000.0 1.360181123087737

33.616787682496685 5.0 0.921483819105715
33.616787682496685 6.344805015839611 0.9221583783147496
33.616787682496685 8.051310137804697 0.9230243994108264
33.616787682496685 10.216798589284712 0.9240960831034378
33.616787682496685 12.96471898702334 0.9254006744057657
33.616787682496685 16.451722811563343 0.9269745516991075
33.616787682496685 20.87659468280201 0.9288495860973088
33.616787682496685 26.491584531418546 0.9310178121298196
33.616787682496685 33.616787682496685 0.9333437478084283
33.616787682496685 42.65839262086404 0.9353619960586813
33.616787682496685 54.13183669370275 0.9358303321464093
33.616787682496685 68.69118979416318 0.9318212713151611
33.616787682496685 87.16644110999944 0.9172833504813693
33.616787682496685 110.6108145535225 0.88329303564207
33.616787682496685 140.3608101970589 0.8331304676656648
33.616787682496685 178.11239451312218 0.8194095320126747
33.616787682496685 226.01768281801222 0.8852942461798062
33.616787682496685 286.807625522434 0.9695559471281461
33.616787682496685 363.94769219915764 1.0293582831181582
33.616787682496685 461.8354285936932 1.0726919183477184
33.616787682496685 586.0511487667402 1.1098590328210995
33.616787682496685 743.6760536467558 1.14440808732329
33.616787682496685 943.6959110675486 1.176515729696907
33.616787682496685 1197.5133099937427 1.2051860277384054
33.616787682496685 1519.5976911565988 1.2293632493274458
33.616787682496685 1928.3102105817359 1.2486510074396218
33.616787682496685 2446.9504592387466 1.2638865374979649
33.616787682496685 3105.0847094578075 1.277782054684209
33.616787682496685 3940.2314078349555 1.2963106822889132
33.616787682496685 5000.0 1.3336276294350595

42.65839262086404 5.0 0.9216282244729951
42.65839262086404 6.344805015839611 0.9220801111347507
42.65839262086404 8.051310137804697 0.9227806823876111
42.65839262086404 10.216798589284712 0.9237296415171876
42.65839262086404 12.96471898702334 0.9249407253625143
42.65839262086404 16.451722811563343 0.9264383428092471
42.65839262086404 20.87659468280201 0.9282467094616886
42.65839262086404 26.491584531418546 0.9303614549517134
42.65839262086404 33.616787682496685 0.9326808548660677
42.65839262086404 42.65839262086404 0.9348500696597164
42.65839262086404 54.13183669370275 0.9359242172758542
42.65839262086404 68.69118979416318 0.9336994186408296
42.65839262086404 87.16644110999944 0.9236976768621327
42.65839262086404 110.6108145535225 0.8995859370967805
42.65839262086404 140.3608101970589 0.8648594193988112
42.65839262086404 178.11239451312218 0.8588997399102395
42.65839262086404 226.01768281801222 0.9109392805968537
42.65839262086404 286.807625522434 0.9771929624669826
42.65839262086404 363.94769219915764 1.0277019284793871
42.65839262086404 461.8354285936932 1.0671657716490661
42.65839262086404 586.0511487667402 1.1024055134429425
42.65839262086404 743.6760536467558 1.1356748081499164
42.65839262086404 943.6959110675486 1.1667562684680453
42.65839262086404 1197.5133099937427 1.194553108918918
42.65839262086404 1519.5976911565988 1.2179891112732082
42.65839262086404 1928.3102105817359 1.2366300252528422
42.65839262086404 2446.9504592387466 1.2511894248666966
42.65839262086404 3105.0847094578075 1.264086957365069
42.65839262086404 3940.2314078349555 1.2806289956729744
42.65839262086404 5000.0 1.313129617601872

54.13183669370275 5.0 0.9225496011301068
54.13183669370275 6.344805015839611 0.9226370722313696
54.13183669370275 8.051310137804697 0.923059982484639
54.13183669370275 10.216798589284712 0.9238022889917474
54.13183669370275 12.96471898702334 0.9248619329256598
54.13183669370275 16.451722811563343 0.9262486198100632
54.13183669370275 20.87659468280201 0.9279750101173112
54.13183669370275 26.491584531418546 0.9300333535862543
54.13183669370275 33.616787682496685 0.9323400406463455
54.13183669370275 42.65839262086404 0.9346120157128929
54.13183669370275 54.13183669370275 0.936103605587514
54.13183669370275 68.69118979416318 0.9350938902261705
54.13183669370275 87.16644110999944 0.9281403876782539
54.13183669370275 110.6108145535225 0.9105892021907485
54.13183669370275 140.3608101970589 0.8860746635408555
54.13183669370275 178.11239451312218 0.8853665847800279
54.13183669370275 226.01768281801222 0.9284265429624476
54.13183669370275 286.807625522434 0.9825230153323268
54.13183669370275 363.94769219915764 1.0263503572656882
54.13183669370275 461.8354285936932 1.0627977842191842
54.13183669370275 586.0511487667402 1.0964256372530479
54.13183669370275 743.6760536467558 1.1285892672137738
54.13183669370275 943.6959110675486 1.1587877595399452
54.13183669370275 1197.5133099937427 1.1858510415310575
54.13183669370275 1519.5976911565988 1.208686815185599
54.13183669370275 1928.3102105817359 1.2268284004874714
54.13183669370275 2446.9504592387466 1.2408889555820304
54.13183669370275 3105.0847094578075 1.2530582611368755
54.13183669370275 3940.2314078349555 1.2681317868514617
54.13183669370275 5000.0 1.297046410771583

68.69118979416318 5.0 0.9246089293032224
68.69118979416318 6.344805015839611 0.9241402331393551
68.69118979416318 8.051310137804697 0.924120232538515
68.69118979416318 10.216798589284712 0.924519599201396
68.69118979416318 12.96471898702334 0.9253203875099105
68.69118979416318 16.451722811563343 0.9265155954798817
68.69118979416318 20.87659468280201 0.9281024597090967
68.69118979416318 26.491584531418546 0.9300633042260662
68.69118979416318 33.616787682496685 0.932319817238907
68.69118979416318 42.65839262086404 0.9346320783335619
68.69118979416318 54.13183669370275 0.936386833622603
68.69118979416318 68.69118979416318 0.9361912628508455
68.69118979416318 87.16644110999944 0.9313059464915325
68.69118979416318 110.6108145535225 0.9182265122913035
68.69118979416318 140.3608101970589 0.9007644765963324
68.69118979416318 178.11239451312218 0.9038216783056697
68.69118979416318 226.01768281801222 0.9407675444316176
68.69118979416318 286.807625522434 0.9863025972638303
68.69118979416318 363.94769219915764 1.0251633459368623
68.69118979416318 461.8354285936932 1.059195841746944
68.69118979416318 586.0511487667402 1.0914442021617297
68.69118979416318 743.6760536467558 1.122630778807314
68.69118979416318 943.6959110675486 1.1520512645188665
68.69118979416318 1197.5133099937427 1.1784850550829318
68.69118979416318 1519.5976911565988 1.200828777855326
68.69118979416318 1928.3102105817359 1.2185877410254458
68.69118979416318 2446.9504592387466 1.232291483175486
68.69118979416318 3105.0847094578075 1.243945128526915
68.69118979416318 3940.2314078349555 1.257945982643008
68.69118979416318 5000.0 1.2841855659161723

87.16644110999944 5.0 0.9282032826722353
87.16644110999944 6.344805015839611 0.9269642401699455
87.16644110999944 8.051310137804697 0.926296340461256
87.16644110999944 10.216798589284712 0.9261674509965855
87.16644110999944 12.96471898702334 0.9265494097221401
87.16644110999944 16.451722811563343 0.9274202013038174
87.16644110999944 20.87659468280201 0.9287601437638945
87.16644110999944 26.491584531418546 0.9305366464529958
87.16644110999944 33.616787682496685 0.9326662386786235
87.16644110999944 42.65839262086404 0.9349303530018028
87.16644110999944 54.13183669370275 0.9368000676671706
87.16644110999944 68.69118979416318 0.9371031489631162
87.16644110999944 87.16644110999944 0.933582434188935
87.16644110999944 110.6108145535225 0.9235561478347818
87.16644110999944 140.3608101970589 0.9111146156069019
87.16644110999944 178.11239451312218 0.9170281027362949
87.16644110999944 226.01768281801222 0.949674682966713
87.16644110999944 286.807625522434 0.9889801642479863
87.16644110999944 363.94769219915764 1.024032631868173
87.16644110999944 461.8354285936932 1.0560695040591817
87.16644110999944 586.0511487667402 1.0870988028608957
87.16644110999944 743.6760536467558 1.1173927759256428
87.16644110999944 943.6959110675486 1.1461042270046833
87.16644110999944 1197.5133099937427 1.1719811236077726
87.16644110999944 1519.5976911565988 1.1939139394224227
87.16644110999944 1928.3102105817359 1.2113835047654282
87.16644110999944 2446.9504592387466 1.2248474278470283
87.16644110999944 3105.0847094578075 1.2361584705081938
87.16644110999944 3940.2314078349555 1.249397774377177
87.16644110999944 5000.0 1.2736527576255425

110.6108145535225 5.0 0.9336261932958563
110.6108145535225 6.344805015839611 0.9314461396567674
110.6108145535225 8.051310137804697 0.9299309153260049
110.6108145535225 10.216798589284712 0.9290666734154507
110.6108145535225 12.96471898702334 0.9288303539654649
110.6108145535225 16.451722811563343 0.9291945637581196
110.6108145535225 20.87659468280201 0.9301270226773263
110.6108145535225 26.491584531418546 0.9315796289298474
110.6108145535225 33.616787682496685 0.9334573453378124
110.6108145535225 42.65839262086404 0.9355469601658116
110.6108145535225 54.13183669370275 0.9373679070945953
110.6108145535225 68.69118979416318 0.9378899854682394
110.6108145535225 87.16644110999944 0.9351812979347979
110.6108145535225 110.6108145535225 0.9271787497762126
110.6108145535225 140.3608101970589 0.9184143527997919
110.6108145535225 178.11239451312218 0.9266427711299244
110.6108145535225 226.01768281801222 0.9561930816928983
110.6108145535225 286.807625522434 0.9908281742664503
110.6108145535225 363.94769219915764 1.0228622166560426
110.6108145535225 461.8354285936932 1.0531868091677419
110.6108145535225 586.0511487667402 1.083095241820774
110.6108145535225 743.6760536467558 1.112540522274455
110.6108145535225 943.6959110675486 1.1405790306862873
110.6108145535225 1197.5133099937427 1.165943828190198
110.6108145535225 1519.5976911565988 1.1875244779870355
110.6108145535225 1928.3102105817359 1.2047800120285785
110.6108145535225 2446.9504592387466 1.218103749603193
110.6108145535225 3105.0847094578075 1.2292185453688305
110.6108145535225 3940.2314078349555 1.2419487694844575
110.6108145535225 5000.0 1.2647549992824236

140.3608101970589 5.0 0.9408291640215901
140.3608101970589 6.344805015839611 0.9376813898324013
140.3608101970589 8.051310137804697 0.9352095837634407
140.3608101970589 10.216798589284712 0.9334456267037337
140.3608101970589 12.96471898702334 0.9323965941132463
140.3608101970589 16.451722811563343 0.9320498378313539
140.3608101970589 20.87659468280201 0.9323746805510628
140.3608101970589 26.491584531418546 0.933315369525455
140.3608101970589 33.616787682496685 0.9347661440322973
140.3608101970589 42.65839262086404 0.9365104272615672
140.3608101970589 54.13183669370275 0.9380900575350438
140.3608101970589 68.69118979416318 0.9385565684232736
140.3608101970589 87.16644110999944 0.936186083751013
140.3608101970589 110.6108145535225 0.929420284680187
140.3608101970589 140.3608101970589 0.9234758474011353
140.3608101970589 178.11239451312218 0.9337370800753126
140.3608101970589 226.01768281801222 0.9609950268625593
140.3608101970589 286.807625522434 0.99200751292945
140.3608101970589 363.94769219915764 1.0215552810076336
140.3608101970589 461.8354285936932 1.0503462053846606
140.3608101970589 586.0511487667402 1.0791788186794549
140.3608101970589 743.6760536467558 1.1077821954481943
140.3608101970589 943.6959110675486 1.1351537609541236
140.3608101970589 1197.5133099937427 1.1600267917315419
140.3608101970589 1519.5976911565988 1.18129527881145
140.3608101970589 1928.3102105817359 1.1983985222542994
140.3608101970589 2446.9504592387466 1.2116701107095595
140.3608101970589 3105.0847094578075 1.222717768168714
140.3608101970589 3940.2314078349555 1.2351514366997274
140.3608101970589 5000.0 1.2569358295635829

178.11239451312218 5.0 0.949139555146959
178.11239451312218 6.344805015839611 0.9452315174549442
178.11239451312218 8.051310137804697 0.9418859157264007
178.11239451312218 10.216798589284712 0.9391982375570656
178.11239451312218 12.96471898702334 0.9372305715831719
178.11239451312218 16.451722811563343 0.9360115866057002
178.11239451312218 20.87659468280201 0.9355362999429679
178.11239451312218 26.491584531418546 0.9357602175337972
178.11239451312218 33.616787682496685 0.9365784979544156
178.11239451312218 42.65839262086404 0.9377725241248194
178.11239451312218 54.13183669370275 0.9388909700209407
178.11239451312218 68.69118979416318 0.9390207747999865
178.11239451312218 87.16644110999944 0.9365567928348155
178.11239451312218 110.6108145535225 0.9304231379084403
178.11239451312218 140.3608101970589 0.9268695028623248
178.11239451312218 178.11239451312218 0.9390632624563322
178.11239451312218 226.01768281801222 0.9645257365941602
178.11239451312218 286.807625522434 0.9925988668892789
178.11239451312218 363.94769219915764 1.020003867573007
178.11239451312218 461.8354285936932 1.047357279972816
178.11239451312218 586.0511487667402 1.0751132347614099
178.11239451312218 743.6760536467558 1.1028481555969787
178.11239451312218 943.6959110675486 1.1295316133163429
178.11239451312218 1197.5133099937427 1.1539113564220227
178.11239451312218 1519.5976911565988 1.1748917056556014
178.11239451312218 1928.3102105817359 1.1918940390379356
178.11239451312218 2446.9504592387466 1.2051942890658618
178.11239451312218 3105.0847094578075 1.2162937285619593
178.11239451312218 3940.2314078349555 1.2286171264777914
178.11239451312218 5000.0 1.249730089863909

226.01768281801222 5.0 0.9571020468713766
226.01768281801222 6.344805015839611 0.9528769533562662
226.01768281801222 8.051310137804697 0.9489868360746941
226.01768281801222 10.216798589284712 0.9455795365430817
226.01768281801222 12.96471898702334 0.9427774296497574
226.01768281801222 16.451722811563343 0.940668053044928
226.01768281801222 20.87659468280201 0.9392963708833137
226.01768281801222 26.491584531418546 0.9386544894169327
226.01768281801222 33.616787682496685 0.9386598691337155
226.01768281801222 42.65839262086404 0.9391043298439545
226.01768281801222 54.13183669370275 0.9395398517898041
226.01768281801222 68.69118979416318 0.9390572304292051
226.01768281801222 87.16644110999944 0.9361098986432604
226.01768281801222 110.6108145535225 0.9302168087542545
226.01768281801222 140.3608101970589 0.9291015776085698
226.01768281801222 178.11239451312218 0.9431951508611471
226.01768281801222 226.01768281801222 0.9670733357281364
226.01768281801222 286.807625522434 0.992615566994737
226.01768281801222 363.94769219915764 1.0180801220237072
226.01768281801222 461.8354285936932 1.0440265595301865
226.01768281801222 586.0511487667402 1.0706658828090905
226.01768281801222 743.6760536467558 1.0974762561187674
226.01768281801222 943.6959110675486 1.1234259945303136
226.01768281801222 1197.5133099937427 1.1472914280787656
226.01768281801222 1519.5976911565988 1.1679938292767067
226.01768281801222 1928.3102105817359 1.1849385567626947
226.01768281801222 2446.9504592387466 1.1983441359273777
226.01768281801222 3105.0847094578075 1.2096093245998212
226.01768281801222 3940.2314078349555 1.221992655482457
226.01768281801222 5000.0 1.242731588865623

286.807625522434 5.0 0.9627113926425924
286.807625522434 6.344805015839611 0.9587145396592286
286.807625522434 8.051310137804697 0.954788806520949
286.807625522434 10.216798589284712 0.9510924009021857
286.807625522434 12.96471898702334 0.947780504750461
286.807625522434 16.451722811563343 0.9449890455260148
286.807625522434 20.87659468280201 0.9428179320745422
286.807625522434 26.491584531418546 0.9413118152222351
286.807625522434 33.616787682496685 0.9404312925014562
286.807625522434 42.65839262086404 0.9399976004118138
286.807625522434 54.13183669370275 0.9395756777827022
286.807625522434 68.69118979416318 0.9382487295304405
286.807625522434 87.16644110999944 0.9345132744885144
286.807625522434 110.6108145535225 0.9288513585907646
286.807625522434 140.3608101970589 0.9307800673749008
286.807625522434 178.11239451312218 0.9465766206473865
286.807625522434 226.01768281801222 0.9687926761563401
286.807625522434 286.807625522434 0.9920070031632807
286.807625522434 363.94769219915764 1.0156287686241516
286.807625522434 461.8354285936932 1.040147213264274
286.807625522434 586.0511487667402 1.0655974699249051
286.807625522434 743.6760536467558 1.0914017910048746
286.807625522434 943.6959110675486 1.1165508766370436
286.807625522434 1197.5133099937427 1.1398637082229346
286.807625522434 1519.5976911565988 1.1602861319309243
286.807625522434 1928.3102105817359 1.1772098335587233
286.807625522434 2446.9504592387466 1.1907951669540686
286.807625522434 3105.0847094578075 1.2023385809585472
286.807625522434 3940.2314078349555 1.214943213498938
286.807625522434 5000.0 1.2355697661738105

363.94769219915764 5.0 0.9641740465889364
363.94769219915764 6.344805015839611 0.9608403996750365
363.94769219915764 8.051310137804697 0.9573746363684394
363.94769219915764 10.216798589284712 0.953899309840518
363.94769219915764 12.96471898702334 0.950555388713414
363.94769219915764 16.451722811563343 0.9474876661716957
363.94769219915764 20.87659468280201 0.9448249920709694
363.94769219915764 26.491584531418546 0.942654473397699
363.94769219915764 33.616787682496685 0.9409845121338432
363.94769219915764 42.65839262086404 0.9396813043232647
363.94769219915764 54.13183669370275 0.9383407086137371
363.94769219915764 68.69118979416318 0.9360394346106283
363.94769219915764 87.16644110999944 0.9313791585739439
363.94769219915764 110.6108145535225 0.9267364851907345
363.94769219915764 140.3608101970589 0.9326906110832193
363.94769219915764 178.11239451312218 0.9494691252995451
363.94769219915764 226.01768281801222 0.9697023649789597
363.94769219915764 286.807625522434 0.990658184056696
363.94769219915764 363.94769219915764 1.0124622456208434
363.94769219915764 461.8354285936932 1.0354929222476426
363.94769219915764 586.0511487667402 1.0596561662087476
363.94769219915764 743.6760536467558 1.0843525965753493
363.94769219915764 943.6959110675486 1.1086164759966421
363.94769219915764 1197.5133099937427 1.1313234924376343
363.94769219915764 1519.5976911565988 1.1514527703808815
363.94769219915764 1928.3102105817359 1.1683857190283877
363.94769219915764 2446.9504592387466 1.182223400679797
363.94769219915764 3105.0847094578075 1.1941576886447047
363.94769219915764 3940.2314078349555 1.207140804130511
363.94769219915764 5000.0 1.227893161436437

461.8354285936932 5.0 0.9607021955070723
461.8354285936932 6.344805015839611 0.9582074871506554
461.8354285936932 8.051310137804697 0.9554862157795107
461.8354285936932 10.216798589284712 0.9526056281104329
461.8354285936932 12.96471898702334 0.9496591144443782
461.8354285936932 16.451722811563343 0.946759257934224
461.8354285936932 20.87659468280201 0.9440234660952385
461.8354285936932 26.491584531418546 0.9415499526948948
461.8354285936932 33.616787682496685 0.9393778788654077
461.8354285936932 42.65839262086404 0.937413120891468
461.8354285936932 54.13183669370275 0.9352669882268284
461.8354285936932 68.69118979416318 0.9319477671202183
461.8354285936932 87.16644110999944 0.926577927473834
461.8354285936932 110.6108145535225 0.9252963582444477
461.8354285936932 140.3608101970589 0.9355024533874634
461.8354285936932 178.11239451312218 0.9518248834879465
461.8354285936932 226.01768281801222 0.9696791052813487
461.8354285936932 286.807625522434 0.9883918994803671
461.8354285936932 363.94769219915764 1.0083601650730376
461.8354285936932 461.8354285936932 1.029817067109122
461.8354285936932 586.0511487667402 1.0525777438259163
461.8354285936932 743.6760536467558 1.0760502580647682
461.8354285936932 943.6959110675486 1.0993312590168074
461.8354285936932 1197.5133099937427 1.1213669529176837
461.8354285936932 1519.5976911565988 1.1411794797119024
461.8354285936932 1928.3102105817359 1.1581448153651457
461.8354285936932 2446.9504592387466 1.1723043467529077
461.8354285936932 3105.0847094578075 1.1847416880418722
461.8354285936932 3940.2314078349555 1.1982581544634554
461.8354285936932 5000.0 1.2193591951667195

586.0511487667402 5.0 0.9528208004145579
586.0511487667402 6.344805015839611 0.9511139114749737
586.0511487667402 8.051310137804697 0.9491815791085851
586.0511487667402 10.216798589284712 0.9470471067680221
586.0511487667402 12.96471898702334 0.9447552835866649
586.0511487667402 16.451722811563343 0.9423717473911508
586.0511487667402 20.87659468280201 0.9399754123884344
586.0511487667402 26.491584531418546 0.9376383071304776
586.0511487667402 33.616787682496685 0.935379823532344
586.0511487667402 42.65839262086404 0.9330593863073775
586.0511487667402 54.13183669370275 0.9301253407458948
586.0511487667402 68.69118979416318 0.9255029254837894
586.0511487667402 87.16644110999944 0.9217019558155575
586.0511487667402 110.6108145535225 0.9268879562519977
586.0511487667402 140.3608101970589 0.9389706234815002
586.0511487667402 178.11239451312218 0.9532264064666923
586.0511487667402 226.01768281801222 0.9684784254489257
586.0511487667402 286.807625522434 0.9849782818151824
586.0511487667402 363.94769219915764 1.0030748846027648
586.0511487667402 461.8354285936932 1.0228589242989814
586.0511487667402 586.0511487667402 1.0440933220968691
586.0511487667402 743.6760536467558 1.0662191858529335
586.0511487667402 943.6959110675486 1.0884119767939353
586.0511487667402 1197.5133099937427 1.1097013803744247
586.0511487667402 1519.5976911565988 1.1291632215021203
586.0511487667402 1928.3102105817359 1.1461748035279997
586.0511487667402 2446.9504592387466 1.1607190721716856
586.0511487667402 3105.0847094578075 1.1737678925651576
586.0511487667402 3940.2314078349555 1.1879688804805144
586.0511487667402 5000.0 1.2096303011202414

743.6760536467558 5.0 0.9428997741477151
743.6760536467558 6.344805015839611 0.9418220768835242
743.6760536467558 8.051310137804697 0.9405673129824836
743.6760536467558 10.216798589284712 0.9391331876308308
743.6760536467558 12.96471898702334 0.9375271672489986
743.6760536467558 16.451722811563343 0.935764559573507
743.6760536467558 20.87659468280201 0.9338570979982543
743.6760536467558 26.491584531418546 0.9317783780289021
743.6760536467558 33.616787682496685 0.9293730862307972
743.6760536467558 42.65839262086404 0.9261649700496122
743.6760536467558 54.13183669370275 0.9215922280734945
743.6760536467558 68.69118979416318 0.918718618492501
743.6760536467558 87.16644110999944 0.9226607053406861
743.6760536467558 110.6108145535225 0.9312538125000597
743.6760536467558 140.3608101970589 0.9416159563678818
743.6760536467558 178.11239451312218 0.9530557879559551
743.6760536467558 226.01768281801222 0.9657905764337039
743.6760536467558 286.807625522434 0.9801531788059499
743.6760536467558 363.94769219915764 0.996344582427234
743.6760536467558 461.8354285936932 1.0143584652696584
743.6760536467558 586.0511487667402 1.0339463696052527
743.6760536467558 743.6760536467558 1.054605228682612
743.6760536467558 943.6959110675486 1.0756031002693676
743.6760536467558 1197.5133099937427 1.0960648144688894
743.6760536467558 1519.5976911565988 1.1151311470933885
743.6760536467558 1928.3102105817359 1.132189691410963
743.6760536467558 2446.9504592387466 1.1471689629897899
743.6760536467558 3105.0847094578075 1.160927301223367
743.6760536467558 3940.2314078349555 1.1759551976814426
743.6760536467558 5000.0 1.1983774395847961

943.6959110675486 5.0 0.9330455565030262
943.6959110675486 6.344805015839611 0.9322772905983372
943.6959110675486 8.051310137804697 0.9313330547494534
943.6959110675486 10.216798589284712 0.9301698882463293
943.6959110675486 12.96471898702334 0.9287224348146808
943.6959110675486 16.451722811563343 0.9268800565190703
943.6959110675486 20.87659468280201 0.9244576551294785
943.6959110675486 26.491584531418546 0.9216744242449386
943.6959110675486 33.616787682496685 0.9178951599035888
943.6959110675486 42.65839262086404 0.9163857901750563
943.6959110675486 54.13183669370275 0.9181053405226642
943.6959110675486 68.69118979416318 0.922261926815417
943.6959110675486 87.16644110999944 0.9277953716558098
943.6959110675486 110.6108145535225 0.9343076439445313
943.6959110675486 140.3608101970589 0.9418833969213835
943.6959110675486 178.11239451312218 0.9507886834337625
943.6959110675486 226.01768281801222 0.9613030746623243
943.6959110675486 286.807625522434 0.9736424376490741
943.6959110675486 363.94769219915764 0.9879144876301286
943.6959110675486 461.8354285936932 1.0040806233206236
943.6959110675486 586.0511487667402 1.0219198525526731
943.6959110675486 743.6760536467558 1.0410044881253953
943.6959110675486 943.6959110675486 1.06070633121157
943.6959110675486 1197.5133099937427 1.0802554707115626
943.6959110675486 1519.5976911565988 1.0988691848278944
943.6959110675486 1928.3102105817359 1.1159567390948946
943.6959110675486 2446.9504592387466 1.1313999444558553
943.6959110675486 3105.0847094578075 1.1459452368304759
943.6959110675486 3940.2314078349555 1.1619243350336943
943.6959110675486 5000.0 1.1852924701086207

1197.5133099937427 5.0 0.9172083058417273
1197.5133099937427 6.344805015839611 0.916949051079451
1197.5133099937427 8.051310137804697 0.9167414872872689
1197.5133099937427 10.216798589284712 0.9166367733241123
1197.5133099937427 12.96471898702334 0.9166952505673884
1197.5133099937427 16.451722811563343 0.916977738959098
1197.5133099937427 20.87659468280201 0.9175355642216381
1197.5133099937427 26.491584531418546 0.9184059138689425
1197.5133099937427 33.616787682496685 0.9196185868029155
1197.5133099937427 42.65839262086404 0.9212140871793982
1197.5133099937427 54.13183669370275 0.9232654116556193
1197.5133099937427 68.69118979416318 0.9258933224747841
1197.5133099937427 87.16644110999944 0.9292691512014031
1197.5133099937427 110.6108145535225 0.9336055845412309
1197.5133099937427 140.3608101970589 0.9391394683873161
1197.5133099937427 178.11239451312218 0.9461104591667396
1197.5133099937427 226.01768281801222 0.9547373121722048
1197.5133099937427 286.807625522434 0.9651916094510283
1197.5133099937427 363.94769219915764 0.9775677655122619
1197.5133099937427 461.8354285936932 0.9918490248596926
1197.5133099937427 586.0511487667402 1.0078723480457776
1197.5133099937427 743.6760536467558 1.0253007288081695
1197.5133099937427 943.6959110675486 1.0436183981402471
1197.5133099937427 1197.5133099937427 1.0621693395512775
1197.5133099937427 1519.5976911565988 1.0802589930689037
1197.5133099937427 1928.3102105817359 1.0973320609508088
1197.5133099937427 2446.9504592387466 1.1132357103974728
1197.5133099937427 3105.0847094578075 1.1286112837165958
1197.5133099937427 3940.2314078349555 1.1456343954161252
1197.5133099937427 5000.0 1.170110225465559

1519.5976911565988 5.0 0.9193302242407798
1519.5976911565988 6.344805015839611 0.9193232933508088
1519.5976911565988 8.051310137804697 0.9193244080315669
1519.5976911565988 10.216798589284712 0.9193410043402904
1519.5976911565988 12.96471898702334 0.9193850395805407
1519.5976911565988 16.451722811563343 0.9194751679251031
1519.5976911565988 20.87659468280201 0.9196396552468263
1519.5976911565988 26.491584531418546 0.91992008612511
1519.5976911565988 33.616787682496685 0.920375750749497
1519.5976911565988 42.65839262086404 0.9210883507886694
1519.5976911565988 54.13183669370275 0.9221663585031353
1519.5976911565988 68.69118979416318 0.9237480369956731
1519.5976911565988 87.16644110999944 0.9260019719497045
1519.5976911565988 110.6108145535225 0.9291240007376891
1519.5976911565988 140.3608101970589 0.9333297255673237
1519.5976911565988 178.11239451312218 0.9388422155897713
1519.5976911565988 226.01768281801222 0.9458748398451278
1519.5976911565988 286.807625522434 0.9546092979521753
1519.5976911565988 363.94769219915764 0.9651689564248127
1519.5976911565988 461.8354285936932 0.9775880949893068
1519.5976911565988 586.0511487667402 0.9917794899753415
1519.5976911565988 743.6760536467558 1.0075065414663353
1519.5976911565988 943.6959110675486 1.0243720071230118
1519.5976911565988 1197.5133099937427 1.0418409777873736
1519.5976911565988 1519.5976911565988 1.059318603543161
1519.5976911565988 1928.3102105817359 1.0763008429736687
1519.5976911565988 2446.9504592387466 1.0926169406634794
1519.5976911565988 3105.0847094578075 1.1088163369125053
1519.5976911565988 3940.2314078349555 1.1269285279492152
1519.5976911565988 5000.0 1.1526408734920948

1928.3102105817359 5.0 0.9139553563691344
1928.3102105817359 6.344805015839611 0.913946254789337
1928.3102105817359 8.051310137804697 0.9139419822090603
1928.3102105817359 10.216798589284712 0.9139477499855827
1928.3102105817359 12.96471898702334 0.9139720794626868
1928.3102105817359 16.451722811563343 0.9140284543253944
1928.3102105817359 20.87659468280201 0.9141375849301737
1928.3102105817359 26.491584531418546 0.9143303638497581
1928.3102105817359 33.616787682496685 0.914651521772363
1928.3102105817359 42.65839262086404 0.9151638192966483
1928.3102105817359 54.13183669370275 0.9159523967123256
1928.3102105817359 68.69118979416318 0.9171286239593194
1928.3102105817359 87.16644110999944 0.9188325355411959
1928.3102105817359 110.6108145535225 0.921232762417184
1928.3102105817359 140.3608101970589 0.9245228613774615
1928.3102105817359 178.11239451312218 0.9289131077815757
1928.3102105817359 226.01768281801222 0.9346171440195543
1928.3102105817359 286.807625522434 0.9418332343165158
1928.3102105817359 363.94769219915764 0.9507203141059181
1928.3102105817359 461.8354285936932 0.9613696139554971
1928.3102105817359 586.0511487667402 0.9737740073751188
1928.3102105817359 743.6760536467558 0.9877998976792729
1928.3102105817359 943.6959110675486 1.0031709689215642
1928.3102105817359 1197.5133099937427 1.0194785860105353
1928.3102105817359 1519.5976911565988 1.0362383878319583
1928.3102105817359 1928.3102105817359 1.0530147187531929
1928.3102105817359 2446.9504592387466 1.069639810644534
1928.3102105817359 3105.0847094578075 1.0865915104476318
1928.3102105817359 3940.2314078349555 1.1057733974705541
1928.3102105817359 5000.0 1.1328107891804051

2446.9504592387466 5.0 0.9039148268892869
2446.9504592387466 6.344805015839611 0.9039358304079825
2446.9504592387466 8.051310137804697 0.9039663461167744
2446.9504592387466 10.216798589284712 0.9040110713758485
2446.9504592387466 12.96471898702334 0.9040770583258974
2446.9504592387466 16.451722811563343 0.9041748401474525
2446.9504592387466 20.87659468280201 0.9043199975549077
2446.9504592387466 26.491584531418546 0.9045352885733148
2446.9504592387466 33.616787682496685 0.9048534202206728
2446.9504592387466 42.65839262086404 0.9053204610750983
2446.9504592387466 54.13183669370275 0.9059997765740967
2446.9504592387466 68.69118979416318 0.9069761180471899
2446.9504592387466 87.16644110999944 0.9083592524965075
2446.9504592387466 110.6108145535225 0.9102862486379895
2446.9504592387466 140.3608101970589 0.9129212882644299
2446.9504592387466 178.11239451312218 0.9164518069691469
2446.9504592387466 226.01768281801222 0.9210798934607498
2446.9504592387466 286.807625522434 0.9270081478565197
2446.9504592387466 363.94769219915764 0.9344197406111426
2446.9504592387466 461.8354285936932 0.9434532118954632
2446.9504592387466 586.0511487667402 0.9541737332981095
2446.9504592387466 743.6760536467558 0.9665447920850601
2446.9504592387466 943.6959110675486 0.9804077312537244
2446.9504592387466 1197.5133099937427 0.9954815373874597
2446.9504592387466 1519.5976911565988 1.0114007961274343
2446.9504592387466 1928.3102105817359 1.027815115244451
2446.9504592387466 2446.9504592387466 1.044583536659082
2446.9504592387466 3105.0847094578075 1.0621396260996068
2446.9504592387466 3940.2314078349555 1.0822945623577214
2446.9504592387466 5000.0 1.110708920193223

3105.0847094578075 5.0 0.8910019352651007
3105.0847094578075 6.344805015839611 0.8910434056857996
3105.0847094578075 8.051310137804697 0.8910979522647504
3105.0847094578075 10.216798589284712 0.8911701788492601
3105.0847094578075 12.96471898702334 0.8912665070926391
3105.0847094578075 16.451722811563343 0.8913959414903999
3105.0847094578075 20.87659468280201 0.8915711536082587
3105.0847094578075 26.491584531418546 0.891809952704392
3105.0847094578075 33.616787682496685 0.8921372780796683
3105.0847094578075 42.65839262086404 0.892587766749805
3105.0847094578075 54.13183669370275 0.8932089027368552
3105.0847094578075 68.69118979416318 0.8940646518708704
3105.0847094578075 87.16644110999944 0.8952392554885191
3105.0847094578075 110.6108145535225 0.8968405812859771
3105.0847094578075 140.3608101970589 0.8990022161636626
3105.0847094578075 178.11239451312218 0.9018831297092387
3105.0847094578075 226.01768281801222 0.9056636831046159
3105.0847094578075 286.807625522434 0.9105367860750944
3105.0847094578075 363.94769219915764 0.9166933420704249
3105.0847094578075 461.8354285936932 0.9243018703802133
3105.0847094578075 586.0511487667402 0.9334832622706668
3105.0847094578075 743.6760536467558 0.9442836744456964
3105.0847094578075 943.6959110675486 0.9566514147380599
3105.0847094578075 1197.5133099937427 0.9704282792003783
3105.0847094578075 1519.5976911565988 0.9853714858602844
3105.0847094578075 1928.3102105817359 1.0012300749940468
3105.0847094578075 2446.9504592387466 1.0179143870334217
3105.0847094578075 3105.0847094578075 1.0358469935719397
3105.0847094578075 3940.2314078349555 1.056797812298369
3105.0847094578075 5000.0 1.086637331986594

3940.2314078349555 5.0 0.8763504639358031
3940.2314078349555 6.344805015839611 0.8764018152284756
3940.2314078349555 8.051310137804697 0.8764679019723878
3940.2314078349555 10.216798589284712 0.8765532187135395
3940.2314078349555 12.96471898702334 0.8766637596643236
3940.2314078349555 16.451722811563343 0.8768075716082896
3940.2314078349555 20.87659468280201 0.8769955148128091
3940.2314078349555 26.491584531418546 0.8772423034221254
3940.2314078349555 33.616787682496685 0.8775679284502143
3940.2314078349555 42.65839262086404 0.8779995027920098
3940.2314078349555 54.13183669370275 0.8785736561990226
3940.2314078349555 68.69118979416318 0.8793394358468175
3940.2314078349555 87.16644110999944 0.8803616451676332
3940.2314078349555 110.6108145535225 0.8817243165880897
3940.2314078349555 140.3608101970589 0.8835337545798448
3940.2314078349555 178.11239451312218 0.8859203663185716
3940.2314078349555 226.01768281801222 0.8890381434152527
3940.2314078349555 286.807625522434 0.8930605325329214
3940.2314078349555 363.94769219915764 0.8981714999098033
3940.2314078349555 461.8354285936932 0.9045510052009287
3940.2314078349555 586.0511487667402 0.9123549789279752
3940.2314078349555 743.6760536467558 0.9216915572616903
3940.2314078349555 943.6959110675486 0.932597900898502
3940.2314078349555 1197.5133099937427 0.9450260788569266
3940.2314078349555 1519.5976911565988 0.9588523754248135
3940.2314078349555 1928.3102105817359 0.9739336891237943
3940.2314078349555 2446.9504592387466 0.990253737344309
3940.2314078349555 3105.0847094578075 1.0082620343556714
3940.2314078349555 3940.2314078349555 1.0297645424361122
3940.2314078349555 5000.0 1.0611826249665572

5000.0 5.0 0.8610464609897872
5000.0 6.344805015839611 0.8610999211653111
5000.0 8.051310137804697 0.8611681927598809
5000.0 10.216798589284712 0.8612555115196272
5000.0 12.96471898702334 0.8613673931872836
5000.0 16.451722811563343 0.8615110529737997
5000.0 20.87659468280201 0.8616959700303681
5000.0 26.491584531418546 0.8619346511382389
5000.0 33.616787682496685 0.8622436480724286
5000.0 42.65839262086404 0.8626449259765789
5000.0 54.13183669370275 0.8631676069864125
5000.0 68.69118979416318 0.8638502051333788
5000.0 87.16644110999944 0.8647433110796103
5000.0 110.6108145535225 0.8659126522406966
5000.0 140.3608101970589 0.8674422582791539
5000.0 178.11239451312218 0.869437185473074
5000.0 226.01768281801222 0.8720250693507935
5000.0 286.807625522434 0.8753554092934397
5000.0 363.94769219915764 0.8795953588113055
5000.0 461.8354285936932 0.8849209243221948
5000.0 586.0511487667402 0.8915029400460405
5000.0 743.6760536467558 0.8994884385160525
5000.0 943.6959110675486 0.9089801327487921
5000.0 1197.5133099937427 0.9200204621530665
5000.0 1519.5976911565988 0.9325925731587593
5000.0 1928.3102105817359 0.9466611451979725
5000.0 2446.9504592387466 0.9622996980962184
5000.0 3105.0847094578075 0.9800270372410861
5000.0 3940.2314078349555 1.0018136807931006
5000.0 5000.0 1.0354247066819968


==> 5_Results/Figures/Mixture_c_co_IOM.tex <==
x y z
5.0 5.0 1.1709382132180202
5.0 6.344805015839611 1.5510614615268548
5.0 8.051310137804697 2.0787036935350924
5.0 10.216798589284712 2.81484290871177
5.0 12.96471898702334 3.8460435932068253
5.0 16.451722811563343 5.295093120155212
5.0 20.87659468280201 7.335893881297072
5.0 26.491584531418546 10.214141664784583
5.0 33.616787682496685 14.275699493351036
5.0 42.65839262086404 20.004877633731535
5.0 54.13183669370275 28.074848444375913
5.0 68.69118979416318 39.411800389624936
5.0 87.16644110999944 55.27266773767836
5.0 110.6108145535225 77.33291096810898
5.0 140.3608101970589 107.77611790007892
5.0 178.11239451312218 149.37305795049497
5.0 226.01768281801222 205.53898627543342
5.0 286.807625522434 280.3703499117872
5.0 363.94769219915764 378.6874092948773
5.0 461.8354285936932 506.13806444043934
5.0 586.0511487667402 669.431199866143
5.0 743.6760536467558 876.7529407870655
5.0 943.6959110675486 1138.387550510953
5.0 1197.5133099937427 1467.5451436080036
5.0 1519.5976911565988 1881.4146514280208
5.0 1928.3102105817359 2402.5230606998193
5.0 2446.9504592387466 3060.6125565863103
5.0 3105.0847094578075 3895.55219087969
5.0 3940.2314078349555 4962.730813500108
5.0 5000.0 6346.11525126037

6.344805015839611 5.0 1.2837381057231476
6.344805015839611 6.344805015839611 1.678039543640308
6.344805015839611 8.051310137804697 2.2217970452026683
6.344805015839611 10.216798589284712 2.976258970639723
6.344805015839611 12.96471898702334 4.02829333670757
6.344805015839611 16.451722811563343 5.501023431433989
6.344805015839611 20.87659468280201 7.568715038601387
6.344805015839611 26.491584531418546 10.477442866641718
6.344805015839611 33.616787682496685 14.573441073310937
6.344805015839611 42.65839262086404 20.341342703215673
6.344805015839611 54.13183669370275 28.454529703770014
6.344805015839611 68.69118979416318 39.83919176200061
6.344805015839611 87.16644110999944 55.75193026549863
6.344805015839611 110.6108145535225 77.86739719182985
6.344805015839611 140.3608101970589 108.36777980709658
6.344805015839611 178.11239451312218 150.02183622780615
6.344805015839611 226.01768281801222 206.2423630515627
6.344805015839611 286.807625522434 281.1232869926047
6.344805015839611 363.94769219915764 379.48281692912184
6.344805015839611 461.8354285936932 506.96774102863884
6.344805015839611 586.0511487667402 670.2869603358221
6.344805015839611 743.6760536467558 877.6275739901668
6.344805015839611 943.6959110675486 1139.27537075049
6.344805015839611 1197.5133099937427 1468.4421218990192
6.344805015839611 1519.5976911565988 1882.3182779203546
6.344805015839611 1928.3102105817359 2403.4321440283516
6.344805015839611 2446.9504592387466 3061.527162153792
6.344805015839611 3105.0847094578075 3896.473982543685
6.344805015839611 3940.2314078349555 4963.664477090669
6.344805015839611 5000.0 6347.073753846146

8.051310137804697 5.0 1.4287476248025313
8.051310137804697 6.344805015839611 1.8410306759628288
8.051310137804697 8.051310137804697 2.4052260172975464
8.051310137804697 10.216798589284712 3.1829241874124494
8.051310137804697 12.96471898702334 4.26137747317508
8.051310137804697 16.451722811563343 5.76413420010401
8.051310137804697 20.87659468280201 7.86591971943786
8.051310137804697 26.491584531418546 10.813287613083475
8.051310137804697 33.616787682496685 14.95294059682995
8.051310137804697 42.65839262086404 20.769918498911874
8.051310137804697 54.13183669370275 28.93786616014961
8.051310137804697 68.69118979416318 40.38297186835621
8.051310137804697 87.16644110999944 56.36141245848748
8.051310137804697 110.6108145535225 78.54681367250379
8.051310137804697 140.3608101970589 109.11958836542011
8.051310137804697 178.11239451312218 150.845949291614
8.051310137804697 226.01768281801222 207.1355840369088
8.051310137804697 286.807625522434 282.07923391066964
8.051310137804697 363.94769219915764 380.49251583768825
8.051310137804697 461.8354285936932 508.02081382326463
8.051310137804697 586.0511487667402 671.3730506329662
8.051310137804697 743.6760536467558 878.7375572276957
8.051310137804697 943.6959110675486 1140.4020518228765
8.051310137804697 1197.5133099937427 1469.5804017994597
8.051310137804697 1519.5976911565988 1883.4649805018041
8.051310137804697 1928.3102105817359 2404.5857629823254
8.051310137804697 2446.9504592387466 3062.6877840737184
8.051310137804697 3105.0847094578075 3897.6437216717404
8.051310137804697 3940.2314078349555 4964.849283141968
8.051310137804697 5000.0 6348.290089717965

10.216798589284712 5.0 1.6157793376268677
10.216798589284712 6.344805015839611 2.050863138341131
10.216798589284712 8.051310137804697 2.6409728758495845
10.216798589284712 10.216798589284712 3.4481323028157087
10.216798589284712 12.96471898702334 4.560079720185287
10.216798589284712 16.451722811563343 6.100900829414338
10.216798589284712 20.87659468280201 8.245901634658837
10.216798589284712 26.491584531418546 11.242240232019459
10.216798589284712 33.616787682496685 15.43721006578674
10.216798589284712 42.65839262086404 21.316362650428687
10.216798589284712 54.13183669370275 29.553671517641234
10.216798589284712 68.69118979416318 41.0753184676006
10.216798589284712 87.16644110999944 57.13693819635628
10.216798589284712 110.6108145535225 79.41085379234711
10.216798589284712 140.3608101970589 110.07523104853715
10.216798589284712 178.11239451312218 151.89306385497358
10.216798589284712 226.01768281801222 208.27011191693182
10.216798589284712 286.807625522434 283.2930948721542
10.216798589284712 363.94769219915764 381.7743587856653
10.216798589284712 461.8354285936932 509.35751658599156
10.216798589284712 586.0511487667402 672.7515197742127
10.216798589284712 743.6760536467558 880.146255937353
10.216798589284712 943.6959110675486 1141.8318816073984
10.216798589284712 1197.5133099937427 1471.02491408648
10.216798589284712 1519.5976911565988 1884.9201589450995
10.216798589284712 1928.3102105817359 2406.0497049513215
10.216798589284712 2446.9504592387466 3064.1606052381494
10.216798589284712 3105.0847094578075 3899.1281095415584
10.216798589284712 3940.2314078349555 4966.352793436254
10.216798589284712 5000.0 6349.8336264096815

12.96471898702334 5.0 1.857993998608223
12.96471898702334 6.344805015839611 2.3219805914630016
12.96471898702334 8.051310137804697 2.944939412066084
12.96471898702334 10.216798589284712 3.7894419992112436
12.96471898702334 12.96471898702334 4.94384088722835
12.96471898702334 16.451722811563343 6.53290048649831
12.96471898702334 20.87659468280201 8.732659563269456
12.96471898702334 26.491584531418546 11.791038237875265
12.96471898702334 33.616787682496685 16.056073378286843
12.96471898702334 42.65839262086404 22.01395858768408
12.96471898702334 54.13183669370275 30.339076643684695
12.96471898702334 68.69118979416318 41.95759360690147
12.96471898702334 87.16644110999944 58.12445084605624
12.96471898702334 110.6108145535225 80.51031788861152
12.96471898702334 140.3608101970589 111.29051653959833
12.96471898702334 178.11239451312218 153.2239739460488
12.96471898702334 226.01768281801222 209.7114932674836
12.96471898702334 286.807625522434 284.8347235642939
12.96471898702334 363.94769219915764 383.4018894223702
12.96471898702334 461.8354285936932 511.05437347883986
12.96471898702334 586.0511487667402 674.5011655202208
12.96471898702334 743.6760536467558 881.9341179790698
12.96471898702334 943.6959110675486 1143.6464653409805
12.96471898702334 1197.5133099937427 1472.8580716097126
12.96471898702334 1519.5976911565988 1886.7668162386447
12.96471898702334 1928.3102105817359 2407.9074618057152
12.96471898702334 2446.9504592387466 3066.0296177259356
12.96471898702334 3105.0847094578075 3901.0117954413467
12.96471898702334 3940.2314078349555 4968.260749934467
12.96471898702334 5000.0 6351.792401097284

16.451722811563343 5.0 2.1732408571781896
16.451722811563343 6.344805015839611 2.673849718724369
16.451722811563343 8.051310137804697 3.338431027584064
16.451722811563343 10.216798589284712 4.2302482766966145
16.451722811563343 12.96471898702334 5.438429387265542
16.451722811563343 16.451722811563343 7.0885948526654685
16.451722811563343 20.87659468280201 9.357706734903958
16.451722811563343 26.491584531418546 12.494643963597317
16.451722811563343 33.616787682496685 16.848376856673806
16.451722811563343 42.65839262086404 22.90590224917982
16.451722811563343 54.13183669370275 31.342109714053905
16.451722811563343 68.69118979416318 43.083133416041164
16.451722811563343 87.16644110999944 59.3830264634769
16.451722811563343 110.6108145535225 81.91035938199897
16.451722811563343 140.3608101970589 112.83685721831048
16.451722811563343 178.11239451312218 154.91631527110803
16.451722811563343 226.01768281801222 211.54329152968967
16.451722811563343 286.807625522434 286.7930530144284
16.451722811563343 363.94769219915764 385.46864071596184
16.451722811563343 461.8354285936932 513.2086343589215
16.451722811563343 586.0511487667402 676.7220751108961
16.451722811563343 743.6760536467558 884.2032919409278
16.451722811563343 943.6959110675486 1145.9493992304308
16.451722811563343 1197.5133099937427 1475.1844822925432
16.451722811563343 1519.5976911565988 1889.1103011678194
16.451722811563343 1928.3102105817359 2410.2649979183893
16.451722811563343 2446.9504592387466 3068.4014179992864
16.451722811563343 3105.0847094578075 3903.4022088316347
16.451722811563343 3940.2314078349555 4970.681969836001
16.451722811563343 5000.0 6354.278149631703

20.87659468280201 5.0 2.5860331307916833
20.87659468280201 6.344805015839611 3.1330167912271047
20.87659468280201 8.051310137804697 3.8503064174440325
20.87659468280201 10.216798589284712 4.802038418570689
20.87659468280201 12.96471898702334 6.078318085718152
20.87659468280201 16.451722811563343 7.805843891654367
20.87659468280201 20.87659468280201 10.162738971790064
20.87659468280201 26.491584531418546 13.399085823930337
20.87659468280201 33.616787682496685 17.865023379816872
20.87659468280201 42.65839262086404 24.04854929729337
20.87659468280201 54.13183669370275 32.6251763354252
20.87659468280201 68.69118979416318 44.52097932360013
20.87659468280201 87.16644110999944 60.98887099122539
20.87659468280201 110.6108145535225 83.69475758940513
20.87659468280201 140.3608101970589 114.80581978853425
20.87659468280201 178.11239451312218 157.06938691244744
20.87659468280201 226.01768281801222 213.8721631786041
20.87659468280201 286.807625522434 289.2814004168716
20.87659468280201 363.94769219915764 388.0936355850383
20.87659468280201 461.8354285936932 515.9439347746393
20.87659468280201 586.0511487667402 679.5414086710384
20.87659468280201 743.6760536467558 887.0835017269416
20.87659468280201 943.6959110675486 1148.8722105840714
20.87659468280201 1197.5133099937427 1478.1369363357824
20.87659468280201 1519.5976911565988 1892.0843312778156
20.87659468280201 1928.3102105817359 2413.256804343254
20.87659468280201 2446.9504592387466 3071.4112949489413
20.87659468280201 3105.0847094578075 3906.4356941214846
20.87659468280201 3940.2314078349555 4973.754560448422
20.87659468280201 5000.0 6357.432692851149

26.491584531418546 5.0 3.130502210741008
26.491584531418546 6.344805015839611 3.736157361831013
26.491584531418546 8.051310137804697 4.520137619724574
26.491584531418546 10.216798589284712 5.547678723719823
26.491584531418546 12.96471898702334 6.910115573587292
26.491584531418546 16.451722811563343 8.735501064626982
26.491584531418546 20.87659468280201 11.203414707713106
26.491584531418546 26.491584531418546 14.565445233748072
26.491584531418546 33.616787682496685 19.173189090295903
26.491584531418546 42.65839262086404 25.51588456939464
26.491584531418546 54.13183669370275 34.269803666814674
26.491584531418546 68.69118979416318 46.36091681877698
26.491584531418546 87.16644110999944 63.04066746330606
26.491584531418546 110.6108145535225 85.97158234739035
26.491584531418546 140.3608101970589 117.31510722172659
26.491584531418546 178.11239451312218 159.8104404349757
26.491584531418546 226.01768281801222 216.8344335005476
26.491584531418546 286.807625522434 292.4442997332335
26.491584531418546 363.94769219915764 391.4284395265603
26.491584531418546 461.8354285936932 519.417528373414
26.491584531418546 586.0511487667402 683.1207713665344
26.491584531418546 743.6760536467558 890.7395235935423
26.491584531418546 943.6959110675486 1152.5819106843383
26.491584531418546 1197.5133099937427 1481.8840142386284
26.491584531418546 1519.5976911565988 1895.8586434533356
26.491584531418546 1928.3102105817359 2417.053587317686
26.491584531418546 2446.9504592387466 3075.230960403136
26.491584531418546 3105.0847094578075 3910.285300170142
26.491584531418546 3940.2314078349555 4977.653810810299
26.491584531418546 5000.0 6361.436048087485

33.616787682496685 5.0 3.8548753671044276
33.616787682496685 6.344805015839611 4.534661313858059
33.616787682496685 8.051310137804697 5.4029208603262235
33.616787682496685 10.216798589284712 6.5262711563439115
33.616787682496685 12.96471898702334 7.997590210664427
33.616787682496685 16.451722811563343 9.94662787258046
33.616787682496685 20.87659468280201 12.554784456377188
33.616787682496685 26.491584531418546 16.0755263615108
33.616787682496685 33.616787682496685 20.862259072421576
33.616787682496685 42.65839262086404 27.405748610923258
33.616787682496685 54.13183669370275 36.383180647915815
33.616787682496685 68.69118979416318 48.72034598736468
33.616787682496685 87.16644110999944 65.66679465576199
33.616787682496685 110.6108145535225 88.88076353107017
33.616787682496685 140.3608101970589 120.51647465889586
33.616787682496685 178.11239451312218 163.3029273640144
33.616787682496685 226.01768281801222 220.60465091449342
33.616787682496685 286.807625522434 296.46632979598417
33.616787682496685 363.94769219915764 395.66622358428475
33.616787682496685 461.8354285936932 523.8295430375329
33.616787682496685 586.0511487667402 687.6656221323943
33.616787682496685 743.6760536467558 895.3807094840154
33.616787682496685 943.6959110675486 1157.2906029228448
33.616787682496685 1197.5133099937427 1486.6397577117366
33.616787682496685 1519.5976911565988 1900.6487144146472
33.616787682496685 1928.3102105817359 2421.8720342215306
33.616787682496685 2446.9504592387466 3080.078367076617
33.616787682496685 3105.0847094578075 3915.1706724539526
33.616787682496685 3940.2314078349555 4982.602214208644
33.616787682496685 5000.0 6366.516734493433

42.65839262086404 5.0 4.828344871599536
42.65839262086404 6.344805015839611 5.601612571834913
42.65839262086404 8.051310137804697 6.57618967955513
42.65839262086404 10.216798589284712 7.8204241585184135
42.65839262086404 12.96471898702334 9.429124303205061
42.65839262086404 16.451722811563343 11.53415829934691
42.65839262086404 20.87659468280201 14.319193263638498
42.65839262086404 26.491584531418546 18.040024547898767
42.65839262086404 33.616787682496685 23.052288956709404
42.65839262086404 42.65839262086404 29.848617622853308
42.65839262086404 54.13183669370275 39.10727810663227
42.65839262086404 68.69118979416318 51.75376019047108
42.65839262086404 87.16644110999944 69.03516542651873
42.65839262086404 110.6108145535225 92.60429118825027
42.65839262086404 140.3608101970589 124.60627981945139
42.65839262086404 178.11239451312218 167.75737888821453
42.65839262086404 226.01768281801222 225.40676731456148
42.65839262086404 286.807625522434 301.58356131079165
42.65839262086404 363.94769219915764 401.0534409041784
42.65839262086404 461.8354285936932 529.4348486146548
42.65839262086404 586.0511487667402 693.4372945559628
42.65839262086404 743.6760536467558 901.2731270618793
42.65839262086404 943.6959110675486 1163.267712636722
42.65839262086404 1197.5133099937427 1492.6759679638596
42.65839262086404 1519.5976911565988 1906.7281150050508
42.65839262086404 1928.3102105817359 2427.9872213933822
42.65839262086404 2446.9504592387466 3086.2301798096078
42.65839262086404 3105.0847094578075 3921.370617976649
42.65839262086404 3940.2314078349555 4988.882199796927
42.65839262086404 5000.0 6372.964869703531

54.13183669370275 5.0 6.151714701517572
54.13183669370275 6.344805015839611 7.042528630495544
54.13183669370275 8.051310137804697 8.150875411973244
54.13183669370275 10.216798589284712 9.547263189421642
54.13183669370275 12.96471898702334 11.328904593668767
54.13183669370275 16.451722811563343 13.63029955226432
54.13183669370275 20.87659468280201 16.637921768515376
54.13183669370275 26.491584531418546 20.610436557326004
54.13183669370275 33.616787682496685 25.90621068931442
54.13183669370275 42.65839262086404 33.020126812928574
54.13183669370275 54.13183669370275 42.63170373361966
54.13183669370275 68.69118979416318 55.665941230169636
54.13183669370275 87.16644110999944 73.3667628132271
54.13183669370275 110.6108145535225 97.38007738623784
54.13183669370275 140.3608101970589 129.8396485807182
54.13183669370275 178.11239451312218 173.4458468542227
54.13183669370275 226.01768281801222 231.52882372002085
54.13183669370275 286.807625522434 308.09845721657973
54.13183669370275 363.94769219915764 407.90491394066083
54.13183669370275 461.8354285936932 536.5583045282048
54.13183669370275 586.0511487667402 700.768378909335
54.13183669370275 743.6760536467558 908.7550508444889
54.13183669370275 943.6959110675486 1170.8555648737283
54.13183669370275 1197.5133099937427 1500.3378530178043
54.13183669370275 1519.5976911565988 1914.4442178616616
54.13183669370275 1928.3102105817359 2435.7483832672892
54.13183669370275 2446.9504592387466 3094.0376218151478
54.13183669370275 3105.0847094578075 3929.2390690657953
54.13183669370275 3940.2314078349555 4996.852310113161
54.13183669370275 5000.0 6381.1488206573695

68.69118979416318 5.0 7.974039197730255
68.69118979416318 6.344805015839611 9.01202814035957
68.69118979416318 8.051310137804697 10.288038766675577
68.69118979416318 10.216798589284712 11.875260946797859
68.69118979416318 12.96471898702334 13.87388503019635
68.69118979416318 16.451722811563343 16.421659925492747
68.69118979416318 20.87659468280201 19.708509365209352
68.69118979416318 26.491584531418546 23.996605514854924
68.69118979416318 33.616787682496685 29.64762039314478
68.69118979416318 42.65839262086404 37.15911435980262
68.69118979416318 54.13183669370275 47.2120081070562
68.69118979416318 68.69118979416318 60.7305149657293
68.69118979416318 87.16644110999944 78.95442690989579
68.69118979416318 110.6108145535225 103.52094484765561
68.69118979416318 140.3608101970589 136.5496294002871
68.69118979416318 178.11239451312218 180.7211885981347
68.69118979416318 226.01768281801222 239.34233758076257
68.69118979416318 286.807625522434 316.39934607935646
68.69118979416318 363.94769219915764 416.62338829518916
68.69118979416318 461.8354285936932 545.6143940224896
68.69118979416318 586.0511487667402 710.0824364871985
68.69118979416318 743.6760536467558 918.2567520499547
68.69118979416318 943.6959110675486 1180.4892427468164
68.69118979416318 1197.5133099937427 1510.0639479447511
68.69118979416318 1519.5976911565988 1924.2381778301942
68.69118979416318 1928.3102105817359 2445.5989608655664
68.69118979416318 2446.9504592387466 3103.9466154898387
68.69118979416318 3105.0847094578075 3939.225371832643
68.69118979416318 3940.2314078349555 5006.967764405677
68.69118979416318 5000.0 6391.536384064827

87.16644110999944 5.0 10.518777757845562
87.16644110999944 6.344805015839611 11.739856313655554
87.16644110999944 8.051310137804697 13.224810466658713
87.16644110999944 10.216798589284712 15.050134605246813
87.16644110999944 12.96471898702334 17.319678145003646
87.16644110999944 16.451722811563343 20.17516710386884
87.16644110999944 20.87659468280201 23.810725942970095
87.16644110999944 26.491584531418546 28.492764620506172
87.16644110999944 33.616787682496685 34.58690142263939
87.16644110999944 42.65839262086404 42.59382042066205
87.16644110999944 54.13183669370275 53.195940664873
87.16644110999944 68.69118979416318 67.31623364691671
87.16644110999944 87.16644110999944 86.18911554769838
87.16644110999944 110.6108145535225 111.44081236696995
87.16644110999944 140.3608101970589 145.1732516260566
87.16644110999944 178.11239451312218 190.04295986425197
87.16644110999944 226.01768281801222 249.32801604088462
87.16644110999944 286.807625522434 326.9859698871772
87.16644110999944 363.94769219915764 427.7249529380041
87.16644110999944 461.8354285936932 557.1325660451658
87.16644110999944 586.0511487667402 721.9193094937161
87.16644110999944 743.6760536467558 930.3258119899194
87.16644110999944 943.6959110675486 1192.7219260761362
87.16644110999944 1197.5133099937427 1522.4114924649289
87.16644110999944 1519.5976911565988 1936.6703611824596
87.16644110999944 1928.3102105817359 2458.102102387229
87.16644110999944 2446.9504592387466 3116.5233919678494
87.16644110999944 3105.0847094578075 3951.900080873779
87.16644110999944 3940.2314078349555 5019.806608386802
87.16644110999944 5000.0 6404.721746531527

110.6108145535225 5.0 14.125016859021375
110.6108145535225 6.344805015839611 15.571637710614523
110.6108145535225 8.051310137804697 17.31473119558316
110.6108145535225 10.216798589284712 19.43482258295935
110.6108145535225 12.96471898702334 22.040209477894205
110.6108145535225 16.451722811563343 25.277430126978533
110.6108145535225 20.87659468280201 29.345659036394665
110.6108145535225 26.491584531418546 34.51635211009546
110.6108145535225 33.616787682496685 41.15975465943249
110.6108145535225 42.65839262086404 49.78009799321448
110.6108145535225 54.13183669370275 61.06128690693128
110.6108145535225 68.69118979416318 75.92437026094711
110.6108145535225 87.16644110999944 95.59677523797717
110.6108145535225 110.6108145535225 121.69096179658773
110.6108145535225 140.3608101970589 156.287124784952
110.6108145535225 178.11239451312218 202.01231772666335
110.6108145535225 226.01768281801222 262.1099831541153
110.6108145535225 286.807625522434 340.50310883730515
110.6108145535225 363.94769219915764 441.87217700197345
110.6108145535225 461.8354285936932 571.7900159431306
110.6108145535225 586.0511487667402 736.967672389417
110.6108145535225 743.6760536467558 945.6595437411263
110.6108145535225 943.6959110675486 1208.2572555087177
110.6108145535225 1197.5133099937427 1538.0887864635285
110.6108145535225 1519.5976911565988 1952.4527300137295
110.6108145535225 1928.3102105817359 2473.973115870328
110.6108145535225 2446.9504592387466 3132.487069980569
110.6108145535225 3105.0847094578075 3967.987770325828
110.6108145535225 3940.2314078349555 5036.102986630108
110.6108145535225 5000.0 6421.459830442188

140.3608101970589 5.0 19.312299465549096
140.3608101970589 6.344805015839611 21.032577787945367
140.3608101970589 8.051310137804697 23.090387349828777
140.3608101970589 10.216798589284712 25.57110955642581
140.3608101970589 12.96471898702334 28.588373647954395
140.3608101970589 16.451722811563343 32.29445082575281
140.3608101970589 20.87659468280201 36.89448241958941
140.3608101970589 26.491584531418546 42.66581471043754
140.3608101970589 33.616787682496685 49.98398633753414
140.3608101970589 42.65839262086404 59.3571116794282
140.3608101970589 54.13183669370275 71.47038095072391
140.3608101970589 68.69118979416318 87.24192871766246
140.3608101970589 87.16644110999944 107.89013100312825
140.3608101970589 110.6108145535225 135.01030663385833
140.3608101970589 140.3608101970589 170.65612750202436
140.3608101970589 178.11239451312218 217.41913908731186
140.3608101970589 226.01768281801222 278.5014214498161
140.3608101970589 286.807625522434 357.7849229139684
140.3608101970589 363.94769219915764 459.91738990517354
140.3608101970589 461.8354285936932 590.4541690705848
140.3608101970589 586.0511487667402 756.1069605176281
140.3608101970589 743.6760536467558 965.1465720901705
140.3608101970589 943.6959110675486 1227.9907135510352
140.3608101970589 1197.5133099937427 1557.9964774557393
140.3608101970589 1519.5976911565988 1972.4901136454828
140.3608101970589 1928.3102105817359 2494.1207949646705
140.3608101970589 2446.9504592387466 3152.7511245736364
140.3608101970589 3105.0847094578075 3988.408794340884
140.3608101970589 3940.2314078349555 5056.789507299235
140.3608101970589 5000.0 6442.710096267127

178.11239451312218 5.0 26.881535701755983
178.11239451312218 6.344805015839611 28.926125393307743
178.11239451312218 8.051310137804697 31.359842677723748
178.11239451312218 10.216798589284712 34.27385673602615
178.11239451312218 12.96471898702334 37.78808751689128
178.11239451312218 16.451722811563343 42.06150502996621
178.11239451312218 20.87659468280201 47.30614352671996
178.11239451312218 26.491584531418546 53.806045791371865
178.11239451312218 33.616787682496685 61.94260752568479
178.11239451312218 42.65839262086404 72.22797532012206
178.11239451312218 54.13183669370275 85.34813491322801
178.11239451312218 68.69118979416318 102.21691117561969
178.11239451312218 87.16644110999944 124.04105315029778
178.11239451312218 110.6108145535225 152.39476655061338
178.11239451312218 140.3608101970589 189.29977948201366
178.11239451312218 178.11239451312218 237.30549122190718
178.11239451312218 226.01768281801222 299.56536837165964
178.11239451312218 286.807625522434 379.9134181782428
178.11239451312218 363.94769219915764 482.9592419164686
178.11239451312218 461.8354285936932 614.2377833186604
178.11239451312218 586.0511487667402 780.4614407567677
178.11239451312218 743.6760536467558 989.9202176717238
178.11239451312218 943.6959110675486 1253.06258773632
178.11239451312218 1197.5133099937427 1583.280292203272
178.11239451312218 1519.5976911565988 1997.9328468387898
178.11239451312218 1928.3102105817359 2519.700081214026
178.11239451312218 2446.9504592387466 3178.476207460933
178.11239451312218 3105.0847094578075 4014.3324760517307
178.11239451312218 3940.2314078349555 5083.051231141942
178.11239451312218 5000.0 6469.6924826481445

226.01768281801222 5.0 38.068281999101956
226.01768281801222 6.344805015839611 40.48347025616433
226.01768281801222 8.051310137804697 43.352149321650465
226.01768281801222 10.216798589284712 46.772401866894725
226.01768281801222 12.96471898702334 50.87149947259962
226.01768281801222 16.451722811563343 55.81609566896047
226.01768281801222 20.87659468280201 61.82598460146476
226.01768281801222 26.491584531418546 69.19257401742355
226.01768281801222 33.616787682496685 78.30345902349256
226.01768281801222 42.65839262086404 89.67465616027847
226.01768281801222 54.13183669370275 103.99205416577611
226.01768281801222 68.69118979416318 122.1632909496835
226.01768281801222 87.16644110999944 145.38038462176524
226.01768281801222 110.6108145535225 175.1919377018159
226.01768281801222 140.3608101970589 213.58187520074338
226.01768281801222 178.11239451312218 263.05050949449594
226.01768281801222 226.01768281801222 326.6952843613147
226.01768281801222 286.807625522434 408.2952931420963
226.01768281801222 363.94769219915764 512.4165058490822
226.01768281801222 461.8354285936932 644.5704010024307
226.01768281801222 586.0511487667402 811.4699596375057
226.01768281801222 743.6760536467558 1021.4270830877288
226.01768281801222 943.6959110675486 1284.9258127672838
226.01768281801222 1197.5133099937427 1615.3984404254963
226.01768281801222 1519.5976911565988 2030.2439593850575
226.01768281801222 1928.3102105817359 2552.1792250737003
226.01768281801222 2446.9504592387466 3211.137479408497
226.01768281801222 3105.0847094578075 4047.2449110954617
226.01768281801222 3940.2314078349555 5116.394549695059
226.01768281801222 5000.0 6503.958976215378

286.807625522434 5.0 54.76459019500822
286.807625522434 6.344805015839611 57.58036519688326
286.807625522434 8.051310137804697 60.928316573232344
286.807625522434 10.216798589284712 64.91505004452631
286.807625522434 12.96471898702334 69.67654884216883
286.807625522434 16.451722811563343 75.3882530761851
286.807625522434 20.87659468280201 82.27853722951508
286.807625522434 26.491584531418546 90.64664953116755
286.807625522434 33.616787682496685 100.88641103161508
286.807625522434 42.65839262086404 113.5171289616842
286.807625522434 54.13183669370275 129.22322264627817
286.807625522434 68.69118979416318 148.90376940911557
286.807625522434 87.16644110999944 173.73251557154612
286.807625522434 110.6108145535225 205.22767951558208
286.807625522434 140.3608101970589 245.32946015244005
286.807625522434 178.11239451312218 296.48233705630105
286.807625522434 226.01768281801222 361.72071291972
286.807625522434 286.807625522434 444.7622166271079
286.807625522434 363.94769219915764 550.1239458744932
286.807625522434 461.8354285936932 683.2907851164492
286.807625522434 586.0511487667402 850.9758345700958
286.807625522434 743.6760536467558 1061.5151663742997
286.807625522434 943.6959110675486 1325.4329086249622
286.807625522434 1197.5133099937427 1656.207829345395
286.807625522434 1519.5976911565988 2071.2850047459315
286.807625522434 1928.3102105817359 2593.4255074672574
286.807625522434 2446.9504592387466 3252.610517924161
286.807625522434 3105.0847094578075 4089.0354901934775
286.807625522434 3940.2314078349555 5158.735179319932
286.807625522434 5000.0 6547.48539265214

363.94769219915764 5.0 79.81325465271381
363.94769219915764 6.344805015839611 83.0272315649736
363.94769219915764 8.051310137804697 86.86533733555403
363.94769219915764 10.216798589284712 91.44532295242364
363.94769219915764 12.96471898702334 96.91405164822342
363.94769219915764 16.451722811563343 103.45739328556489
363.94769219915764 20.87659468280201 111.3133783822058
363.94769219915764 26.491584531418546 120.78956793478822
363.94769219915764 33.616787682496685 132.2858179554773
363.94769219915764 42.65839262086404 146.32379626391415
363.94769219915764 54.13183669370275 163.5846745692106
363.94769219915764 68.69118979416318 184.9562570189646
363.94769219915764 87.16644110999944 211.59031767741183
363.94769219915764 110.6108145535225 244.9700528731227
363.94769219915764 140.3608101970589 286.9865346377103
363.94769219915764 178.11239451312218 340.0225484804195
363.94769219915764 226.01768281801222 407.04352908822915
363.94769219915764 286.807625522434 491.70010010316327
363.94769219915764 363.94769219915764 598.4558446729346
363.94769219915764 461.8354285936932 732.7658991164449
363.94769219915764 586.0511487667402 901.3424003413691
363.94769219915764 743.6760536467558 1112.5469338676508
363.94769219915764 943.6959110675486 1376.9473665055896
363.94769219915764 1197.5133099937427 1708.0743732813605
363.94769219915764 1519.5976911565988 2123.4257651623166
363.94769219915764 1928.3102105817359 2645.81473853999
363.94769219915764 2446.9504592387466 3305.2810307548325
363.94769219915764 3105.0847094578075 4142.107442513641
363.94769219915764 3940.2314078349555 5212.510769337706
363.94769219915764 5000.0 6602.789439492288

461.8354285936932 5.0 117.34266017264537
461.8354285936932 6.344805015839611 120.9051804955425
461.8354285936932 8.051310137804697 125.19060734339834
461.8354285936932 10.216798589284712 130.331797349156
461.8354285936932 12.96471898702334 136.4901045584283
461.8354285936932 16.451722811563343 143.864800184228
461.8354285936932 20.87659468280201 152.70570861901004
461.8354285936932 26.491584531418546 163.32990198929627
461.8354285936932 33.616787682496685 176.14349434225187
461.8354285936932 42.65839262086404 191.66976490158868
461.8354285936932 54.13183669370275 210.58495804253974
461.8354285936932 68.69118979416318 233.76306709093114
461.8354285936932 87.16644110999944 262.33063007562936
461.8354285936932 110.6108145535225 297.7320234037746
461.8354285936932 140.3608101970589 341.8050995765959
461.8354285936932 178.11239451312218 396.8667904330174
461.8354285936932 226.01768281801222 465.8094828400798
461.8354285936932 286.807625522434 552.2128517675667
461.8354285936932 363.94769219915764 660.4832442142109
461.8354285936932 461.8354285936932 796.0428598484094
461.8354285936932 586.0511487667402 965.6008295014907
461.8354285936932 743.6760536467558 1177.544054249292
461.8354285936932 943.6959110675486 1442.4861977998085
461.8354285936932 1197.5133099937427 1774.0140993901805
461.8354285936932 1519.5976911565988 2189.6845199525196
461.8354285936932 1928.3102105817359 2712.371225538534
461.8354285936932 2446.9504592387466 3372.1851136232053
461.8354285936932 3105.0847094578075 4209.51926805705
461.8354285936932 3940.2314078349555 5280.825321336276
461.8354285936932 5000.0 6673.083211212996

586.0511487667402 5.0 173.0521794586785
586.0511487667402 6.344805015839611 176.86199024526096
586.0511487667402 8.051310137804697 181.48710634340713
586.0511487667402 10.216798589284712 187.07985372502756
586.0511487667402 12.96471898702334 193.82092067739995
586.0511487667402 16.451722811563343 201.9277492245076
586.0511487667402 20.87659468280201 211.66613692013553
586.0511487667402 26.491584531418546 223.36587238174292
586.0511487667402 33.616787682496685 237.44134791089581
586.0511487667402 42.65839262086404 254.4182539931974
586.0511487667402 54.13183669370275 274.9676046608463
586.0511487667402 68.69118979416318 299.94841374169295
586.0511487667402 87.16644110999944 330.46026905385537
586.0511487667402 110.6108145535225 367.9068158371318
586.0511487667402 140.3608101970589 414.07087144228876
586.0511487667402 178.11239451312218 471.201911282474
586.0511487667402 226.01768281801222 542.1177390780236
586.0511487667402 286.807625522434 630.325230535301
586.0511487667402 363.94769219915764 740.1709516981871
586.0511487667402 461.8354285936932 877.0409169391929
586.0511487667402 586.0511487667402 1047.6379317084572
586.0511487667402 743.6760536467558 1260.3718857381286
586.0511487667402 943.6959110675486 1525.9019511171177
586.0511487667402 1197.5133099937427 1857.8734679483302
586.0511487667402 1519.5976911565988 2273.9073666546674
586.0511487667402 1928.3102105817359 2796.946772799824
586.0511487667402 2446.9504592387466 3457.1887356581065
586.0511487667402 3105.0847094578075 4295.165987343681
586.0511487667402 3940.2314078349555 5367.634917900409
586.0511487667402 5000.0 6762.471260560038

743.6760536467558 5.0 254.31606189241066
743.6760536467558 6.344805015839611 258.2340686490798
743.6760536467558 8.051310137804697 263.0366750339128
743.6760536467558 10.216798589284712 268.8978067623495
743.6760536467558 12.96471898702334 276.0213630648267
743.6760536467558 16.451722811563343 284.648176870999
743.6760536467558 20.87659468280201 295.06594599893583
743.6760536467558 26.491584531418546 307.62309280733547
743.6760536467558 33.616787682496685 322.74758034629133
743.6760536467558 42.65839262086404 340.9717927822694
743.6760536467558 54.13183669370275 362.9646887972268
743.6760536467558 68.69118979416318 389.57254251366015
743.6760536467558 87.16644110999944 421.8696594695626
743.6760536467558 110.6108145535225 461.2204736688812
743.6760536467558 140.3608101970589 509.3544482690743
743.6760536467558 178.11239451312218 568.4554703555057
743.6760536467558 226.01768281801222 641.2684094489263
743.6760536467558 286.807625522434 731.22801635426
743.6760536467558 363.94769219915764 842.6199698393285
743.6760536467558 461.8354285936932 980.7909223673355
743.6760536467558 586.0511487667402 1152.4326609799814
743.6760536467558 743.6760536467558 1365.9732877759166
743.6760536467558 943.6959110675486 1632.1143089475036
743.6760536467558 1197.5133099937427 1964.5593643050074
743.6760536467558 1519.5976911565988 2380.9972944945657
743.6760536467558 1928.3102105817359 2904.4496296085263
743.6760536467558 2446.9504592387466 3565.2176407467477
743.6760536467558 3105.0847094578075 4404.011863514219
743.6760536467558 3940.2314078349555 5477.987439055766
743.6760536467558 5000.0 6876.209874576575

943.6959110675486 5.0 370.0287067202014
943.6959110675486 6.344805015839611 373.90737553471934
943.6959110675486 8.051310137804697 378.7041522328169
943.6959110675486 10.216798589284712 384.6119321944002
943.6959110675486 12.96471898702334 391.85738709861994
943.6959110675486 16.451722811563343 400.70687223369083
943.6959110675486 20.87659468280201 411.47464051883867
943.6959110675486 26.491584531418546 424.5344556281949
943.6959110675486 33.616787682496685 440.3358532355151
943.6959110675486 42.65839262086404 459.42639245319214
943.6959110675486 54.13183669370275 482.48129187184014
943.6959110675486 68.69118979416318 510.3418994413494
943.6959110675486 87.16644110999944 544.0645352351659
943.6959110675486 110.6108145535225 584.9813843243643
943.6959110675486 140.3608101970589 634.7753489171712
943.6959110675486 178.11239451312218 695.5712320202234
943.6959110675486 226.01768281801222 770.0466267620442
943.6959110675486 286.807625522434 861.5679720651956
943.6959110675486 363.94769219915764 974.3609644039316
943.6959110675486 461.8354285936932 1113.730306274545
943.6959110675486 586.0511487667402 1286.3511821955526
943.6959110675486 743.6760536467558 1500.6629551856126
943.6959110675486 943.6959110675486 1767.403423803563
943.6959110675486 1197.5133099937427 2100.3316112614602
943.6959110675486 1519.5976911565988 2517.2063864289717
943.6959110675486 1928.3102105817359 3041.1372396759057
943.6959110675486 2446.9504592387466 3702.5520819378626
943.6959110675486 3105.0847094578075 4542.389910422563
943.6959110675486 3940.2314078349555 5618.33347361569
943.6959110675486 5000.0 7021.050276914599

1197.5133099937427 5.0 530.3067434372465
1197.5133099937427 6.344805015839611 534.0221876128523
1197.5133099937427 8.051310137804697 538.6510353322703
1197.5133099937427 10.216798589284712 544.3979563714925
1197.5133099937427 12.96471898702334 551.5062852659023
1197.5133099937427 16.451722811563343 560.2639522054064
1197.5133099937427 20.87659468280201 571.0109323402198
1197.5133099937427 26.491584531418546 584.1491775650472
1197.5133099937427 33.616787682496685 600.1563388338456
1197.5133099937427 42.65839262086404 619.6048675103345
1197.5133099937427 54.13183669370275 643.1882622316673
1197.5133099937427 68.69118979416318 671.7563211579044
1197.5133099937427 87.16644110999944 706.3613165973884
1197.5133099937427 110.6108145535225 748.3171283772933
1197.5133099937427 140.3608101970589 799.2736295838429
1197.5133099937427 178.11239451312218 861.3091689251081
1197.5133099937427 226.01768281801222 937.045003472997
1197.5133099937427 286.807625522434 1029.7873788871784
1197.5133099937427 363.94769219915764 1143.7060901414798
1197.5133099937427 461.8354285936932 1284.0631851953942
1197.5133099937427 586.0511487667402 1457.5120970765538
1197.5133099937427 743.6760536467558 1672.4955308642861
1197.5133099937427 943.6959110675486 1939.779593472785
1197.5133099937427 1197.5133099937427 2273.173691827256
1197.5133099937427 1519.5976911565988 2690.507770830646
1197.5133099937427 1928.3102105817359 3214.9903193213486
1197.5133099937427 2446.9504592387466 3877.205008114085
1197.5133099937427 3105.0847094578075 4718.388525883817
1197.5133099937427 3940.2314078349555 5796.932388563337
1197.5133099937427 5000.0 7205.700528573532

1519.5976911565988 5.0 746.3678814193613
1519.5976911565988 6.344805015839611 749.840268365314
1519.5976911565988 8.051310137804697 754.1908083734883
1519.5976911565988 10.216798589284712 759.6270803609569
1519.5976911565988 12.96471898702334 766.3995358825551
1519.5976911565988 16.451722811563343 774.8084425519118
1519.5976911565988 20.87659468280201 785.2118981750974
1519.5976911565988 26.491584531418546 798.0355452056401
1519.5976911565988 33.616787682496685 813.7850179020378
1519.5976911565988 42.65839262086404 833.0626299164843
1519.5976911565988 54.13183669370275 856.5902467431974
1519.5976911565988 68.69118979416318 885.2406414947937
1519.5976911565988 87.16644110999944 920.0798450158252
1519.5976911565988 110.6108145535225 962.423169471988
1519.5976911565988 140.3608101970589 1013.9077827044788
1519.5976911565988 178.11239451312218 1076.5851845021969
1519.5976911565988 226.01768281801222 1153.0378288306886
1519.5976911565988 286.807625522434 1246.5257928542683
1519.5976911565988 363.94769219915764 1361.1720769191938
1519.5976911565988 461.8354285936932 1502.199337185859
1519.5976911565988 586.0511487667402 1676.2367998627324
1519.5976911565988 743.6760536467558 1891.7238806279463
1519.5976911565988 943.6959110675486 2159.4471099939733
1519.5976911565988 1197.5133099937427 2493.260932229558
1519.5976911565988 1519.5976911565988 2911.0679858963967
1519.5976911565988 1928.3102105817359 3436.1904815457146
1519.5976911565988 2446.9504592387466 4099.407946393669
1519.5976911565988 3105.0847094578075 4942.3528199730235
1519.5976911565988 3940.2314078349555 6024.388328502955
1519.5976911565988 5000.0 7441.46330961325

1928.3102105817359 5.0 1030.8972071705225
1928.3102105817359 6.344805015839611 1034.0937504090523
1928.3102105817359 8.051310137804697 1038.1151644448291
1928.3102105817359 10.216798589284712 1043.164489444248
1928.3102105817359 12.96471898702334 1049.4900770233799
1928.3102105817359 16.451722811563343 1057.3938780252856
1928.3102105817359 20.87659468280201 1067.2408474020122
1928.3102105817359 26.491584531418546 1079.4697866087445
1928.3102105817359 33.616787682496685 1094.6062615415487
1928.3102105817359 42.65839262086404 1113.2787055517551
1928.3102105817359 54.13183669370275 1136.2394055829293
1928.3102105817359 68.69118979416318 1164.3926915771776
1928.3102105817359 87.16644110999944 1198.8332486330808
1928.3102105817359 110.6108145535225 1240.8978998636176
1928.3102105817359 140.3608101970589 1292.234605643285
1928.3102105817359 178.11239451312218 1354.8928137977384
1928.3102105817359 226.01768281801222 1431.4400743074054
1928.3102105817359 286.807625522434 1525.1111260559096
1928.3102105817359 363.94769219915764 1639.998043308778
1928.3102105817359 461.8354285936932 1781.2936888886154
1928.3102105817359 586.0511487667402 1955.6060951071183
1928.3102105817359 743.6760536467558 2171.369086597681
1928.3102105817359 943.6959110675486 2439.384892034273
1928.3102105817359 1197.5133099937427 2773.5502572347236
1928.3102105817359 1519.5976911565988 3191.8457845578932
1928.3102105817359 1928.3102105817359 3717.7299495355937
1928.3102105817359 2446.9504592387466 4382.236832898551
1928.3102105817359 3105.0847094578075 5227.53945468265
1928.3102105817359 3940.2314078349555 6314.370013193715
1928.3102105817359 5000.0 7743.1532222479755

2446.9504592387466 5.0 1398.9680683382808
2446.9504592387466 6.344805015839611 1401.893125985109
2446.9504592387466 8.051310137804697 1405.5835858002856
2446.9504592387466 10.216798589284712 1410.2333919380249
2446.9504592387466 12.96471898702334 1416.082394042659
2446.9504592387466 16.451722811563343 1423.4257611988494
2446.9504592387466 20.87659468280201 1432.6248477614663
2446.9504592387466 26.491584531418546 1444.1197024706048
2446.9504592387466 33.616787682496685 1458.4436111693499
2446.9504592387466 42.65839262086404 1476.2403658813134
2446.9504592387466 54.13183669370275 1498.2854887551887
2446.9504592387466 68.69118979416318 1525.5133177951143
2446.9504592387466 87.16644110999944 1559.052740254046
2446.9504592387466 110.6108145535225 1600.2751422284482
2446.9504592387466 140.3608101970589 1650.8590229985796
2446.9504592387466 178.11239451312218 1712.8763511637715
2446.9504592387466 226.01768281801222 1788.906542369292
2446.9504592387466 286.807625522434 1882.1851292747767
2446.9504592387466 363.94769219915764 1996.7960436482126
2446.9504592387466 461.8354285936932 2137.9196668570685
2446.9504592387466 586.0511487667402 2312.15378475494
2446.9504592387466 743.6760536467558 2527.9318200281054
2446.9504592387466 943.6959110675486 2796.0738117524525
2446.9504592387466 1197.5133099937427 3130.52280085479
2446.9504592387466 1519.5976911565988 3549.3511956301168
2446.9504592387466 1928.3102105817359 4076.1912923932255
2446.9504592387466 2446.9504592387466 4742.422709608595
2446.9504592387466 3105.0847094578075 5590.983603754201
2446.9504592387466 3940.2314078349555 6684.606517397783
2446.9504592387466 5000.0 8130.506377847261

3105.0847094578075 5.0 1869.3582237021546
3105.0847094578075 6.344805015839611 1872.0390403600834
3105.0847094578075 8.051310137804697 1875.4279774450788
3105.0847094578075 10.216798589284712 1879.7080938863337
3105.0847094578075 12.96471898702334 1885.1076342616866
3105.0847094578075 16.451722811563343 1891.9101359816264
3105.0847094578075 20.87659468280201 1900.466370767248
3105.0847094578075 26.491584531418546 1911.2083599284608
3105.0847094578075 33.616787682496685 1924.6657676412856
3105.0847094578075 42.65839262086404 1941.485180065126
3105.0847094578075 54.13183669370275 1962.4531061977434
3105.0847094578075 68.69118979416318 1988.5241206872822
3105.0847094578075 87.16644110999944 2020.8563684248525
3105.0847094578075 110.6108145535225 2060.8577357089457
3105.0847094578075 140.3608101970589 2110.247139080663
3105.0847094578075 178.11239451312218 2171.1365835294887
3105.0847094578075 226.01768281801222 2246.1409116884493
3105.0847094578075 286.807625522434 2338.5232809902864
3105.0847094578075 363.94769219915764 2452.3865451907936
3105.0847094578075 461.8354285936932 2592.9229937630917
3105.0847094578075 586.0511487667402 2766.7400341185403
3105.0847094578075 743.6760536467558 2982.2859062213734
3105.0847094578075 943.6959110675486 3250.411291454786
3105.0847094578075 1197.5133099937427 3585.1215852925416
3105.0847094578075 1519.5976911565988 4004.6110256620427
3105.0847094578075 1928.3102105817359 4532.7509249790355
3105.0847094578075 2446.9504592387466 5201.41545949942
3105.0847094578075 3105.0847094578075 6054.676935726378
3105.0847094578075 3940.2314078349555 7158.340339030146
3105.0847094578075 5000.0 8630.590518633928

3940.2314078349555 5.0 2466.074030652523
3940.2314078349555 6.344805015839611 2468.548420980238
3940.2314078349555 8.051310137804697 2471.6805024828564
3940.2314078349555 10.216798589284712 2475.6426093722785
3940.2314078349555 12.96471898702334 2480.650857899745
3940.2314078349555 16.451722811563343 2486.975554825583
3940.2314078349555 20.87659468280201 2494.95375429173
3940.2314078349555 26.491584531418546 2505.0042949802387
3940.2314078349555 33.616787682496685 2517.6456983357175
3940.2314078349555 42.65839262086404 2533.5174261277793
3940.2314078349555 54.13183669370275 2553.4051690041074
3940.2314078349555 68.69118979416318 2578.2712711952468
3940.2314078349555 87.16644110999944 2609.292016687297
3940.2314078349555 110.6108145535225 2647.904449505074
3940.2314078349555 140.3608101970589 2695.8667411841957
3940.2314078349555 178.11239451312218 2755.3376346040072
3940.2314078349555 226.01768281801222 2828.9822408584405
3940.2314078349555 286.807625522434 2920.1133099341073
3940.2314078349555 363.94769219915764 3032.879216364603
3940.2314078349555 461.8354285936932 3172.512734035892
3940.2314078349555 586.0511487667402 3345.658916629551
3940.2314078349555 743.6760536467558 3560.807641383888
3940.2314078349555 943.6959110675486 3828.8679607468107
3940.2314078349555 1197.5133099937427 4163.943200253288
3940.2314078349555 1519.5976911565988 4584.408418132204
3940.2314078349555 1928.3102105817359 5114.490819859624
3940.2314078349555 2446.9504592387466 5786.819049651319
3940.2314078349555 3105.0847094578075 6647.2535043907355
3940.2314078349555 3940.2314078349555 7766.663020881524
3940.2314078349555 5000.0 9282.671265905772

5000.0 5.0 3219.9930592855426
5000.0 6.344805015839611 3222.3013980847963
5000.0 8.051310137804697 3225.2258133093405
5000.0 10.216798589284712 3228.929187465939
5000.0 12.96471898702334 3233.6165922714304
5000.0 16.451722811563343 3239.5457415820547
5000.0 20.87659468280201 3247.039801513016
5000.0 26.491584531418546 3256.50299272872
5000.0 33.616787682496685 3268.4394813855997
5000.0 42.65839262086404 3283.476139383436
5000.0 54.13183669370275 3302.3899128878147
5000.0 68.69118979416318 3326.1407654426166
5000.0 87.16644110999944 3355.911671175299
5000.0 110.6108145535225 3393.1578504523686
5000.0 140.3608101970589 3439.668621538554
5000.0 178.11239451312218 3497.646841544163
5000.0 226.01768281801222 3569.812953505257
5000.0 286.807625522434 3659.543076970909
5000.0 363.94769219915764 3771.0533808301957
5000.0 461.8354285936932 3909.6464015626584
5000.0 586.0511487667402 4082.0397319492313
5000.0 743.6760536467558 4296.804974238085
5000.0 943.6959110675486 4564.9583055743315
5000.0 1197.5133099937427 4900.768995000788
5000.0 1519.5976911565988 5322.9061224014695
5000.0 1928.3102105817359 5856.173538724204
5000.0 2446.9504592387466 6534.447988372113
5000.0 3105.0847094578075 7406.665229055791
5000.0 3940.2314078349555 8552.963403839942
5000.0 5000.0 10150.77267079673


==> 5_Results/Figures/Mixture_c_co_IOM_DM_diff.tex <==
x y z
5.0 5.0 0.9923782826952283
5.0 6.344805015839611 0.9946076421056143
5.0 8.051310137804697 0.9967361356040831
5.0 10.216798589284712 0.9988372426021646
5.0 12.96471898702334 1.0010002506949647
5.0 16.451722811563343 1.0033369272404344
5.0 20.87659468280201 1.0059893329197203
5.0 26.491584531418546 1.0091379270922698
5.0 33.616787682496685 1.0130078664694784
5.0 42.65839262086404 1.0178692902648283
5.0 54.13183669370275 1.0240245194719608
5.0 68.69118979416318 1.031772507669131
5.0 87.16644110999944 1.041341193919268
5.0 110.6108145535225 1.0527867892366458
5.0 140.3608101970589 1.0658775848339868
5.0 178.11239451312218 1.0800067657776589
5.0 226.01768281801222 1.0941943272622499
5.0 286.807625522434 1.1072203541904262
5.0 363.94769219915764 1.1178734737017595
5.0 461.8354285936932 1.1252301470517765
5.0 586.0511487667402 1.1288551308399049
5.0 743.6760536467558 1.1288489474247607
5.0 943.6959110675486 1.1257609429818582
5.0 1197.5133099937427 1.1204152567155625
5.0 1519.5976911565988 1.1137420509240064
5.0 1928.3102105817359 1.1066614937922237
5.0 2446.9504592387466 1.100049923683449
5.0 3105.0847094578075 1.0948121004870977
5.0 3940.2314078349555 1.0921392674423245
5.0 5000.0 1.0943016108674282

6.344805015839611 5.0 0.9878798498484961
6.344805015839611 6.344805015839611 0.9906564460782055
6.344805015839611 8.051310137804697 0.9932736528470979
6.344805015839611 10.216798589284712 0.995812530020786
6.344805015839611 12.96471898702334 0.9983691335789816
6.344805015839611 16.451722811563343 1.0010612365259355
6.344805015839611 20.87659468280201 1.0040361384496765
6.344805015839611 26.491584531418546 1.0074787129401204
6.344805015839611 33.616787682496685 1.0116175827074778
6.344805015839611 42.65839262086404 1.0167252204393031
6.344805015839611 54.13183669370275 1.023104946251097
6.344805015839611 68.69118979416318 1.0310552654350502
6.344805015839611 87.16644110999944 1.0408023751182676
6.344805015839611 110.6108145535225 1.0524000410847398
6.344805015839611 140.3608101970589 1.0656144757133883
6.344805015839611 178.11239451312218 1.079838401831599
6.344805015839611 226.01768281801222 1.0940938198583063
6.344805015839611 286.807625522434 1.1071652021753289
6.344805015839611 363.94769219915764 1.1178468905612382
6.344805015839611 461.8354285936932 1.1252209353638332
6.344805015839611 586.0511487667402 1.1288564558525647
6.344805015839611 743.6760536467558 1.1288568101730871
6.344805015839611 943.6959110675486 1.125772862902997
6.344805015839611 1197.5133099937427 1.1204295216849791
6.344805015839611 1519.5976911565988 1.1137573740912068
6.344805015839611 1928.3102105817359 1.1066769116115125
6.344805015839611 2446.9504592387466 1.1000647860163377
6.344805015839611 3105.0847094578075 1.0948260878807723
6.344805015839611 3940.2314078349555 1.0921524587334845
6.344805015839611 5000.0 1.0943147942437257

8.051310137804697 5.0 0.9821483761729787
8.051310137804697 6.344805015839611 0.9856244534140421
8.051310137804697 8.051310137804697 0.9888663850280537
8.051310137804697 10.216798589284712 0.9919647521475911
8.051310137804697 12.96471898702334 0.9950241832007348
8.051310137804697 16.451722811563343 0.998170088847184
8.051310137804697 20.87659468280201 1.0015564481281873
8.051310137804697 26.491584531418546 1.0053737715339686
8.051310137804697 33.616787682496685 1.0098551145500878
8.051310137804697 42.65839262086404 1.015275945286317
8.051310137804697 54.13183669370275 1.0219408913875263
8.051310137804697 68.69118979416318 1.0301479433282141
8.051310137804697 87.16644110999944 1.0401211644781738
8.051310137804697 110.6108145535225 1.0519113186441709
8.051310137804697 140.3608101970589 1.0652820938642937
8.051310137804697 178.11239451312218 1.0796257297203542
8.051310137804697 226.01768281801222 1.0939668403148137
8.051310137804697 286.807625522434 1.1070954897393137
8.051310137804697 363.94769219915764 1.1178132583873936
8.051310137804697 461.8354285936932 1.125209257576922
8.051310137804697 586.0511487667402 1.1288581106272844
8.051310137804697 743.6760536467558 1.128866749812267
8.051310137804697 943.6959110675486 1.125787952217301
8.051310137804697 1197.5133099937427 1.120447592780564
8.051310137804697 1519.5976911565988 1.1137767950268123
8.051310137804697 1928.3102105817359 1.1066964590674537
8.051310137804697 2446.9504592387466 1.1000836338466116
8.051310137804697 3105.0847094578075 1.0948438295411502
8.051310137804697 3940.2314078349555 1.092169193344801
8.051310137804697 5000.0 1.0943315216256766

10.216798589284712 5.0 0.9748481728479123
10.216798589284712 6.344805015839611 0.9792171437265385
10.216798589284712 8.051310137804697 0.9832571062578753
10.216798589284712 10.216798589284712 0.9870703647933793
10.216798589284712 12.96471898702334 0.9907722304134525
10.216798589284712 16.451722811563343 0.9944977111214098
10.216798589284712 20.87659468280201 0.9984092259127765
10.216798589284712 26.491584531418546 1.0027044338559505
10.216798589284712 33.616787682496685 1.0076220279439232
10.216798589284712 42.65839262086404 1.0134413026821127
10.216798589284712 54.13183669370275 1.020468588218334
10.216798589284712 68.69118979416318 1.0290012945136133
10.216798589284712 87.16644110999944 1.0392608904324838
10.216798589284712 110.6108145535225 1.0512944845681766
10.216798589284712 140.3608101970589 1.0648627372323243
10.216798589284712 178.11239451312218 1.079357434569544
10.216798589284712 226.01768281801222 1.093806613362272
10.216798589284712 286.807625522434 1.1070074686946056
10.216798589284712 363.94769219915764 1.1177707435391726
10.216798589284712 461.8354285936932 1.125194457995918
10.216798589284712 586.0511487667402 1.1288601680424837
10.216798589284712 743.6760536467558 1.1288793021232955
10.216798589284712 943.6959110675486 1.1258070412192227
10.216798589284712 1197.5133099937427 1.1204704751888586
10.216798589284712 1519.5976911565988 1.1138014015478868
10.216798589284712 1928.3102105817359 1.1067212364358032
10.216798589284712 2446.9504592387466 1.100107531878486
10.216798589284712 3105.0847094578075 1.094866330469714
10.216798589284712 3940.2314078349555 1.0921904214737734
10.216798589284712 5000.0 1.0943527451109034

12.96471898702334 5.0 0.9655606883313769
12.96471898702334 6.344805015839611 0.9710655454845877
12.96471898702334 8.051310137804697 0.9761225983806969
12.96471898702334 10.216798589284712 0.9808480143549138
12.96471898702334 12.96471898702334 0.985370025328604
12.96471898702334 16.451722811563343 0.9898354324599005
12.96471898702334 20.87659468280201 0.9944171384320005
12.96471898702334 26.491584531418546 0.9993217461620918
12.96471898702334 33.616787682496685 1.004795037484693
12.96471898702334 42.65839262086404 1.0111211438476086
12.96471898702334 54.13183669370275 1.0186085844953783
12.96471898702334 68.69118979416318 1.0275541213714317
12.96471898702334 87.16644110999944 1.0381760923604872
12.96471898702334 110.6108145535225 1.0505171991220763
12.96471898702334 140.3608101970589 1.064334527644952
12.96471898702334 178.11239451312218 1.0790195326911705
12.96471898702334 226.01768281801222 1.093604754361669
12.96471898702334 286.807625522434 1.106896486410577
12.96471898702334 363.94769219915764 1.1177170579564903
12.96471898702334 461.8354285936932 1.125175709789064
12.96471898702334 586.0511487667402 1.1288627113232907
12.96471898702334 743.6760536467558 1.1288951333652701
12.96471898702334 943.6959110675486 1.1258311701989279
12.96471898702334 1197.5133099937427 1.1204994331588383
12.96471898702334 1519.5976911565988 1.1138325653847672
12.96471898702334 1928.3102105817359 1.1067526335904796
12.96471898702334 2446.9504592387466 1.1001378267802306
12.96471898702334 3105.0847094578075 1.0948948630840418
12.96471898702334 3940.2314078349555 1.0922173471684005
12.96471898702334 5000.0 1.0943796722038692

16.451722811563343 5.0 0.9537757513001373
16.451722811563343 6.344805015839611 0.9607157561533584
16.451722811563343 8.051310137804697 0.9670626868487322
16.451722811563343 10.216798589284712 0.9729479018722024
16.451722811563343 12.96471898702334 0.9785144243365004
16.451722811563343 16.451722811563343 0.983922966073416
16.451722811563343 20.87659468280201 0.9893590504865636
16.451722811563343 26.491584531418546 0.9950401941590019
16.451722811563343 33.616787682496685 1.0012209051000966
16.451722811563343 42.65839262086404 1.0081913066845194
16.451722811563343 54.13183669370275 1.0162626614250003
16.451722811563343 68.69118979416318 1.0257309949946396
16.451722811563343 87.16644110999944 1.036810890229727
16.451722811563343 110.6108145535225 1.0495397951574474
16.451722811563343 140.3608101970589 1.0636706610835454
16.451722811563343 178.11239451312218 1.0785948885319752
16.451722811563343 226.01768281801222 1.093350968648565
16.451722811563343 286.807625522434 1.1067568068647249
16.451722811563343 363.94769219915764 1.1176493613175345
16.451722811563343 461.8354285936932 1.1251519727318526
16.451722811563343 586.0511487667402 1.1288658318931069
16.451722811563343 743.6760536467558 1.1289150673705308
16.451722811563343 943.6959110675486 1.1258616379936812
16.451722811563343 1197.5133099937427 1.12053605311884
16.451722811563343 1519.5976911565988 1.1138720133104598
16.451722811563343 1928.3102105817359 1.1067924040659576
16.451722811563343 2446.9504592387466 1.1001762203550909
16.451722811563343 3105.0847094578075 1.0949310373874854
16.451722811563343 3940.2314078349555 1.0922514955600877
16.451722811563343 5000.0 1.0944138341034328

20.87659468280201 5.0 0.9388958746783389
20.87659468280201 6.344805015839611 0.9476269831678572
20.87659468280201 8.051310137804697 0.955594644112565
20.87659468280201 10.216798589284712 0.9629443915496481
20.87659468280201 12.96471898702334 0.9698344466857471
20.87659468280201 16.451722811563343 0.9764407115900826
20.87659468280201 20.87659468280201 0.9829630483299543
20.87659468280201 26.491584531418546 0.9896316934628102
20.87659468280201 33.616787682496685 0.9967114839669369
20.87659468280201 42.65839262086404 1.0044996899799308
20.87659468280201 54.13183669370275 1.0133108557493775
20.87659468280201 68.69118979416318 1.023440062191728
20.87659468280201 87.16644110999944 1.0350974334686864
20.87659468280201 110.6108145535225 1.048314215504218
20.87659468280201 140.3608101970589 1.0628386982326028
20.87659468280201 178.11239451312218 1.0780627500299966
20.87659468280201 226.01768281801222 1.093032752449758
20.87659468280201 286.807625522434 1.1065814236554696
20.87659468280201 363.94769219915764 1.117564152416943
20.87659468280201 461.8354285936932 1.1251219424603809
20.87659468280201 586.0511487667402 1.1288696231294373
20.87659468280201 743.6760536467558 1.1289401153635823
20.87659468280201 943.6959110675486 1.1259000589643084
20.87659468280201 1197.5133099937427 1.120582319536712
20.87659468280201 1519.5976911565988 1.113921914294658
20.87659468280201 1928.3102105817359 1.10684275674132
20.87659468280201 2446.9504592387466 1.1002248607845087
20.87659468280201 3105.0847094578075 1.0949768889501283
20.87659468280201 3940.2314078349555 1.0922947975472475
20.87659468280201 5000.0 1.0944571721109992

26.491584531418546 5.0 0.9202699585072004
26.491584531418546 6.344805015839611 0.9311905752430181
26.491584531418546 8.051310137804697 0.9411622760689755
26.491584531418546 10.216798589284712 0.9503387259554618
26.491584531418546 12.96471898702334 0.9588902129636895
26.491584531418546 16.451722811563343 0.9670067263600614
26.491584531418546 20.87659468280201 0.974902648933382
26.491584531418546 26.491584531418546 0.9828217905595725
26.491584531418546 33.616787682496685 0.9910403363160318
26.491584531418546 42.65839262086404 0.9998634805943909
26.491584531418546 54.13183669370275 1.009609278556096
26.491584531418546 68.69118979416318 1.0205714980125746
26.491584531418546 87.16644110999944 1.032954821745213
26.491584531418546 110.6108145535225 1.046783277664269
26.491584531418546 140.3608101970589 1.0618000635788412
26.491584531418546 178.11239451312218 1.0773984009585618
26.491584531418546 226.01768281801222 1.092635147027052
26.491584531418546 286.807625522434 1.1063618877984764
26.491584531418546 363.94769219915764 1.1174571568878569
26.491584531418546 461.8354285936932 1.1250839912392507
26.491584531418546 586.0511487667402 1.1288741697195046
26.491584531418546 743.6760536467558 1.1289715067562593
26.491584531418546 943.6959110675486 1.1259484280466878
26.491584531418546 1197.5133099937427 1.120640705092144
26.491584531418546 1519.5976911565988 1.1139849851397565
26.491584531418546 1928.3102105817359 1.106906468522241
26.491584531418546 2446.9504592387466 1.100286455843285
26.491584531418546 3105.0847094578075 1.0950349888533477
26.491584531418546 3940.2314078349555 1.0923496962415964
26.491584531418546 5000.0 1.0945121468851724

33.616787682496685 5.0 0.8972824558481305
33.616787682496685 6.344805015839611 0.9107914451958126
33.616787682496685 8.051310137804697 0.9231766253122572
33.616787682496685 10.216798589284712 0.9345848999216597
33.616787682496685 12.96471898702334 0.9451886420114678
33.616787682496685 16.451722811563343 0.9551857463680069
33.616787682496685 20.87659468280201 0.9648016657079843
33.616787682496685 26.491584531418546 0.9742921067035478
33.616787682496685 33.616787682496685 0.9839438832380145
33.616787682496685 42.65839262086404 0.9940696990930994
33.616787682496685 54.13183669370275 1.0049904839960755
33.616787682496685 68.69118979416318 1.0169977029672905
33.616787682496685 87.16644110999944 1.0302892537383188
33.616787682496685 110.6108145535225 1.0448807653841607
33.616787682496685 140.3608101970589 1.0605100658237852
33.616787682496685 178.11239451312218 1.0765731125453353
33.616787682496685 226.01768281801222 1.0921406424925304
33.616787682496685 286.807625522434 1.1060881945167513
33.616787682496685 363.94769219915764 1.1173232267681208
33.616787682496685 461.8354285936932 1.1250361021103488
33.616787682496685 586.0511487667402 1.1288795276377845
33.616787682496685 743.6760536467558 1.1290107175519606
33.616787682496685 943.6959110675486 1.1260091920391422
33.616787682496685 1197.5133099937427 1.1207142750111398
33.616787682496685 1519.5976911565988 1.114064616728435
33.616787682496685 1928.3102105817359 1.1069870215136408
33.616787682496685 2446.9504592387466 1.1003644124694534
33.616787682496685 3105.0847094578075 1.0951085804876488
33.616787682496685 3940.2314078349555 1.0924192804206128
33.616787682496685 5000.0 1.0945818764521815

42.65839262086404 5.0 0.8695300765274772
42.65839262086404 6.344805015839611 0.8859421507165741
42.65839262086404 8.051310137804697 0.9011146354103476
42.65839262086404 10.216798589284712 0.9151604426197865
42.65839262086404 12.96471898702334 0.9282332129806479
42.65839262086404 16.451722811563343 0.9405236660111003
42.65839262086404 20.87659468280201 0.9522579143934083
42.65839262086404 26.491584531418546 0.96369663613426
42.65839262086404 33.616787682496685 0.9751327019195549
42.65839262086404 42.65839262086404 0.9868830735608114
42.65839262086404 54.13183669370275 0.9992690180875291
42.65839262086404 68.69118979416318 1.012577266928719
42.65839262086404 87.16644110999944 1.0269967711443069
42.65839262086404 110.6108145535225 1.0425332362897355
42.65839262086404 140.3608101970589 1.0589189896356783
42.65839262086404 178.11239451312218 1.0755547134138335
42.65839262086404 226.01768281801222 1.0915294012000358
42.65839262086404 286.807625522434 1.1057488089354601
42.65839262086404 363.94769219915764 1.1171562820313965
42.65839262086404 461.8354285936932 1.1249758021300995
42.65839262086404 586.0511487667402 1.128885692338518
42.65839262086404 743.6760536467558 1.1290594904061444
42.65839262086404 943.6959110675486 1.1260853227703802
42.65839262086404 1197.5133099937427 1.1208068045080821
42.65839262086404 1519.5976911565988 1.1141650218990955
42.65839262086404 1928.3102105817359 1.1070887678816028
42.65839262086404 2446.9504592387466 1.100463007360763
42.65839262086404 3105.0847094578075 1.0952017488079693
42.65839262086404 3940.2314078349555 1.0925074512770327
42.65839262086404 5000.0 1.0946703103321318

54.13183669370275 5.0 0.8371045200929973
54.13183669370275 6.344805015839611 0.856518049980994
54.13183669370275 8.051310137804697 0.8747069160140447
54.13183669370275 10.216798589284712 0.8917116360975272
54.13183669370275 12.96471898702334 0.9076335483240292
54.13183669370275 16.451722811563343 0.9226287344436707
54.13183669370275 20.87659468280201 0.9369026135132728
54.13183669370275 26.491584531418546 0.9507048506325488
54.13183669370275 33.616787682496685 0.9643226105612944
54.13183669370275 42.65839262086404 0.9780684700400467
54.13183669370275 54.13183669370275 0.9922573847150039
54.13183669370275 68.69118979416318 1.0071661773971898
54.13183669370275 87.16644110999944 1.0229709238485203
54.13183669370275 110.6108145535225 1.039665041852657
54.13183669370275 140.3608101970589 1.0569751770318025
54.13183669370275 178.11239451312218 1.0743093094512528
54.13183669370275 226.01768281801222 1.0907800859265946
54.13183669370275 286.807625522434 1.1053309679227128
54.13183669370275 363.94769219915764 1.1169493488081144
54.13183669370275 461.8354285936932 1.1249001078238396
54.13183669370275 586.0511487667402 1.1288925490209116
54.13183669370275 743.6760536467558 1.1291198367932438
54.13183669370275 943.6959110675486 1.1261803837297117
54.13183669370275 1197.5133099937427 1.120922903644343
54.13183669370275 1519.5976911565988 1.1142914039155443
54.13183669370275 1928.3102105817359 1.1072171245596845
54.13183669370275 2446.9504592387466 1.100587593136857
54.13183669370275 3105.0847094578075 1.0953196282118962
54.13183669370275 3940.2314078349555 1.0926191298737087
54.13183669370275 5000.0 1.0947824489030782

68.69118979416318 5.0 0.8009427688253252
68.69118979416318 6.344805015839611 0.8230878130171229
68.69118979416318 8.051310137804697 0.8442292749939687
68.69118979416318 10.216798589284712 0.8642980372260233
68.69118979416318 12.96471898702334 0.8833027350533934
68.69118979416318 16.451722811563343 0.9013260718794067
68.69118979416318 20.87659468280201 0.9185185901248749
68.69118979416318 26.491584531418546 0.9350904553015913
68.69118979416318 33.616787682496685 0.9513003395388632
68.69118979416318 42.65839262086404 0.9674386163542598
68.69118979416318 54.13183669370275 0.9838002292194616
68.69118979416318 68.69118979416318 1.0006417429030203
68.69118979416318 87.16644110999944 1.018119013999357
68.69118979416318 110.6108145535225 1.036208907839936
68.69118979416318 140.3608101970589 1.054631538885377
68.69118979416318 178.11239451312218 1.0728049911845432
68.69118979416318 226.01768281801222 1.0898717479016713
68.69118979416318 286.807625522434 1.1048214827536122
68.69118979416318 363.94769219915764 1.1166947888858387
68.69118979416318 461.8354285936932 1.124806260363489
68.69118979416318 586.0511487667402 1.1288998029898516
68.69118979416318 743.6760536467558 1.129194006861542
68.69118979416318 943.6959110675486 1.1262985756457697
68.69118979416318 1197.5133099937427 1.121068140061575
68.69118979416318 1519.5976911565988 1.114450140477592
68.69118979416318 1928.3102105817359 1.1073787976335647
68.69118979416318 2446.9504592387466 1.1007448436765725
68.69118979416318 3105.0847094578075 1.0954686553840318
68.69118979416318 3940.2314078349555 1.0927605137995349
68.69118979416318 5000.0 1.0949246192394235

87.16644110999944 5.0 0.7631040510178674
87.16644110999944 6.344805015839611 0.78724835677209
87.16644110999944 8.051310137804697 0.8108510763556398
87.16644110999944 10.216798589284712 0.833721964871757
87.16644110999944 12.96471898702334 0.8557486736313996
87.16644110999944 16.451722811563343 0.8769025746342101
87.16644110999944 20.87659468280201 0.8972380818864577
87.16644110999944 26.491584531418546 0.9168860356896009
87.16644110999944 33.616787682496685 0.9360410372902547
87.16644110999944 42.65839262086404 0.9549412046683303
87.16644110999944 54.13183669370275 0.9738372089558193
87.16644110999944 68.69118979416318 0.9929466973575144
87.16644110999944 87.16644110999944 1.0123920059673202
87.16644110999944 110.6108145535225 1.0321253898916847
87.16644110999944 140.3608101970589 1.0518575597837703
87.16644110999944 178.11239451312218 1.0710187498489419
87.16644110999944 226.01768281801222 1.0887874545401317
87.16644110999944 286.807625522434 1.1042083903885818
87.16644110999944 363.94769219915764 1.1163848739037179
87.16644110999944 461.8354285936932 1.1246886565735903
87.16644110999944 586.0511487667402 1.128906887334339
87.16644110999944 743.6760536467558 1.1292844068933892
87.16644110999944 943.6959110675486 1.126444737696874
87.16644110999944 1197.5133099937427 1.1212491402593825
87.16644110999944 1519.5976911565988 1.1146489716438677
87.16644110999944 1928.3102105817359 1.107582031849149
87.16644110999944 2446.9504592387466 1.1009430399218958
87.16644110999944 3105.0847094578075 1.095656872858628
87.16644110999944 3940.2314078349555 1.0929393923905995
87.16644110999944 5000.0 1.0951048211617629

110.6108145535225 5.0 0.7267600667570459
110.6108145535225 6.344805015839611 0.7517691262988727
110.6108145535225 8.051310137804697 0.7768872435105785
110.6108145535225 10.216798589284712 0.8018381348625996
110.6108145535225 12.96471898702334 0.8263978352692387
110.6108145535225 16.451722811563343 0.8504130879557865
110.6108145535225 20.87659468280201 0.8738123132497195
110.6108145535225 26.491584531418546 0.8966076521865212
110.6108145535225 33.616787682496685 0.9188871243840504
110.6108145535225 42.65839262086404 0.9407957656629915
110.6108145535225 54.13183669370275 0.9625039644240712
110.6108145535225 68.69118979416318 0.9841610084960631
110.6108145535225 87.16644110999944 1.0058336494802544
110.6108145535225 110.6108145535225 1.0274350451901184
110.6108145535225 140.3608101970589 1.0486593148938264
110.6108145535225 178.11239451312218 1.068948168636848
110.6108145535225 226.01768281801222 1.0875205750509902
110.6108145535225 286.807625522434 1.103483951069781
110.6108145535225 363.94769219915764 1.1160129473370037
110.6108145535225 461.8354285936932 1.1245440222321648
110.6108145535225 586.0511487667402 1.1289128598923073
110.6108145535225 743.6760536467558 1.1293934392047054
110.6108145535225 943.6959110675486 1.1266242697286943
110.6108145535225 1197.5133099937427 1.1214736385959698
110.6108145535225 1519.5976911565988 1.1148971696670549
110.6108145535225 1928.3102105817359 1.1078368731112498
110.6108145535225 2446.9504592387466 1.1011923928386025
110.6108145535225 3105.0847094578075 1.0958942870758759
110.6108145535225 3940.2314078349555 1.0931655302025618
110.6108145535225 5000.0 1.0953331601408336

140.3608101970589 5.0 0.695777369165875
140.3608101970589 6.344805015839611 0.7203482907257767
140.3608101970589 8.051310137804697 0.7457309692365484
140.3608101970589 10.216798589284712 0.771635792633956
140.3608101970589 12.96471898702334 0.7977829336717783
140.3608101970589 16.451722811563343 0.8239259209824533
140.3608101970589 20.87659468280201 0.8498733833643572
140.3608101970589 26.491584531418546 0.8755029733526704
140.3608101970589 33.616787682496685 0.9007646566615765
140.3608101970589 42.65839262086404 0.9256705027015323
140.3608101970589 54.13183669370275 0.9502689637389429
140.3608101970589 68.69118979416318 0.9746026857416326
140.3608101970589 87.16644110999944 0.9986513077584696
140.3608101970589 110.6108145535225 1.0222658472250519
140.3608101970589 140.3608101970589 1.0451095866769888
140.3608101970589 178.11239451312218 1.0666294228827033
140.3608101970589 226.01768281801222 1.086084751031325
140.3608101970589 286.807625522434 1.1026496174731233
140.3608101970589 363.94769219915764 1.1155761279992935
140.3608101970589 461.8354285936932 1.1243685760334292
140.3608101970589 586.0511487667402 1.1289163183148465
140.3608101970589 743.6760536467558 1.1295232379329456
140.3608101970589 943.6959110675486 1.1268429276170533
140.3608101970589 1197.5133099937427 1.1217504260891942
140.3608101970589 1519.5976911565988 1.115205652822438
140.3608101970589 1928.3102105817359 1.108155419595021
140.3608101970589 2446.9504592387466 1.1015053920504603
140.3608101970589 3105.0847094578075 1.09619328040059
140.3608101970589 3940.2314078349555 1.093451127660702
140.3608101970589 5000.0 1.095622387011104

178.11239451312218 5.0 0.6740267300175766
178.11239451312218 6.344805015839611 0.6969808126707137
178.11239451312218 8.051310137804697 0.7213483889847465
178.11239451312218 10.216798589284712 0.7468990918936548
178.11239451312218 12.96471898702334 0.7733726564375755
178.11239451312218 16.451722811563343 0.800497940603007
178.11239451312218 20.87659468280201 0.8280142742928124
178.11239451312218 26.491584531418546 0.8556925535657415
178.11239451312218 33.616787682496685 0.8833478841528002
178.11239451312218 42.65839262086404 0.9108426620756328
178.11239451312218 54.13183669370275 0.9380733705148637
178.11239451312218 68.69118979416318 0.9649401358309351
178.11239451312218 87.16644110999944 0.991300282663269
178.11239451312218 110.6108145535225 1.016912716350978
178.11239451312218 140.3608101970589 1.041387455890915
178.11239451312218 178.11239451312218 1.0641619944553231
178.11239451312218 226.01768281801222 1.084528224461539
178.11239451312218 286.807625522434 1.1017242044903952
178.11239451312218 363.94769219915764 1.1150759709088212
178.11239451312218 461.8354285936932 1.124160019945091
178.11239451312218 586.0511487667402 1.1289154052965695
178.11239451312218 743.6760536467558 1.129675282798013
178.11239451312218 943.6959110675486 1.1271064324939548
178.11239451312218 1197.5133099937427 1.1220891301238503
178.11239451312218 1519.5976911565988 1.1155869834835028
178.11239451312218 1928.3102105817359 1.1085520184605608
178.11239451312218 2446.9504592387466 1.1018971551908108
178.11239451312218 3105.0847094578075 1.096569068563234
178.11239451312218 3940.2314078349555 1.093811365150963
178.11239451312218 5000.0 1.0959885681718324

226.01768281801222 5.0 0.6647199295884986
226.01768281801222 6.344805015839611 0.6851968957331317
226.01768281801222 8.051310137804697 0.707492276881539
226.01768281801222 10.216798589284712 0.7314737489815474
226.01768281801222 12.96471898702334 0.7569579524899364
226.01768281801222 16.451722811563343 0.7837181786702376
226.01768281801222 20.87659468280201 0.8114968545843362
226.01768281801222 26.491584531418546 0.8400211934317602
226.01768281801222 33.616787682496685 0.8690185961526766
226.01768281801222 42.65839262086404 0.8982269487263868
226.01768281801222 54.13183669370275 0.9273942379767498
226.01768281801222 68.69118979416318 0.9562655533456738
226.01768281801222 87.16644110999944 0.984552161557998
226.01768281801222 110.6108145535225 1.011893476214101
226.01768281801222 140.3608101970589 1.0378199444855354
226.01768281801222 178.11239451312218 1.0617377429041979
226.01768281801222 226.01768281801222 1.0829522336258939
226.01768281801222 286.807625522434 1.100751275161533
226.01768281801222 363.94769219915764 1.1145280646789373
226.01768281801222 461.8354285936932 1.1239194520463398
226.01768281801222 586.0511487667402 1.128908031789683
226.01768281801222 743.6760536467558 1.129849901018241
226.01768281801222 943.6959110675486 1.1274198321676956
226.01768281801222 1197.5133099937427 1.1224997356740267
226.01768281801222 1519.5976911565988 1.1160551629580928
226.01768281801222 1928.3102105817359 1.109043338621928
226.01768281801222 2446.9504592387466 1.102385732174056
226.01768281801222 3105.0847094578075 1.0970401812808974
226.01768281801222 3940.2314078349555 1.0942650310695579
226.01768281801222 5000.0 1.0964519141616946

286.807625522434 5.0 0.669959607866981
286.807625522434 6.344805015839611 0.6874579820905549
286.807625522434 8.051310137804697 0.7069606775915522
286.807625522434 10.216798589284712 0.7284372100121784
286.807625522434 12.96471898702334 0.7518019769813584
286.807625522434 16.451722811563343 0.7769124107679997
286.807625522434 20.87659468280201 0.8035704883163273
286.807625522434 26.491584531418546 0.8315278603639304
286.807625522434 33.616787682496685 0.8604937655081039
286.807625522434 42.65839262086404 0.8901434002310299
286.807625522434 54.13183669370275 0.9201230916942046
286.807625522434 68.69118979416318 0.9500483354637049
286.807625522434 87.16644110999944 0.9794924428351366
286.807625522434 110.6108145535225 1.0079677047728213
286.807625522434 140.3608101970589 1.03490717797913
286.807625522434 178.11239451312218 1.0596613934454997
286.807625522434 226.01768281801222 1.0815266747758683
286.807625522434 286.807625522434 1.099815754314274
286.807625522434 363.94769219915764 1.1139653457376633
286.807625522434 461.8354285936932 1.1236543130233014
286.807625522434 586.0511487667402 1.1288925159574907
286.807625522434 743.6760536467558 1.1300457267996962
286.807625522434 943.6959110675486 1.127786573197915
286.807625522434 1197.5133099937427 1.1229917451114837
286.807625522434 1519.5976911565988 1.1166251045553557
286.807625522434 1928.3102105817359 1.1096482153484442
286.807625522434 2446.9504592387466 1.1029922884326662
286.807625522434 3105.0847094578075 1.0976289234053525
286.807625522434 3940.2314078349555 1.0948352239981907
286.807625522434 5000.0 1.0970377995663352

363.94769219915764 5.0 0.690461092483627
363.94769219915764 6.344805015839611 0.7047891956029083
363.94769219915764 8.051310137804697 0.7211102664687804
363.94769219915764 10.216798589284712 0.7394801500827699
363.94769219915764 12.96471898702334 0.7599050953199195
363.94769219915764 16.451722811563343 0.7823344185031414
363.94769219915764 20.87659468280201 0.8066545376990146
363.94769219915764 26.491584531418546 0.8326848844837934
363.94769219915764 33.616787682496685 0.8601760593555584
363.94769219915764 42.65839262086404 0.8888100954800434
363.94769219915764 54.13183669370275 0.9182018809437346
363.94769219915764 68.69118979416318 0.9479000943252842
363.94769219915764 87.16644110999944 0.9773862042850133
363.94769219915764 110.6108145535225 1.0060719998809156
363.94769219915764 140.3608101970589 1.033299975143359
363.94769219915764 178.11239451312218 1.0583555317088935
363.94769219915764 226.01768281801222 1.0805024715547409
363.94769219915764 286.807625522434 1.0990497810570967
363.94769219915764 363.94769219915764 1.113446165570736
363.94769219915764 461.8354285936932 1.1233823453865295
363.94769219915764 586.0511487667402 1.1288688672235139
363.94769219915764 743.6760536467558 1.1302592808819747
363.94769219915764 943.6959110675486 1.1282073037426938
363.94769219915764 1197.5133099937427 1.1235728863935368
363.94769219915764 1519.5976911565988 1.1173116434487496
363.94769219915764 1928.3102105817359 1.1103871229553621
363.94769219915764 2446.9504592387466 1.1037410510771362
363.94769219915764 3105.0847094578075 1.0983617398754186
363.94769219915764 3940.2314078349555 1.0955501026243828
363.94769219915764 5000.0 1.0977780144493416

461.8354285936932 5.0 0.7253350710856966
461.8354285936932 6.344805015839611 0.7365530535262199
461.8354285936932 8.051310137804697 0.7495935253230782
461.8354285936932 10.216798589284712 0.7645755106171834
461.8354285936932 12.96471898702334 0.7815790715815092
461.8354285936932 16.451722811563343 0.8006348805986491
461.8354285936932 20.87659468280201 0.821714134006957
461.8354285936932 26.491584531418546 0.8447190014180374
461.8354285936932 33.616787682496685 0.8694739077178588
461.8354285936932 42.65839262086404 0.8957180919834142
461.8354285936932 54.13183669370275 0.9230999680902084
461.8354285936932 68.69118979416318 0.9511738165025649
461.8354285936932 87.16644110999944 0.9793994851559974
461.8354285936932 110.6108145535225 1.007146495486668
461.8354285936932 140.3608101970589 1.0337056138905574
461.8354285936932 178.11239451312218 1.0583132206689967
461.8354285936932 226.01768281801222 1.0801951436887096
461.8354285936932 286.807625522434 1.0986343656718414
461.8354285936932 363.94769219915764 1.1130591342519196
461.8354285936932 461.8354285936932 1.123135852649686
461.8354285936932 586.0511487667402 1.128840847414958
461.8354285936932 743.6760536467558 1.1304849412012759
461.8354285936932 943.6959110675486 1.1286785486267885
461.8354285936932 1197.5133099937427 1.1242473426023307
461.8354285936932 1519.5976911565988 1.1181279454852937
461.8354285936932 1928.3102105817359 1.111281098089913
461.8354285936932 2446.9504592387466 1.1046588551913712
461.8354285936932 3105.0847094578075 1.099269370914986
461.8354285936932 3940.2314078349555 1.0964436335304448
461.8354285936932 5000.0 1.098712300621343

586.0511487667402 5.0 0.7719574559362142
586.0511487667402 6.344805015839611 0.7803336389566122
586.0511487667402 8.051310137804697 0.7902514545029246
586.0511487667402 10.216798589284712 0.8018653662233919
586.0511487667402 12.96471898702334 0.8153050866341481
586.0511487667402 16.451722811563343 0.8306635063307718
586.0511487667402 20.87659468280201 0.8479842216977249
586.0511487667402 26.491584531418546 0.8672489490905215
586.0511487667402 33.616787682496685 0.8883650264924066
586.0511487667402 42.65839262086404 0.9111533020619069
586.0511487667402 54.13183669370275 0.9353370424183044
586.0511487667402 68.69118979416318 0.9605330380602458
586.0511487667402 87.16644110999944 0.9862467939479734
586.0511487667402 110.6108145535225 1.0118745407163254
586.0511487667402 140.3608101970589 1.036715768788047
586.0511487667402 178.11239451312218 1.0600008207551461
586.0511487667402 226.01768281801222 1.0809379924529074
586.0511487667402 286.807625522434 1.0987821594739817
586.0511487667402 363.94769219915764 1.1129208498826517
586.0511487667402 461.8354285936932 1.1229644283423976
586.0511487667402 586.0511487667402 1.1288185616955702
586.0511487667402 743.6760536467558 1.1307156266479328
586.0511487667402 943.6959110675486 1.1291915774020587
586.0511487667402 1197.5133099937427 1.1250136256473855
586.0511487667402 1519.5976911565988 1.1190832408421816
586.0511487667402 1928.3102105817359 1.1123499313977088
586.0511487667402 2446.9504592387466 1.1057740858366785
586.0511487667402 3105.0847094578075 1.1003866314150657
586.0511487667402 3940.2314078349555 1.0975562589859944
586.0511487667402 5000.0 1.099890254934127

743.6760536467558 5.0 0.8261427842468126
743.6760536467558 6.344805015839611 0.8321022114940263
743.6760536467558 8.051310137804697 0.8392712380723761
743.6760536467558 10.216798589284712 0.8478106469172209
743.6760536467558 12.96471898702334 0.8578710060237519
743.6760536467558 16.451722811563343 0.8695827755642183
743.6760536467558 20.87659468280201 0.8830411514745661
743.6760536467558 26.491584531418546 0.8982933055351947
743.6760536467558 33.616787682496685 0.9153235614069177
743.6760536467558 42.65839262086404 0.9340387694990584
743.6760536467558 54.13183669370275 0.9542541192677919
743.6760536467558 68.69118979416318 0.9756803533257411
743.6760536467558 87.16644110999944 0.9979141745296232
743.6760536467558 110.6108145535225 1.0204347728727825
743.6760536467558 140.3608101970589 1.042610611992227
743.6760536467558 178.11239451312218 1.0637214396879666
743.6760536467558 226.01768281801222 1.0830001692485678
743.6760536467558 286.807625522434 1.0996968128703966
743.6760536467558 363.94769219915764 1.1131611915998045
743.6760536467558 461.8354285936932 1.1229330955039354
743.6760536467558 586.0511487667402 1.128820612024224
743.6760536467558 743.6760536467558 1.1309443759398217
743.6760536467558 943.6959110675486 1.1297319687154963
743.6760536467558 1197.5133099937427 1.125862451875427
743.6760536467558 1519.5976911565988 1.1201799788179747
743.6760536467558 1928.3102105817359 1.113609510324593
743.6760536467558 2446.9504592387466 1.1071148019034467
743.6760536467558 3105.0847094578075 1.1017516130028204
743.6760536467558 3940.2314078349555 1.098935385366993
743.6760536467558 5000.0 1.1013737510570716

943.6959110675486 5.0 0.8828282301823976
943.6959110675486 6.344805015839611 0.8868762747282393
943.6959110675486 8.051310137804697 0.8918095675643191
943.6959110675486 10.216798589284712 0.8977713004529111
943.6959110675486 12.96471898702334 0.9049069028402404
943.6959110675486 16.451722811563343 0.913355162107553
943.6959110675486 20.87659468280201 0.9232370410277959
943.6959110675486 26.491584531418546 0.934642427650001
943.6959110675486 33.616787682496685 0.9476153717108372
943.6959110675486 42.65839262086404 0.9621384547107373
943.6959110675486 54.13183669370275 0.97811629257795
943.6959110675486 68.69118979416318 0.9953629733026923
943.6959110675486 87.16644110999944 1.0135857407585143
943.6959110675486 110.6108145535225 1.032378510685358
943.6959110675486 140.3608101970589 1.0512208707589212
943.6959110675486 178.11239451312218 1.0694903532856304
943.6959110675486 226.01768281801222 1.0864927315351813
943.6959110675486 286.807625522434 1.101514089737039
943.6959110675486 363.94769219915764 1.1138940954356904
943.6959110675486 461.8354285936932 1.123112667196806
943.6959110675486 586.0511487667402 1.1288739918207131
943.6959110675486 743.6760536467558 1.131166548562621
943.6959110675486 943.6959110675486 1.13028042267113
943.6959110675486 1197.5133099937427 1.1267752897329235
943.6959110675486 1519.5976911565988 1.121410801031652
943.6959110675486 1928.3102105817359 1.1150683864541775
943.6959110675486 2446.9504592387466 1.1087059005002626
943.6959110675486 3105.0847094578075 1.1034041107680619
943.6959110675486 3940.2314078349555 1.1006356083400912
943.6959110675486 5000.0 1.1032408466049828

1197.5133099937427 5.0 0.9371502202258065
1197.5133099937427 6.344805015839611 0.939788665216181
1197.5133099937427 8.051310137804697 0.9430365336038793
1197.5133099937427 10.216798589284712 0.9470072652302599
1197.5133099937427 12.96471898702334 0.951822721861014
1197.5133099937427 16.451722811563343 0.9576079828910271
1197.5133099937427 20.87659468280201 0.9644836830078384
1197.5133099937427 26.491584531418546 0.9725557550389482
1197.5133099937427 33.616787682496685 0.9819027659437332
1197.5133099937427 42.65839262086404 0.9925613373733682
1197.5133099937427 54.13183669370275 1.0045103911411053
1197.5133099937427 68.69118979416318 1.0176551767407722
1197.5133099937427 87.16644110999944 1.031812327711482
1197.5133099937427 110.6108145535225 1.0466977269614834
1197.5133099937427 140.3608101970589 1.0619198784713795
1197.5133099937427 178.11239451312218 1.0769826876085544
1197.5133099937427 226.01768281801222 1.0913025285521252
1197.5133099937427 286.807625522434 1.1042444010293375
1197.5133099937427 363.94769219915764 1.1151795638852129
1197.5133099937427 461.8354285936932 1.1235615626777806
1197.5133099937427 586.0511487667402 1.129009702020585
1197.5133099937427 743.6760536467558 1.1313817013858143
1197.5133099937427 943.6959110675486 1.1308151464096103
1197.5133099937427 1197.5133099937427 1.1277244910007815
1197.5133099937427 1519.5976911565988 1.1227561794425365
1197.5133099937427 1928.3102105817359 1.116724037234928
1197.5133099937427 2446.9504592387466 1.1105654317997942
1197.5133099937427 3105.0847094578075 1.1053832152598146
1197.5133099937427 3940.2314078349555 1.1027187272444037
1197.5133099937427 5000.0 1.1055873972866466

1519.5976911565988 5.0 0.9854416523269295
1519.5976911565988 6.344805015839611 0.9871025981042054
1519.5976911565988 8.051310137804697 0.9891626497881839
1519.5976911565988 10.216798589284712 0.9917038100199418
1519.5976911565988 12.96471898702334 0.9948179160571738
1519.5976911565988 16.451722811563343 0.9986043633311822
1519.5976911565988 20.87659468280201 1.00316594198429
1519.5976911565988 26.491584531418546 1.0086023756863376
1519.5976911565988 33.616787682496685 1.0150013250981904
1519.5976911565988 42.65839262086404 1.0224268862988737
1519.5976911565988 54.13183669370275 1.0309059692510072
1519.5976911565988 68.69118979416318 1.0404132878337664
1519.5976911565988 87.16644110999944 1.050855417540106
1519.5976911565988 110.6108145535225 1.0620589680473613
1519.5976911565988 140.3608101970589 1.0737567548493039
1519.5976911565988 178.11239451312218 1.0855851224469442
1519.5976911565988 226.01768281801222 1.0970891880155993
1519.5976911565988 286.807625522434 1.1077433844314621
1519.5976911565988 363.94769219915764 1.1169908802985795
1519.5976911565988 461.8354285936932 1.1243028938082846
1519.5976911565988 586.0511487667402 1.1292529229561898
1519.5976911565988 743.6760536467558 1.1315932078006772
1519.5976911565988 943.6959110675486 1.1313150331785915
1519.5976911565988 1197.5133099937427 1.1286754314977698
1519.5976911565988 1519.5976911565988 1.1241836294932344
1519.5976911565988 1928.3102105817359 1.1185595878403582
1519.5976911565988 2446.9504592387466 1.1127004590737817
1519.5976911565988 3105.0847094578075 1.1077242259520959
1519.5976911565988 3940.2314078349555 1.1052538943373578
1519.5976911565988 5000.0 1.1085416264026553

1928.3102105817359 5.0 1.0256989217891106
1928.3102105817359 6.344805015839611 1.026715861702579
1928.3102105817359 8.051310137804697 1.0279841644053516
1928.3102105817359 10.216798589284712 1.0295591862315887
1928.3102105817359 12.96471898702334 1.03150484394174
1928.3102105817359 16.451722811563343 1.0338930498921404
1928.3102105817359 20.87659468280201 1.0368019858090614
1928.3102105817359 26.491584531418546 1.0403127910636154
1928.3102105817359 33.616787682496685 1.0445042386752468
1928.3102105817359 42.65839262086404 1.0494450884131608
1928.3102105817359 54.13183669370275 1.0551840430488941
1928.3102105817359 68.69118979416318 1.0617367585228064
1928.3102105817359 87.16644110999944 1.0690750003566662
1928.3102105817359 110.6108145535225 1.0771088660089534
1928.3102105817359 140.3608101970589 1.0856763595622594
1928.3102105817359 178.11239451312218 1.0945337020101147
1928.3102105817359 226.01768281801222 1.1033527828366603
1928.3102105817359 286.807625522434 1.1117290773973554
1928.3102105817359 363.94769219915764 1.119204310628323
1928.3102105817359 461.8354285936932 1.1253070471842495
1928.3102105817359 586.0511487667402 1.1296111079996183
1928.3102105817359 743.6760536467558 1.131805584536806
1928.3102105817359 943.6959110675486 1.1317634261780485
1928.3102105817359 1197.5133099937427 1.129591663261568
1928.3102105817359 1519.5976911565988 1.125650483822319
1928.3102105817359 1928.3102105817359 1.1205431536261754
1928.3102105817359 2446.9504592387466 1.1151042309034676
1928.3102105817359 3105.0847094578075 1.110456266137342
1928.3102105817359 3940.2314078349555 1.108319557483893
1928.3102105817359 5000.0 1.1122734538006036

2446.9504592387466 5.0 1.0574558923139374
2446.9504592387466 6.344805015839611 1.058065331014446
2446.9504592387466 8.051310137804697 1.058828476779387
2446.9504592387466 10.216798589284712 1.059780876372542
2446.9504592387466 12.96471898702334 1.0609644938663398
2446.9504592387466 16.451722811563343 1.062427892056422
2446.9504592387466 20.87659468280201 1.0642258174566772
2446.9504592387466 26.491584531418546 1.0664178598560436
2446.9504592387466 33.616787682496685 1.0690658109316211
2446.9504592387466 42.65839262086404 1.072229318625083
2446.9504592387466 54.13183669370275 1.0759595209263018
2446.9504592387466 68.69118979416318 1.0802895791558056
2446.9504592387466 87.16644110999944 1.0852273168209092
2446.9504592387466 110.6108145535225 1.0907389674609373
2446.9504592387466 140.3608101970589 1.0967394194183098
2446.9504592387466 178.11239451312218 1.1030805883498387
2446.9504592387466 226.01768281801222 1.1095440009287356
2446.9504592387466 286.807625522434 1.1158400052721476
2446.9504592387466 363.94769219915764 1.1216174015933844
2446.9504592387466 461.8354285936932 1.1264872036040958
2446.9504592387466 586.0511487667402 1.1300631527595735
2446.9504592387466 743.6760536467558 1.132018000087337
2446.9504592387466 943.6959110675486 1.1321490070846212
2446.9504592387466 1197.5133099937427 1.1304404383447346
2446.9504592387466 1519.5976911565988 1.1271094907355956
2446.9504592387466 1928.3102105817359 1.1226305718891507
2446.9504592387466 2446.9504592387466 1.117756138045249
2446.9504592387466 3105.0847094578075 1.113602451440792
2446.9504592387466 3940.2314078349555 1.1120104800822233
2446.9504592387466 5000.0 1.1170315677253266

3105.0847094578075 5.0 1.0813162136534036
3105.0847094578075 6.344805015839611 1.0816756663768097
3105.0847094578075 8.051310137804697 1.0821270965795433
3105.0847094578075 10.216798589284712 1.082692527286945
3105.0847094578075 12.96471898702334 1.0833983780145375
3105.0847094578075 16.451722811563343 1.08427585702459
3105.0847094578075 20.87659468280201 1.0853610840672334
3105.0847094578075 26.491584531418546 1.0866947463344125
3105.0847094578075 33.616787682496685 1.0883210253908675
3105.0847094578075 42.65839262086404 1.0902854591528826
3105.0847094578075 54.13183669370275 1.092631399768937
3105.0847094578075 68.69118979416318 1.0953939228011296
3105.0847094578075 87.16644110999944 1.0985955570098704
3105.0847094578075 110.6108145535225 1.102233500263237
3105.0847094578075 140.3608101970589 1.1062717148769452
3105.0847094578075 178.11239451312218 1.110629868724373
3105.0847094578075 226.01768281801222 1.1151741116018812
3105.0847094578075 286.807625522434 1.1197114257206366
3105.0847094578075 363.94769219915764 1.123990524454887
3105.0847094578075 461.8354285936932 1.1277127873889365
3105.0847094578075 586.0511487667402 1.1305567559629561
3105.0847094578075 743.6760536467558 1.1322181943386715
3105.0847094578075 943.6959110675486 1.1324645995702394
3105.0847094578075 1197.5133099937427 1.131198194100924
3105.0847094578075 1519.5976911565988 1.1285179107348007
3105.0847094578075 1928.3102105817359 1.1247740754818623
3105.0847094578075 2446.9504592387466 1.1206285182253168
3105.0847094578075 3105.0847094578075 1.11718816430772
3105.0847094578075 3940.2314078349555 1.116459403575446
3105.0847094578075 5000.0 1.1232236862366203

3940.2314078349555 5.0 1.0984362074741785
3940.2314078349555 6.344805015839611 1.098645935732222
3940.2314078349555 8.051310137804697 1.0989098940210011
3940.2314078349555 10.216798589284712 1.0992413951272848
3940.2314078349555 12.96471898702334 1.0996565976043147
3940.2314078349555 16.451722811563343 1.100174877307587
3940.2314078349555 20.87659468280201 1.100819095472847
3940.2314078349555 26.491584531418546 1.1016156569228674
3940.2314078349555 33.616787682496685 1.1025941976771032
3940.2314078349555 42.65839262086404 1.103786689159412
3940.2314078349555 54.13183669370275 1.1052256827093807
3940.2314078349555 68.69118979416318 1.1069407341931008
3940.2314078349555 87.16644110999944 1.1089563796129362
3940.2314078349555 110.6108145535225 1.1112831282223117
3940.2314078349555 140.3608101970589 1.113911873742186
3940.2314078349555 178.11239451312218 1.1168049276688972
3940.2314078349555 226.01768281801222 1.1198872990005762
3940.2314078349555 286.807625522434 1.1230393178729754
3940.2314078349555 363.94769219915764 1.1260927987784513
3940.2314078349555 461.8354285936932 1.1288336187947696
3940.2314078349555 586.0511487667402 1.1310140834053424
3940.2314078349555 743.6760536467558 1.1323783805855796
3940.2314078349555 943.6959110675486 1.1327032086348596
3940.2314078349555 1197.5133099937427 1.1318531641953902
3940.2314078349555 1519.5976911565988 1.129847596492456
3940.2314078349555 1928.3102105817359 1.1269371256346954
3940.2314078349555 2446.9504592387466 1.1237045380436474
3940.2314078349555 3105.0847094578075 1.1212672216131037
3940.2314078349555 3940.2314078349555 1.1218966668342287
3940.2314078349555 5000.0 1.1316313173688257

5000.0 5.0 1.1101205142448738
5000.0 6.344805015839611 1.1102423378930575
5000.0 8.051310137804697 1.1103959048583676
5000.0 10.216798589284712 1.1105891521468882
5000.0 12.96471898702334 1.110831796619511
5000.0 16.451722811563343 1.1111356202654334
5000.0 20.87659468280201 1.111514724879138
5000.0 26.491584531418546 1.111985703395677
5000.0 33.616787682496685 1.1125676407918632
5000.0 42.65839262086404 1.1132818164574292
5000.0 54.13183669370275 1.11415093637402
5000.0 68.69118979416318 1.11519767097057
5000.0 87.16644110999944 1.1164414676151282
5000.0 110.6108145535225 1.1178977051577725
5000.0 140.3608101970589 1.1195691827837266
5000.0 178.11239451312218 1.121442194273797
5000.0 226.01768281801222 1.123479053443122
5000.0 286.807625522434 1.1256111337548833
5000.0 363.94769219915764 1.127733381029226
5000.0 461.8354285936932 1.129702449264443
5000.0 586.0511487667402 1.1313413193884796
5000.0 743.6760536467558 1.1324538398832444
5000.0 943.6959110675486 1.1328528182858772
5000.0 1197.5133099937427 1.1324048805786786
5000.0 1519.5976911565988 1.1310950280305363
5000.0 1928.3102105817359 1.129117092155066
5000.0 2446.9504592387466 1.127016141674475
5000.0 3105.0847094578075 1.125990353347266
5000.0 3940.2314078349555 1.1288177691374999
5000.0 5000.0 1.1440779302124306


==> 5_Results/Figures/Mixture_qeff_IOM.tex <==
x y z

5.0 5.0 -245.78759606726635
5.0 6.344805015839611 -243.16856769567949
5.0 8.051310137804697 -240.7139560723963
5.0 10.216798589284712 -238.35774470239357
5.0 12.96471898702334 -236.02016048907626
5.0 16.451722811563343 -233.60073579434356
5.0 20.87659468280201 -230.9688006087472
5.0 26.491584531418546 -227.95060623104973
5.0 33.616787682496685 -224.3122211808468
5.0 42.65839262086404 -219.73749273615476
5.0 54.13183669370275 -213.80098005776154
5.0 68.69118979416318 -205.93721734614337
5.0 87.16644110999944 -195.41040888614043
5.0 110.6108145535225 -181.29287308010908
5.0 140.3608101970589 -162.46549673014124
5.0 178.11239451312218 -137.6562511563534
5.0 226.01768281801222 -105.52836198239856
5.0 286.807625522434 -64.81308696399628
5.0 363.94769219915764 -14.455003623318134
5.0 461.8354285936932 46.28657785621226
5.0 586.0511487667402 117.84012122060767
5.0 743.6760536467558 200.4665774585569
5.0 943.6959110675486 294.5557301995427
5.0 1197.5133099937427 401.07759956011887
5.0 1519.5976911565988 522.2353464386879
5.0 1928.3102105817359 662.4890544081595
5.0 2446.9504592387466 830.4115607632239
5.0 3105.0847094578075 1042.6120214157627
5.0 3940.2314078349555 1333.424343075265
5.0 5000.0 1783.810420836976

6.344805015839611 5.0 -251.38166815790737
6.344805015839611 6.344805015839611 -248.1450285416313
6.344805015839611 8.051310137804697 -245.1343599689135
6.344805015839611 10.216798589284712 -242.27758282954846
6.344805015839611 12.96471898702334 -239.48928120986875
6.344805015839611 16.451722811563343 -236.66376635517872
6.344805015839611 20.87659468280201 -233.66556703316064
6.344805015839611 26.491584531418546 -230.3165536189399
6.344805015839611 33.616787682496685 -226.3788426587912
6.344805015839611 42.65839262086404 -221.5327819094582
6.344805015839611 54.13183669370275 -215.3499279623079
6.344805015839611 68.69118979416318 -207.2623775760062
6.344805015839611 87.16644110999944 -196.53254756552178
6.344805015839611 110.6108145535225 -182.2316940422411
6.344805015839611 140.3608101970589 -163.24037811891412
6.344805015839611 178.11239451312218 -138.28685230871088
6.344805015839611 226.01768281801222 -106.03489529094622
6.344805015839611 286.807625522434 -65.21606758448706
6.344805015839611 363.94769219915764 -14.774444625556953
6.344805015839611 461.8354285936932 46.032310112983396
6.344805015839611 586.0511487667402 117.63539530636899
6.344805015839611 743.6760536467558 200.29916257004743
6.344805015839611 943.6959110675486 294.4168977071299
6.344805015839611 1197.5133099937427 400.96177873678334
6.344805015839611 1519.5976911565988 522.1396081186399
6.344805015839611 1928.3102105817359 662.4127352077744
6.344805015839611 2446.9504592387466 830.3563706154755
6.344805015839611 3105.0847094578075 1042.5832275647963
6.344805015839611 3940.2314078349555 1333.4347627995821
6.344805015839611 5000.0 1783.8942101816747

8.051310137804697 5.0 -258.3886390145849
8.051310137804697 6.344805015839611 -254.38699810860953
8.051310137804697 8.051310137804697 -250.6856349179161
8.051310137804697 10.216798589284712 -247.20553546976544
8.051310137804697 12.96471898702334 -243.8547363693183
8.051310137804697 16.451722811563343 -240.52141705691247
8.051310137804697 20.87659468280201 -237.06441035767148
8.051310137804697 26.491584531418546 -233.30034562982564
8.051310137804697 33.616787682496685 -228.98657948504433
8.051310137804697 42.65839262086404 -223.79922294122343
8.051310137804697 54.13183669370275 -217.30618531147275
8.051310137804697 68.69118979416318 -208.9365996669394
8.051310137804697 87.16644110999944 -197.95071610886407
8.051310137804697 110.6108145535225 -183.4185206297243
8.051310137804697 140.3608101970589 -164.22021855184084
8.051310137804697 178.11239451312218 -139.08445950912528
8.051310137804697 226.01768281801222 -106.67575122782864
8.051310137804697 286.807625522434 -65.7260580235261
8.051310137804697 363.94769219915764 -15.178835823280224
8.051310137804697 461.8354285936932 45.710322070186066
8.051310137804697 586.0511487667402 117.37606306976295
8.051310137804697 743.6760536467558 200.08703211306965
8.051310137804697 943.6959110675486 294.2409398024688
8.051310137804697 1197.5133099937427 400.81495643272274
8.051310137804697 1519.5976911565988 522.0182259668
8.051310137804697 1928.3102105817359 662.3159661386894
8.051310137804697 2446.9504592387466 830.2863951624686
8.051310137804697 3105.0847094578075 1042.5467386407927
8.051310137804697 3940.2314078349555 1333.4480355389223
8.051310137804697 5000.0 1784.0006086952035

10.216798589284712 5.0 -267.13530116266884
10.216798589284712 6.344805015839611 -262.19225394440537
10.216798589284712 8.051310137804697 -257.6378855681419
10.216798589284712 10.216798589284712 -253.38553802905153
10.216798589284712 12.96471898702334 -249.33587836937795
10.216798589284712 16.451722811563343 -245.37006550846354
10.216798589284712 20.87659468280201 -241.34031864422104
10.216798589284712 26.491584531418546 -237.0571116061028
10.216798589284712 33.616787682496685 -232.27215916020032
10.216798589284712 42.65839262086404 -226.65651592800805
10.216798589284712 54.13183669370275 -219.7737190931207
10.216798589284712 68.69118979416318 -211.04934483788566
10.216798589284712 87.16644110999944 -199.74105418323688
10.216798589284712 110.6108145535225 -184.9173446521063
10.216798589284712 140.3608101970589 -165.4580611743445
10.216798589284712 178.11239451312218 -140.0924212156151
10.216798589284712 226.01768281801222 -107.4859008763633
10.216798589284712 286.807625522434 -66.37100805758428
10.216798589284712 363.94769219915764 -15.690440665040114
10.216798589284712 461.8354285936932 45.3028038782636
10.216798589284712 586.0511487667402 117.04771444439757
10.216798589284712 743.6760536467558 199.81834889115817
10.216798589284712 943.6959110675486 294.0180018088695
10.216798589284712 1197.5133099937427 400.6288854920467
10.216798589284712 1519.5976911565988 521.8643672930793
10.216798589284712 1928.3102105817359 662.1932938678974
10.216798589284712 2446.9504592387466 830.1976934881241
10.216798589284712 3105.0847094578075 1042.5005150558727
10.216798589284712 3940.2314078349555 1333.4649594663815
10.216798589284712 5000.0 1784.1357420062805

12.96471898702334 5.0 -278.00659153826973
12.96471898702334 6.344805015839611 -271.91461143971674
12.96471898702334 8.051310137804697 -266.31446084465415
12.96471898702334 10.216798589284712 -261.11151066059483
12.96471898702334 12.96471898702334 -256.1984937064776
12.96471898702334 16.451722811563343 -251.4488171553976
12.96471898702334 20.87659468280201 -246.70724873790414
12.96471898702334 26.491584531418546 -241.7772140989423
12.96471898702334 33.616787682496685 -236.40388573430482
12.96471898702334 42.65839262086404 -230.25239963167132
12.96471898702334 54.13183669370275 -222.88114504528312
12.96471898702334 68.69118979416318 -213.71150423506333
12.96471898702334 87.16644110999944 -201.9981048738382
12.96471898702334 110.6108145535225 -186.8077498040293
12.96471898702334 140.3608101970589 -167.0199703045655
12.96471898702334 178.11239451312218 -141.36480529448136
12.96471898702334 226.01768281801222 -108.50902807423608
12.96471898702334 286.807625522434 -67.18588577380524
12.96471898702334 363.94769219915764 -16.33715914343429
12.96471898702334 461.8354285936932 44.78739886079438
12.96471898702334 586.0511487667402 116.63223056842435
12.96471898702334 743.6760536467558 199.47820646341506
12.96471898702334 943.6959110675486 293.73565754328456
12.96471898702334 1197.5133099937427 400.39315576911895
12.96471898702334 1519.5976911565988 521.6694008207792
12.96471898702334 1928.3102105817359 662.0378268171648
12.96471898702334 2446.9504592387466 830.0852864774151
12.96471898702334 3105.0847094578075 1042.441986982365
12.96471898702334 3940.2314078349555 1333.4865662382635
12.96471898702334 5000.0 1784.3074105771084

16.451722811563343 5.0 -291.4457300928252
16.451722811563343 6.344805015839611 -283.96622258793104
16.451722811563343 8.051310137804697 -277.0957975045749
16.451722811563343 10.216798589284712 -270.7322423476112
16.451722811563343 12.96471898702334 -264.7603215593681
16.451722811563343 16.451722811563343 -259.04533715121806
16.451722811563343 20.87659468280201 -253.4240219584667
16.451722811563343 26.491584531418546 -247.69201867131733
16.451722811563343 33.616787682496685 -241.58714316871647
16.451722811563343 42.65839262086404 -234.76778799008434
16.451722811563343 54.13183669370275 -226.78642917587604
16.451722811563343 68.69118979416318 -217.05962579156358
16.451722811563343 87.16644110999944 -204.83854835916964
16.451722811563343 110.6108145535225 -189.1881535861903
16.451722811563343 140.3608101970589 -168.98780003932188
16.451722811563343 178.11239451312218 -142.9687274709372
16.451722811563343 226.01768281801222 -109.79946283081517
16.451722811563343 286.807625522434 -68.214269351236
16.451722811563343 363.94769219915764 -17.15383493409945
16.451722811563343 461.8354285936932 44.13612560352294
16.451722811563343 586.0511487667402 116.10688604722327
16.451722811563343 743.6760536467558 199.0478722531402
16.451722811563343 943.6959110675486 293.3782651887932
16.451722811563343 1197.5133099937427 400.0946456093375
16.451722811563343 1519.5976911565988 521.4224365928626
16.451722811563343 1928.3102105817359 661.8408655890157
16.451722811563343 2446.9504592387466 829.9428907884958
16.451722811563343 3105.0847094578075 1042.367922892774
16.451722811563343 3940.2314078349555 1333.5141952637696
16.451722811563343 5000.0 1784.5255568504235

20.87659468280201 5.0 -307.94740590093943
20.87659468280201 6.344805015839611 -298.81449618810257
20.87659468280201 8.051310137804697 -290.41920768532464
20.87659468280201 10.216798589284712 -282.6533073530354
20.87659468280201 12.96471898702334 -275.3944825023027
20.87659468280201 16.451722811563343 -268.5002858497746
20.87659468280201 20.87659468280201 -261.79935935465164
20.87659468280201 26.491584531418546 -255.07920716018725
20.87659468280201 33.616787682496685 -248.06973742489527
20.87659468280201 42.65839262086404 -240.42195290227255
20.87659468280201 54.13183669370275 -231.6817761669472
20.87659468280201 68.69118979416318 -221.26040996423262
20.87659468280201 87.16644110999944 -208.40524871221623
20.87659468280201 110.6108145535225 -192.1793776133377
20.87659468280201 140.3608101970589 -171.46228673724727
20.87659468280201 178.11239451312218 -144.98698669524492
20.87659468280201 226.01768281801222 -111.42439782966585
20.87659468280201 286.807625522434 -69.51019529880614
20.87659468280201 363.94769219915764 -18.18379237955969
20.87659468280201 461.8354285936932 43.31409504826388
20.87659468280201 586.0511487667402 115.44326850004563
20.87659468280201 743.6760536467558 198.50386770213663
20.87659468280201 943.6959110675486 292.92617817791916
20.87659468280201 1197.5133099937427 399.71684570704883
20.87659468280201 1519.5976911565988 521.1097563292228
20.87659468280201 1928.3102105817359 661.591444391157
20.87659468280201 2446.9504592387466 829.7625892625774
20.87659468280201 3105.0847094578075 1042.2742695155057
20.87659468280201 3940.2314078349555 1333.5495949464112
20.87659468280201 5000.0 1784.80286825844

26.491584531418546 5.0 -328.03999560396824
26.491584531418546 6.344805015839611 -316.97011848748207
26.491584531418546 8.051310137804697 -306.77158917560155
26.491584531418546 10.216798589284712 -297.33346948833423
26.491584531418546 12.96471898702334 -288.52870912646586
26.491584531418546 16.451722811563343 -280.2086367118627
26.491584531418546 20.87659468280201 -272.19467011294364
26.491584531418546 26.491584531418546 -264.26653174709236
26.491584531418546 33.616787682496685 -256.1462110485254
26.491584531418546 42.65839262086404 -247.47708123454413
26.491584531418546 54.13183669370275 -237.7981827789722
26.491584531418546 68.69118979416318 -226.51508666757263
26.491584531418546 87.16644110999944 -212.87132737699767
26.491584531418546 110.6108145535225 -195.9283402428273
26.491584531418546 140.3608101970589 -174.56632274959065
26.491584531418546 178.11239451312218 -147.52091434543127
26.491584531418546 226.01768281801222 -113.46633293096147
26.491584531418546 286.807625522434 -71.14023633312763
26.491584531418546 363.94769219915764 -19.48059665063647
26.491584531418546 461.8354285936932 42.27801566308881
26.491584531418546 586.0511487667402 114.60599990278115
26.491584531418546 743.6760536467558 197.81686514416197
26.491584531418546 943.6959110675486 292.35478858071474
26.491584531418546 1197.5133099937427 399.2390326392406
26.491584531418546 1519.5976911565988 520.7141131899416
26.491584531418546 1928.3102105817359 661.275765731185
26.491584531418546 2446.9504592387466 829.5344254777519
26.491584531418546 3105.0847094578075 1042.1559596172983
26.491584531418546 3940.2314078349555 1333.5950624162915
26.491584531418546 5000.0 1785.1555589095442

33.616787682496685 5.0 -352.25197362121526
33.616787682496685 6.344805015839611 -338.9616704118516
33.616787682496685 8.051310137804697 -326.6709985262337
33.616787682496685 10.216798589284712 -315.2720065889612
33.616787682496685 12.96471898702334 -304.63730910705726
33.616787682496685 16.451722811563343 -294.61528281923484
33.616787682496685 20.87659468280201 -285.022435310309
33.616787682496685 26.491584531418546 -275.6322396558935
33.616787682496685 33.616787682496685 -266.15969665886814
33.616787682496685 42.65839262086404 -256.2410589210317
33.616787682496685 54.13183669370275 -245.4087606206317
33.616787682496685 68.69118979416318 -233.06296829850635
33.616787682496685 87.16644110999944 -218.44372343528403
33.616787682496685 110.6108145535225 -200.61146696049127
33.616787682496685 140.3608101970589 -178.44811679746545
33.616787682496685 178.11239451312218 -150.69323096079415
33.616787682496685 226.01768281801222 -116.02561089711207
33.616787682496685 286.807625522434 -73.18572529357698
33.616787682496685 363.94769219915764 -21.10999259338996
33.616787682496685 461.8354285936932 40.97450369610442
33.616787682496685 586.0511487667402 113.55125841523022
33.616787682496685 743.6760536467558 196.95038860697923
33.616787682496685 943.6959110675486 291.63338373781517
33.616787682496685 1197.5133099937427 398.6352701237047
33.616787682496685 1519.5976911565988 520.2138791265079
33.616787682496685 1928.3102105817359 660.8765102820807
33.616787682496685 2446.9504592387466 829.2459097013389
33.616787682496685 3105.0847094578075 1042.006685523972
33.616787682496685 3940.2314078349555 1333.653638968467
33.616787682496685 5000.0 1785.604388154633

42.65839262086404 5.0 -381.0575883080646
42.65839262086404 6.344805015839611 -365.291789335834
42.65839262086404 8.051310137804697 -350.63218671897266
42.65839262086404 10.216798589284712 -336.9823907439363
42.65839262086404 12.96471898702334 -324.2217396135525
42.65839262086404 16.451722811563343 -312.2013031802194
42.65839262086404 20.87659468280201 -300.73705736606644
42.65839262086404 26.491584531418546 -289.59951647554726
42.65839262086404 33.616787682496685 -278.4990974187349
42.65839262086404 42.65839262086404 -267.0666671809913
42.65839262086404 54.13183669370275 -254.8293479232575
42.65839262086404 68.69118979416318 -241.1830030859287
42.65839262086404 87.16644110999944 -225.36531808928157
42.65839262086404 110.6108145535225 -206.4371092534161
42.65839262086404 140.3608101970589 -183.28370944568815
42.65839262086404 178.11239451312218 -154.650524798089
42.65839262086404 226.01768281801222 -119.2227757301539
42.65839262086404 286.807625522434 -75.74494774085133
42.65839262086404 363.94769219915764 -23.15191338966997
42.65839262086404 461.8354285936932 39.33825813100202
42.65839262086404 586.0511487667402 112.22512640614423
42.65839262086404 743.6760536467558 195.85932196078238
42.65839262086404 943.6959110675486 290.7238059120177
42.65839262086404 1197.5133099937427 397.87322029913594
42.65839262086404 1519.5976911565988 519.5820197502999
42.65839262086404 1928.3102105817359 660.3719992503948
42.65839262086404 2446.9504592387466 828.8814245872618
42.65839262086404 3105.0847094578075 1041.8186396639467
42.65839262086404 3940.2314078349555 1333.729387232248
42.65839262086404 5000.0 1786.1759961648568

54.13183669370275 5.0 -414.7983144441382
54.13183669370275 6.344805015839611 -396.370378700678
54.13183669370275 8.051310137804697 -379.1110919458424
54.13183669370275 10.216798589284712 -362.9471949452022
54.13183669370275 12.96471898702334 -347.7748180384674
54.13183669370275 16.451722811563343 -333.45625277319414
54.13183669370275 20.87659468280201 -319.81398681993187
54.13183669370275 26.491584531418546 -306.621260933965
54.13183669370275 33.616787682496685 -293.5884149712733
54.13183669370275 42.65839262086404 -280.34449076061355
54.13183669370275 54.13183669370275 -266.4141740806681
54.13183669370275 68.69118979416318 -251.19149972966534
54.13183669370275 87.16644110999944 -233.91415711268792
54.13183669370275 110.6108145535225 -213.64582135259843
54.13183669370275 140.3608101970589 -189.27796291691857
54.13183669370275 178.11239451312218 -159.56469760764503
54.13183669370275 226.01768281801222 -123.20028381598058
54.13183669370275 286.807625522434 -78.93497965070765
54.13183669370275 363.94769219915764 -25.70234713579839
54.13183669370275 461.8354285936932 37.290230434362
54.13183669370275 586.0511487667402 110.56183719347064
54.13183669370275 743.6760536467558 194.4882580392432
54.13183669370275 943.6959110675486 289.57892336333043
54.13183669370275 1197.5133099937427 396.9127585453871
54.13183669370275 1519.5976911565988 518.7848830058465
54.13183669370275 1928.3102105817359 659.7352063302947
54.13183669370275 2446.9504592387466 828.4215229539386
54.13183669370275 3105.0847094578075 1041.5822300272503
54.13183669370275 3940.2314078349555 1333.8277898175565
54.13183669370275 5000.0 1786.904668401523

68.69118979416318 5.0 -453.58036938994974
68.69118979416318 6.344805015839611 -432.4228689348756
68.69118979416318 8.051310137804697 -412.42469365771603
68.69118979416318 10.216798589284712 -393.54963596832704
68.69118979416318 12.96471898702334 -375.7234807807881
68.69118979416318 16.451722811563343 -358.83127533174866
68.69118979416318 20.87659468280201 -342.71209178015806
68.69118979416318 26.491584531418546 -327.15050086719384
68.69118979416318 33.616787682496685 -311.86399831135486
68.69118979416318 42.65839262086404 -296.4858453168408
68.69118979416318 54.13183669370275 -280.54340396303724
68.69118979416318 68.69118979416318 -263.43336436725303
68.69118979416318 87.16644110999944 -244.39759188129938
68.69118979416318 110.6108145535225 -222.50674989073923
68.69118979416318 140.3608101970589 -196.66266350144906
68.69118979416318 178.11239451312218 -165.63234483125598
68.69118979416318 226.01768281801222 -128.12280905755688
68.69118979416318 286.807625522434 -82.89263216593417
68.69118979416318 363.94769219915764 -28.87469406025457
68.69118979416318 461.8354285936932 34.73602887466359
68.69118979416318 586.0511487667402 108.48206869131536
68.69118979416318 743.6760536467558 192.76977340943404
68.69118979416318 943.6959110675486 288.14095502139526
68.69118979416318 1197.5133099937427 395.7044070804891
68.69118979416318 1519.5976911565988 517.7808021743144
68.69118979416318 1928.3102105817359 658.9326002056691
68.69118979416318 2446.9504592387466 827.842119076272
68.69118979416318 3105.0847094578075 1041.2857904944367
68.69118979416318 3940.2314078349555 1333.9563306847585
68.69118979416318 5000.0 1787.8346875592179

87.16644110999944 5.0 -497.1551171371225
87.16644110999944 6.344805015839611 -473.37666355675765
87.16644110999944 8.051310137804697 -450.6463802981975
87.16644110999944 10.216798589284712 -428.97964416212244
87.16644110999944 12.96471898702334 -408.34640776390734
87.16644110999944 16.451722811563343 -388.66838656895015
87.16644110999944 20.87659468280201 -369.8141459116305
87.16644110999944 26.491584531418546 -351.5912552858008
87.16644110999944 33.616787682496685 -333.73471522120644
87.16644110999944 42.65839262086404 -315.8910949487622
87.16644110999944 54.13183669370275 -297.59843866284064
87.16644110999944 68.69118979416318 -278.26327954052886
87.16644110999944 87.16644110999944 -257.1383321253147
87.16644110999944 110.6108145535225 -233.30767221330234
87.16644110999944 140.3608101970589 -205.6897722059398
87.16644110999944 178.11239451312218 -173.0705488573485
87.16644110999944 226.01768281801222 -134.17499871059317
87.16644110999944 286.807625522434 -87.7736704196036
87.16644110999944 363.94769219915764 -32.800027212672376
87.16644110999944 461.8354285936932 31.564957814823174
87.16644110999944 586.0511487667402 105.89154726575634
87.16644110999944 743.6760536467558 190.62279446832645
87.16644110999944 943.6959110675486 286.3397473063742
87.16644110999944 1197.5133099937427 394.1876415666825
87.16644110999944 1519.5976911565988 516.5185407644599
87.16644110999944 1928.3102105817359 657.9228447596215
87.16644110999944 2446.9504592387466 827.11359275002
87.16644110999944 3105.0847094578075 1040.915327071426
87.16644110999944 3940.2314078349555 1334.1253543409603
87.16644110999944 5000.0 1789.0235013558413

110.6108145535225 5.0 -544.7979514463241
110.6108145535225 6.344805015839611 -518.7366718980779
110.6108145535225 8.051310137804697 -493.4834897388632
110.6108145535225 10.216798589284712 -469.1174978729632
110.6108145535225 12.96471898702334 -445.6666255580826
110.6108145535225 16.451722811563343 -423.1038390134431
110.6108145535225 20.87659468280201 -401.3418283135761
110.6108145535225 26.491584531418546 -380.2253065598734
110.6108145535225 33.616787682496685 -359.52009231579177
110.6108145535225 42.65839262086404 -338.8983837015626
110.6108145535225 54.13183669370275 -317.92024106349027
110.6108145535225 68.69118979416318 -296.0125255684534
110.6108145535225 87.16644110999944 -272.44864828574146
110.6108145535225 110.6108145535225 -246.3355011072349
110.6108145535225 140.3608101970589 -216.61721586267777
110.6108145535225 178.11239451312218 -182.10701249135263
110.6108145535225 226.01768281801222 -141.55508058368332
110.6108145535225 286.807625522434 -93.74910805409809
110.6108145535225 363.94769219915764 -37.62538334934061
110.6108145535225 461.8354285936932 27.65031110488235
110.6108145535225 586.0511487667402 102.68038913823466
110.6108145535225 743.6760536467558 187.951341923585
110.6108145535225 943.6959110675486 284.0911900194096
110.6108145535225 1197.5133099937427 392.28918893838954
110.6108145535225 1519.5976911565988 514.9356537207186
110.6108145535225 1928.3102105817359 656.6554045851417
110.6108145535225 2446.9504592387466 826.1998566558514
110.6108145535225 3105.0847094578075 1040.454376836772
110.6108145535225 3940.2314078349555 1334.349351505536
110.6108145535225 5000.0 1790.546040504828

140.3608101970589 5.0 -595.2108378954572
140.3608101970589 6.344805015839611 -567.4702506085364
140.3608101970589 8.051310137804697 -540.1525075995501
140.3608101970589 10.216798589284712 -513.4059069224063
140.3608101970589 12.96471898702334 -487.32583285713645
140.3608101970589 16.451722811563343 -461.9487824720918
140.3608101970589 20.87659468280201 -437.2456211486028
140.3608101970589 26.491584531418546 -413.1131654705928
140.3608101970589 33.616787682496685 -389.36327507343276
140.3608101970589 42.65839262086404 -365.7087927719899
140.3608101970589 54.13183669370275 -341.74634888532773
140.3608101970589 68.69118979416318 -316.9371281992662
140.3608101970589 87.16644110999944 -290.5886877290577
140.3608101970589 110.6108145535225 -261.8436606421228
140.3608101970589 140.3608101970589 -229.6841420944179
140.3608101970589 178.11239451312218 -192.96199042919397
140.3608101970589 226.01768281801222 -150.4622861606813
140.3608101970589 286.807625522434 -100.99699318464809
140.3608101970589 363.94769219915764 -43.508883425289696
140.3608101970589 461.8354285936932 22.851807690899022
140.3608101970589 586.0511487667402 98.72382193449539
140.3608101970589 743.6760536467558 184.64410913616803
140.3608101970589 943.6959110675486 281.29608810648097
140.3608101970589 1197.5133099937427 389.92153382774677
140.3608101970589 1519.5976911565988 512.9569155784047
140.3608101970589 1928.3102105817359 655.069169580011
140.3608101970589 2446.9504592387466 825.0574937454612
140.3608101970589 3105.0847094578075 1039.8841157799234
140.3608101970589 3940.2314078349555 1334.648904862298
140.3608101970589 5000.0 1792.5006846146598

178.11239451312218 5.0 -646.4821761102144
178.11239451312218 6.344805015839611 -617.9312761025603
178.11239451312218 8.051310137804697 -589.2772035419239
178.11239451312218 10.216798589284712 -560.7311526489698
178.11239451312218 12.96471898702334 -532.4563815985562
178.11239451312218 16.451722811563343 -504.55871733429603
178.11239451312218 20.87659468280201 -477.07710200598103
178.11239451312218 26.491584531418546 -449.97334002163734
178.11239451312218 33.616787682496685 -423.12021230437995
178.11239451312218 42.65839262086404 -396.2873185277731
178.11239451312218 54.13183669370275 -369.1246102106952
178.11239451312218 68.69118979416318 -341.14456872025403
178.11239451312218 87.16644110999944 -311.7057889929565
178.11239451312218 110.6108145535225 -280.00319347515597
178.11239451312218 140.3608101970589 -245.07269325220568
178.11239451312218 178.11239451312218 -205.8193957557687
178.11239451312218 226.01768281801222 -161.07584392112403
178.11239451312218 286.807625522434 -109.68783047126135
178.11239451312218 363.94769219915764 -50.61019263374055
178.11239451312218 461.8354285936932 17.021335586989153
178.11239451312218 586.0511487667402 93.88517862612662
178.11239451312218 743.6760536467558 180.57554349380234
178.11239451312218 943.6959110675486 277.8399837425518
178.11239451312218 1197.5133099937427 386.9819954249019
178.11239451312218 1519.5976911565988 510.49308333302815
178.11239451312218 1928.3102105817359 653.091309446404
178.11239451312218 2446.9504592387466 823.6351575221343
178.11239451312218 3105.0847094578075 1039.1839485362125
178.11239451312218 3940.2314078349555 1335.0536638450403
178.11239451312218 5000.0 1795.0176297542685

226.01768281801222 5.0 -696.14280993581
226.01768281801222 6.344805015839611 -667.8607062294468
226.01768281801222 8.051310137804697 -638.8441990138253
226.01768281801222 10.216798589284712 -609.3440659133848
226.01768281801222 12.96471898702334 -579.577485809501
226.01768281801222 16.451722811563343 -549.7138451955511
226.01768281801222 20.87659468280201 -519.8612758954
226.01768281801222 26.491584531418546 -490.0532563237166
226.01768281801222 33.616787682496685 -460.2345400800341
226.01768281801222 42.65839262086404 -430.2458357608716
226.01768281801222 54.13183669370275 -399.807131679489
226.01768281801222 68.69118979416318 -368.50050114296255
226.01768281801222 87.16644110999944 -335.75477958277406
226.01768281801222 110.6108145535225 -300.83662526570515
226.01768281801222 140.3608101970589 -262.85476319673853
226.01768281801222 178.11239451312218 -220.78528304621705
226.01768281801222 226.01768281801222 -173.52370142927884
226.01768281801222 286.807625522434 -119.96188590431211
226.01768281801222 363.94769219915764 -59.074746897126715
226.01768281801222 461.8354285936932 10.01335537243358
226.01768281801222 586.0511487667402 88.0222846742995
226.01768281801222 743.6760536467558 175.60933600963926
226.01768281801222 943.6959110675486 273.59464302159404
226.01768281801222 1197.5133099937427 383.3529326281482
226.01768281801222 1519.5976911565988 507.4404317986041
226.01768281801222 1928.3102105817359 650.6367187107326
226.01768281801222 2446.9504592387466 821.8735726849
226.01768281801222 3105.0847094578075 1038.332968606299
226.01768281801222 3940.2314078349555 1335.6069337074805
226.01768281801222 5000.0 1798.2708189845525

286.807625522434 5.0 -741.3527392007027
286.807625522434 6.344805015839611 -714.5036044200606
286.807625522434 8.051310137804697 -686.2572125468432
286.807625522434 10.216798589284712 -656.8609332583665
286.807625522434 12.96471898702334 -626.5531328524876
286.807625522434 16.451722811563343 -595.544301332709
286.807625522434 20.87659468280201 -563.9988382569686
286.807625522434 26.491584531418546 -532.0173791731359
286.807625522434 33.616787682496685 -499.61927510069245
286.807625522434 42.65839262086404 -466.7248260515694
286.807625522434 54.13183669370275 -433.1371953857938
286.807625522434 68.69118979416318 -398.52470327901983
286.807625522434 87.16644110999944 -362.40549933174725
286.807625522434 110.6108145535225 -324.1384165622403
286.807625522434 140.3608101970589 -282.92570838872416
286.807625522434 178.11239451312218 -237.83432175689677
286.807625522434 226.01768281801222 -187.84065721667184
286.807625522434 286.807625522434 -131.8974974509738
286.807625522434 363.94769219915764 -69.01058089933076
286.807625522434 461.8354285936932 1.701215172798129
286.807625522434 586.0511487667402 80.99844691108365
286.807625522434 743.6760536467558 169.60540951252824
286.807625522434 943.6959110675486 268.4221523608858
286.807625522434 1197.5133099937427 378.9038730271809
286.807625522434 1519.5976911565988 503.68172972775255
286.807625522434 1928.3102105817359 647.6086283156328
286.807625522434 2446.9504592387466 819.7066896474134
286.807625522434 3105.0847094578075 1037.3129244153315
286.807625522434 3940.2314078349555 1336.3728113990837
286.807625522434 5000.0 1802.4952572953443

363.94769219915764 5.0 -779.2257966418597
363.94769219915764 6.344805015839611 -754.8708504772426
363.94769219915764 8.051310137804697 -728.5300718761714
363.94769219915764 10.216798589284712 -700.3898369768895
363.94769219915764 12.96471898702334 -670.6585568103515
363.94769219915764 16.451722811563343 -639.5459873390996
363.94769219915764 20.87659468280201 -607.2414677504953
363.94769219915764 26.491584531418546 -573.8919759338164
363.94769219915764 33.616787682496685 -539.5804097910645
363.94769219915764 42.65839262086404 -504.3042221292394
363.94769219915764 54.13183669370275 -467.9545905112004
363.94769219915764 68.69118979416318 -430.2967932678098
363.94769219915764 87.16644110999944 -390.9534518627356
363.94769219915764 110.6108145535225 -349.393732378599
363.94769219915764 140.3608101970589 -304.93314920665625
363.94769219915764 178.11239451312218 -256.74945184679245
363.94769219915764 226.01768281801222 -203.91881762276398
363.94769219915764 286.807625522434 -145.47163344260935
363.94769219915764 363.94769219915764 -80.45787143179359
363.94769219915764 461.8354285936932 -8.000041985761527
363.94769219915764 586.0511487667402 72.69899615182385
363.94769219915764 743.6760536467558 162.43151027083877
363.94769219915764 943.6959110675486 262.18273457243276
363.94769219915764 1197.5133099937427 373.4966112190964
363.94769219915764 1519.5976911565988 499.08961006395293
363.94769219915764 1928.3102105817359 643.9012858806409
363.94769219915764 2446.9504592387466 817.0648721734924
363.94769219915764 3105.0847094578075 1036.1137136406405
363.94769219915764 3940.2314078349555 1337.4473617613075
363.94769219915764 5000.0 1808.0126223087755

461.8354285936932 5.0 -807.2379065115892
461.8354285936932 6.344805015839611 -786.1321007851025
461.8354285936932 8.051310137804697 -762.6357499527844
461.8354285936932 10.216798589284712 -736.8196768497355
461.8354285936932 12.96471898702334 -708.8036455526135
461.8354285936932 16.451722811563343 -678.7402189543886
461.8354285936932 20.87659468280201 -646.7941031015694
461.8354285936932 26.491584531418546 -613.1186799382149
461.8354285936932 33.616787682496685 -577.8311865082719
461.8354285936932 42.65839262086404 -540.9876346018464
461.8354285936932 54.13183669370275 -502.55833717312134
461.8354285936932 68.69118979416318 -462.405016752366
461.8354285936932 87.16644110999944 -420.2610329181798
461.8354285936932 110.6108145535225 -375.71725934678216
461.8354285936932 140.3608101970589 -328.2173108338611
461.8354285936932 178.11239451312218 -277.06653163938836
461.8354285936932 226.01768281801222 -221.45831388225542
461.8354285936932 286.807625522434 -160.51757865723675
461.8354285936932 363.94769219915764 -93.35378826329179
461.8354285936932 461.8354285936932 -19.105360081409344
461.8354285936932 586.0511487667402 63.053461965131646
461.8354285936932 743.6760536467558 153.98011565181878
461.8354285936932 943.6959110675486 254.7473508520725
461.8354285936932 1197.5133099937427 366.9944923263429
461.8354285936932 1519.5976911565988 493.5335932557423
461.8354285936932 1928.3102105817359 639.4059273786315
461.8354285936932 2446.9504592387466 813.8814673984107
461.8354285936932 3105.0847094578075 1034.7430303835336
461.8354285936932 3940.2314078349555 1338.9762422896647
461.8354285936932 5000.0 1815.2699220727864

586.0511487667402 5.0 -823.5964475715041
586.0511487667402 6.344805015839611 -806.055536591201
586.0511487667402 8.051310137804697 -785.9698282558998
586.0511487667402 10.216798589284712 -763.268084891638
586.0511487667402 12.96471898702334 -737.937639131464
586.0511487667402 16.451722811563343 -710.0195214098994
586.0511487667402 20.87659468280201 -679.5960978809999
586.0511487667402 26.491584531418546 -646.772284220116
586.0511487667402 33.616787682496685 -611.6520451402125
586.0511487667402 42.65839262086404 -574.3120844476562
586.0511487667402 54.13183669370275 -534.774547270229
586.0511487667402 68.69118979416318 -492.9804627370854
586.0511487667402 87.16644110999944 -448.7657946745808
586.0511487667402 110.6108145535225 -401.8424485617684
586.0511487667402 140.3608101970589 -351.78729727030986
586.0511487667402 178.11239451312218 -298.04278597547864
586.0511487667402 226.01768281801222 -239.9321268979552
586.0511487667402 286.807625522434 -176.68938242405147
586.0511487667402 363.94769219915764 -107.49887839832536
586.0511487667402 461.8354285936932 -31.529434050209147
586.0511487667402 586.0511487667402 52.06172599182537
586.0511487667402 743.6760536467558 144.19037307860845
586.0511487667402 943.6959110675486 246.01569530502275
586.0511487667402 1197.5133099937427 359.2770496279136
586.0511487667402 1519.5976911565988 486.8922686573037
586.0511487667402 1928.3102105817359 634.0218429830848
586.0511487667402 2446.9504592387466 810.1047667580224
586.0511487667402 3105.0847094578075 1033.2427237228057
586.0511487667402 3940.2314078349555 1341.1826979211046
586.0511487667402 5000.0 1824.8991415670225

743.6760536467558 5.0 -827.4520151356755
743.6760536467558 6.344805015839611 -813.3596066672126
743.6760536467558 8.051310137804697 -796.8092187123575
743.6760536467558 10.216798589284712 -777.6029267854783
743.6760536467558 12.96471898702334 -755.588540220379
743.6760536467558 16.451722811563343 -730.667277223858
743.6760536467558 20.87659468280201 -702.7944784287083
743.6760536467558 26.491584531418546 -671.9722805983674
743.6760536467558 33.616787682496685 -638.234455613378
743.6760536467558 42.65839262086404 -601.6247461081107
743.6760536467558 54.13183669370275 -562.1707625764648
743.6760536467558 68.69118979416318 -519.8558498806347
743.6760536467558 87.16644110999944 -474.59146844569796
743.6760536467558 110.6108145535225 -426.1927886520666
743.6760536467558 140.3608101970589 -374.360453734394
743.6760536467558 178.11239451312218 -318.67164816249533
743.6760536467558 226.01768281801222 -258.5831409746884
743.6760536467558 286.807625522434 -193.44699628871058
743.6760536467558 363.94769219915764 -122.53514140583093
743.6760536467558 461.8354285936932 -45.06146637224356
743.6760536467558 586.0511487667402 39.81992495538998
743.6760536467558 743.6760536467558 133.0729594680438
743.6760536467558 943.6959110675486 235.93909663075874
743.6760536467558 1197.5133099937427 350.2606980904943
743.6760536467558 1519.5976911565988 479.0721921326458
743.6760536467558 1928.3102105817359 627.6747147273218
743.6760536467558 2446.9504592387466 805.7182713791408
743.6760536467558 3105.0847094578075 1031.7158852129314
743.6760536467558 3940.2314078349555 1344.4124067633584
743.6760536467558 5000.0 1837.811536208018

943.6959110675486 5.0 -818.9367962206775
943.6959110675486 6.344805015839611 -807.8782435538451
943.6959110675486 8.051310137804697 -794.6161074905622
943.6959110675486 10.216798589284712 -778.8720917223845
943.6959110675486 12.96471898702334 -760.3863737841912
943.6959110675486 16.451722811563343 -738.9320903312951
943.6959110675486 20.87659468280201 -714.3269251501843
943.6959110675486 26.491584531418546 -686.4390622530505
943.6959110675486 33.616787682496685 -655.1854475476484
943.6959110675486 42.65839262086404 -620.5215353251187
943.6959110675486 54.13183669370275 -582.4231194400736
943.6959110675486 68.69118979416318 -540.8620821891836
943.6959110675486 87.16644110999944 -495.7787396696217
943.6959110675486 110.6108145535225 -447.05391236540345
943.6959110675486 140.3608101970589 -394.484036708282
943.6959110675486 178.11239451312218 -337.76258779523914
943.6959110675486 226.01768281801222 -276.47055226044904
943.6959110675486 286.807625522434 -210.07712628947093
943.6959110675486 363.94769219915764 -137.94828992414568
943.6959110675486 461.8354285936932 -59.354687379472125
943.6959110675486 586.0511487667402 26.539038361190705
943.6959110675486 743.6760536467558 120.73333190617586
943.6959110675486 943.6959110675486 224.546049515066
943.6959110675486 1197.5133099937427 339.9251334027763
943.6959110675486 1519.5976911565988 470.03476341483974
943.6959110675486 1928.3102105817359 620.3448942806172
943.6959110675486 2446.9504592387466 800.7734206499808
943.6959110675486 3105.0847094578075 1030.3710191663322
943.6959110675486 3940.2314078349555 1349.206134595427
943.6959110675486 5000.0 1855.3509019526318

1197.5133099937427 5.0 -799.0996913120089
1197.5133099937427 6.344805015839611 -790.5356241129889
1197.5133099937427 8.051310137804697 -780.0978784158615
1197.5133099937427 10.216798589284712 -767.4796989410047
1197.5133099937427 12.96471898702334 -752.3648582002484
1197.5133099937427 16.451722811563343 -734.4412432375848
1197.5133099937427 20.87659468280201 -713.4159384621844
1197.5133099937427 26.491584531418546 -689.0293734669522
1197.5133099937427 33.616787682496685 -661.0655983754009
1197.5133099937427 42.65839262086404 -629.3559362938286
1197.5133099937427 54.13183669370275 -593.7741942991006
1197.5133099937427 68.69118979416318 -554.2230746926903
1197.5133099937427 87.16644110999944 -510.61300681452394
1197.5133099937427 110.6108145535225 -462.8359228619829
1197.5133099937427 140.3608101970589 -410.73730871408907
1197.5133099937427 178.11239451312218 -354.09012132055113
1197.5133099937427 226.01768281801222 -292.5737725031695
1197.5133099937427 286.807625522434 -225.76005850902584
1197.5133099937427 363.94769219915764 -153.10508040846753
1197.5133099937427 461.8354285936932 -73.94095264765747
1197.5133099937427 586.0511487667402 12.547308104817148
1197.5133099937427 743.6760536467558 107.38655961801305
1197.5133099937427 943.6959110675486 211.96594060896587
1197.5133099937427 1197.5133099937427 328.3435035203979
1197.5133099937427 1519.5976911565988 459.831653974667
1197.5133099937427 1928.3102105817359 612.1087830107244
1197.5133099937427 2446.9504592387466 795.4407780158117
1197.5133099937427 3105.0847094578075 1029.5935849125817
1197.5133099937427 3940.2314078349555 1356.4193577059013
1197.5133099937427 5000.0 1879.551108650032

1519.5976911565988 5.0 -769.7805468113161
1519.5976911565988 6.344805015839611 -763.1788638226608
1519.5976911565988 8.051310137804697 -755.0371911169414
1519.5976911565988 10.216798589284712 -745.058932462397
1519.5976911565988 12.96471898702334 -732.9183796513439
1519.5976911565988 16.451722811563343 -718.2689244724397
1519.5976911565988 20.87659468280201 -700.754946585671
1519.5976911565988 26.491584531418546 -680.0264491602779
1519.5976911565988 33.616787682496685 -655.754487525559
1519.5976911565988 42.65839262086404 -627.6445751870392
1519.5976911565988 54.13183669370275 -595.4449388373955
1519.5976911565988 68.69118979416318 -558.9469958425866
1519.5976911565988 87.16644110999944 -517.976663397787
1519.5976911565988 110.6108145535225 -472.3768193150486
1519.5976911565988 140.3608101970589 -421.98283779155463
1519.5976911565988 178.11239451312218 -366.5942694541336
1519.5976911565988 226.01768281801222 -305.9460438860265
1519.5976911565988 286.807625522434 -239.6818167578881
1519.5976911565988 363.94769219915764 -167.3298401054999
1519.5976911565988 461.8354285936932 -88.27729919126614
1519.5976911565988 586.0511487667402 -1.7314537284601101
1519.5976911565988 743.6760536467558 93.3561724657543
1519.5976911565988 943.6959110675486 198.44497035847007
1519.5976911565988 1197.5133099937427 315.7128748500568
1519.5976911565988 1519.5976911565988 448.6485947622018
1519.5976911565988 1928.3102105817359 603.1970768895644
1519.5976911565988 2446.9504592387466 790.0887894254502
1519.5976911565988 3105.0847094578075 1030.0623812894937
1519.5976911565988 3940.2314078349555 1367.4240278501593
1519.5976911565988 5000.0 1913.5869878762378

1928.3102105817359 5.0 -733.4177491555988
1928.3102105817359 6.344805015839611 -728.3197083638074
1928.3102105817359 8.051310137804697 -721.9795493270503
1928.3102105817359 10.216798589284712 -714.131514370958
1928.3102105817359 12.96471898702334 -704.4710061102519
1928.3102105817359 16.451722811563343 -692.6569181250625
1928.3102105817359 20.87659468280201 -678.3175729866898
1928.3102105817359 26.491584531418546 -661.0606461464031
1928.3102105817359 33.616787682496685 -640.4866745427867
1928.3102105817359 42.65839262086404 -616.2047309157892
1928.3102105817359 54.13183669370275 -587.8477396426701
1928.3102105817359 68.69118979416318 -555.084212088736
1928.3102105817359 87.16644110999944 -517.6231676820366
1928.3102105817359 110.6108145535225 -475.2098731318233
1928.3102105817359 140.3608101970589 -427.61162997596466
1928.3102105817359 178.11239451312218 -374.5945290554064
1928.3102105817359 226.01768281801222 -315.89343410541005
1928.3102105817359 286.807625522434 -251.17774663848104
1928.3102105817359 363.94769219915764 -180.01416874382085
1928.3102105817359 461.8354285936932 -101.82417479466176
1928.3102105817359 586.0511487667402 -15.827161912739484
1928.3102105817359 743.6760536467558 79.0516090133815
1928.3102105817359 943.6959110675486 184.34878695873795
1928.3102105817359 1197.5133099937427 302.38133715879167
1928.3102105817359 1519.5976911565988 436.8576619674386
1928.3102105817359 1928.3102105817359 594.0761024135618
1928.3102105817359 2446.9504592387466 785.4056346041216
1928.3102105817359 3105.0847094578075 1032.942737468663
1928.3102105817359 3940.2314078349555 1384.4613801703308
1928.3102105817359 5000.0 1962.6064422315349

2446.9504592387466 5.0 -692.8147056042349
2446.9504592387466 6.344805015839611 -688.8519920905605
2446.9504592387466 8.051310137804697 -683.8948678780148
2446.9504592387466 10.216798589284712 -677.7152535426344
2446.9504592387466 12.96471898702334 -670.0439198799477
2446.9504592387466 16.451722811563343 -660.5684622795648
2446.9504592387466 20.87659468280201 -648.9337595809366
2446.9504592387466 26.491584531418546 -634.7458188083851
2446.9504592387466 33.616787682496685 -617.5796751046428
2446.9504592387466 42.65839262086404 -596.9913896667194
2446.9504592387466 54.13183669370275 -572.5331847307257
2446.9504592387466 68.69118979416318 -543.7695654506806
2446.9504592387466 87.16644110999944 -510.29126785146036
2446.9504592387466 110.6108145535225 -471.72334491513266
2446.9504592387466 140.3608101970589 -427.72412790468024
2446.9504592387466 178.11239451312218 -377.9730443354197
2446.9504592387466 226.01768281801222 -322.1468550214522
2446.9504592387466 286.807625522434 -259.8850782918671
2446.9504592387466 363.94769219915764 -190.74535671122476
2446.9504592387466 461.8354285936932 -114.14726122308957
2446.9504592387466 586.0511487667402 -29.297184685027787
2446.9504592387466 743.6760536467558 64.92411801454591
2446.9504592387466 943.6959110675486 170.15029489428525
2446.9504592387466 1197.5133099937427 288.8713547919724
2446.9504592387466 1519.5976911565988 425.0822148747693
2446.9504592387466 1928.3102105817359 585.5656992947443
2446.9504592387466 2446.9504592387466 782.5947893194298
2446.9504592387466 3105.0847094578075 1040.2209519130947
2446.9504592387466 3940.2314078349555 1411.2923807001207
2446.9504592387466 5000.0 2035.3758880798814

3105.0847094578075 5.0 -650.9456875683686
3105.0847094578075 6.344805015839611 -647.8329642167496
3105.0847094578075 8.051310137804697 -643.923227157246
3105.0847094578075 10.216798589284712 -639.0249105905782
3105.0847094578075 12.96471898702334 -632.9072008631438
3105.0847094578075 16.451722811563343 -625.2954959129593
3105.0847094578075 20.87659468280201 -615.8680853945134
3105.0847094578075 26.491584531418546 -604.2549465949364
3105.0847094578075 33.616787682496685 -590.0396911011771
3105.0847094578075 42.65839262086404 -572.7654715135936
3105.0847094578075 54.13183669370275 -551.9452111013784
3105.0847094578075 68.69118979416318 -527.075627704919
3105.0847094578075 87.16644110999944 -497.65315082246843
3105.0847094578075 110.6108145535225 -463.1887339532259
3105.0847094578075 140.3608101970589 -423.2174133611966
3105.0847094578075 178.11239451312218 -377.2984933780908
3105.0847094578075 226.01768281801222 -325.0028635508961
3105.0847094578075 286.807625522434 -265.8850897716152
3105.0847094578075 363.94769219915764 -199.43868938713558
3105.0847094578075 461.8354285936932 -125.0318026174732
3105.0847094578075 586.0511487667402 -41.816305442686826
3105.0847094578075 743.6760536467558 51.40746568947907
3105.0847094578075 943.6959110675486 156.40881927841656
3105.0847094578075 1197.5133099937427 275.9083190990932
3105.0847094578075 1519.5976911565988 414.29142919900005
3105.0847094578075 1928.3102105817359 579.0278180887453
3105.0847094578075 2446.9504592387466 783.713362259823
3105.0847094578075 3105.0847094578075 1055.3247419073105
3105.0847094578075 3940.2314078349555 1454.4904529555415
3105.0847094578075 5000.0 2147.8480541530807

3940.2314078349555 5.0 -610.893573582081
3940.2314078349555 6.344805015839611 -608.4128009485521
3940.2314078349555 8.051310137804697 -605.2879097542032
3940.2314078349555 10.216798589284712 -601.3590321927873
3940.2314078349555 12.96471898702334 -596.4307506883015
3940.2314078349555 16.451722811563343 -590.2664157998811
3940.2314078349555 20.87659468280201 -582.5827093390421
3940.2314078349555 26.491584531418546 -573.0451275017895
3940.2314078349555 33.616787682496685 -561.2652554886245
3940.2314078349555 42.65839262086404 -546.8008979834822
3940.2314078349555 54.13183669370275 -529.1599820572405
3940.2314078349555 68.69118979416318 -507.8088273861217
3940.2314078349555 87.16644110999944 -482.1844286701303
3940.2314078349555 110.6108145535225 -451.709241556091
3940.2314078349555 140.3608101970589 -415.8051498160157
3940.2314078349555 178.11239451312218 -373.9023337471267
3940.2314078349555 226.01768281801222 -325.43740185733077
3940.2314078349555 286.807625522434 -269.83573696702615
3940.2314078349555 363.94769219915764 -206.4724232356316
3940.2314078349555 461.8354285936932 -134.60621920345147
3940.2314078349555 586.0511487667402 -53.27681130588553
3940.2314078349555 743.6760536467558 38.85387521686971
3940.2314078349555 943.6959110675486 143.75781425238165
3940.2314078349555 1197.5133099937427 264.4829448591272
3940.2314078349555 1519.5976911565988 405.97398121469996
3940.2314078349555 1928.3102105817359 576.715767832351
3940.2314078349555 2446.9504592387466 792.326165962193
3940.2314078349555 3105.0847094578075 1084.394156789218
3940.2314078349555 3940.2314078349555 1526.2904557978072
3940.2314078349555 5000.0 2331.9339536664156

5000.0 5.0 -576.0171910421327
5000.0 6.344805015839611 -574.0012147701091
5000.0 8.051310137804697 -571.4566486969152
5000.0 10.216798589284712 -568.2493212448885
5000.0 12.96471898702334 -564.213533592882
5000.0 16.451722811563343 -559.1460578974174
5000.0 20.87659468280201 -552.7997461500645
5000.0 26.491584531418546 -544.8771487734357
5000.0 33.616787682496685 -535.0247662859174
5000.0 42.65839262086404 -522.8287710929449
5000.0 54.13183669370275 -507.8132513822652
5000.0 68.69118979416318 -489.4419423532404
5000.0 87.16644110999944 -467.1241313494552
5000.0 110.6108145535225 -440.22446145542153
5000.0 140.3608101970589 -408.07510631717923
5000.0 178.11239451312218 -369.9867589967221
5000.0 226.01768281801222 -325.25306219317827
5000.0 286.807625522434 -273.1413105681645
5000.0 363.94769219915764 -212.86084538167415
5000.0 461.8354285936932 -143.49884215475322
5000.0 586.0511487667402 -63.90875568757929
5000.0 743.6760536467558 27.47339857375937
5000.0 943.6959110675486 132.93475530886644
5000.0 1197.5133099937427 256.0190861641822
5000.0 1519.5976911565988 402.52448154208014
5000.0 1928.3102105817359 582.5306586311281
5000.0 2446.9504592387466 814.9548992137843
5000.0 3105.0847094578075 1139.2476883324289
5000.0 3940.2314078349555 1651.818302255584
5000.0 5000.0 2661.294217289984

